Upsilon invariant for graphs and the homology cobordism group of homology cylinders

Upsilon is a homomorphism on the smooth concordance group of knots defined by Ozsv\'{a}th, Stipsicz and Szab\'{o}. In this paper, we define a generalization of upsilon for a family of embedded graphs in rational homolog spheres. We show that our invariant will induce a homomorphism on the homology cobordism group of homology cylinders, and present some applications. To define this invariant, we use tangle Floer homology. We lift relative gradings on tangle Floer homology to absolute gradings (for certain tangles) and prove a concatenation formula for it.

==> diagram.tex <==
\message{==================================================================}%
\message{<Paul Taylor's commutative diagrams - version 3.96, December 2019>}%
%%
%%
%% This code runs the LaTeX \ProvidesPackage command iff it is defined.
%% included at the request of Michael Downes <mjd@ams.org> March 2002.
%% Put \listfiles in your LaTeX preamble to see what this is for.
\expandafter\ifx\csname ProvidesPackage\endcsname\relax\toks0=\expandafter{\fi
\ProvidesPackage
   {diagrams}[2019/12/31 v3.96 Paul Taylor's commutative diagrams]%%
\toks0=\bgroup}%%
%%======================================================================%
%%      TeX  macros for drawing category-theoretic diagrams             %
%%                                                                      %
%%                              Paul  Taylor                            %
%%                                                                      %
%%             		www.PaulTaylor.EU/diagrams			%
%%	www.ctan.org/tex-archive/macros/generic/diagrams/taylor/	%
%%			   diagrams@PaulTaylor.EU			%
%%                                                                      %
%%                           PLEASE READ THE MANUAL!                    %
%%                                                                      %
%%      Please ensure that you are registered with me as a user so that %
%%      you can be informed of future releases.  Any electronic mail    %
%%      message with "commutative" or "diagram" in the subject line     %
%%      (such as your request for the package, a question about it, or  %
%%      even an otherwise blank message) automatically registers you.   %
%%                                                                      %
%%                                                                      %
%% CONTENTS:                                                            %
%%  (O) corruption-sensitive hacks    (to approx line 318)              %
%   (1) dimensions and counts                                           %
%   (2) make arrow parts                                                %
%   (3) new arrow                                                       %
%   (4) horizontal state checking and arrow setup                       %
%   (5) syntax of arrow commands                                        %
%   (6) positioning and optional arguments                              %
%   (7) the diagram - options and output                                %
%   (8) the matrix                                                      %
%   (9) horizontals                                                     %
%  (10) piles                                                           %
%  (11) verticals                                                       %
%  (12) transfer to box arrays                                          %
%  (13) paragraph bombing                                               %
%  (14) reformatting objects and crosses                                %
%  (15) LaTeX line characters                                           %
%  (16) diagonals                                                       %
%  (17) stretchable diagonals                                           %
%  (18) PostScript arrows                                               %
%  (19) trigonometry                                                    %
%  (20) PDF-TeX support                                                 %
%  (21) error recovery                                                  %
%%      Arrow components & commands - starts approx line 1234           %
%% (22) auxillary macros for adjustment of components                   %
%% (23) bits of arrows  (\rhvee etc)                                    %
%% (24) arrow commands  (\rTo etc)                                      %
%% (25) miscellaneous                                                   %
%% Apart from these five sections, the rest is intended to be totally   %
%% meaningless in the undocumented version, which is approximately      %
%% 1922  lines long. Please do not waste trees by printing it out.      %
%  This is because I regard my code as private. The comments contain a  %
%  lot of fossils, ideas and other notes to myself which I do not wish  %
%  to make available to others. If you're reading this, please stop now.%
%%                                                                      %
%% COPYRIGHT NOTICE:                                                    %
%%      This package may be copied and used freely for any academic     %
%%      (not commercial or military) purpose, on condition that it      %
%%      is not altered in any way, and that an acknowledgement is       %
%%      included in any published work making substantial use of it.    %
%%                                                                      %
%%      IT IS SUPPLIED "AS IS", WITHOUT WARRANTY, EXPRESS OR IMPLIED.   %
%%                                                                      %
%%      If you are doing something where mistakes cost money (or where  %
%%      success brings financial profit) then you must use commercial   %
%%      software, not this package. In any case, please remember to     %
%%      keep several backup copies of all files, and check everything   %
%%      visually before sending final copy to the publishers.           %
%%                                                                      %
%%      You may use this package as a (substantial) aid to writing an   %
%%      academic research or text book on condition that                %
%%       (i) you contact me at a suitable time to ensure that you have  %
%%           an up-to-date version (and any infelicities can be fixed), %
%%      (ii) you send me a copy of the book when it's published.        %
%%                                                                      %
%% HISTORY                                                              %
%% 3.95 Released 31 December 2014					%
%%	Fixed spurious extra vertical space when running under LuaTeX	%
%	by adding \baselineskip\z@ to \bomb@parameters  14 May 2014	%
%%	with help from Linas Stonys.					%
%% 3.94 Released 11 May 2011						%
%%	defined <= tail							%
%% 3.93 Released 9 June 2009						%
%	added \pdfsyncstop to avoid clash with pdfsync			%
%	\ifx\diagram\isundefined					%
%	removed obsolete \laf \lad \xlad \lahh \lat \xlat \xlahh	%
%       changed \lq and \rq back to ` and ' for catcodes and octals.	%
%%	Added support for XeTeX, with help from Apostolos Syropoulos.	%
%% 3.92 Released 31 December 2007                                       %
%	Made noPS and noPostScript just generate error messages.	%
%       Unknown PS translator is just ignored.				%
%	Swapped \Yup and \Ydown						%
%       Two-year (instead of one-year) time-bombs.                      %
%% 3.91 Released 31 August 2006                                         %
%%	Renamed "noPostScript" option as "UglyObsolete".		%
%       Fixed? "PostScript translator `' unknown"			%
%       \everymath{}\everyhbox{} since pdfsync sets them                %
%% 3.90 Released 11 April 2004                                          %
%%      use PostScript=Rokicki not pure DVI by default                  %
%       pass PS prog name to \bad@ps@prog as #1 not as \@value          %
%       always warn that "labels as positional arguments are obsolete"  %
%       as ``superscript'' labels were introduced 14 years ago          %
%       test \ifx\pdfoutput\relax as well as \undefined                 %
%% 3.89 Released 7 July 2002                                            %
%%      Added support for pdftex, which is recognised automatically.    %
%% 3.88 Released 1 September 2000                                       %
%%      Square hook tail: \newarrow{SquareInto}{sqhook}--->             %
%% 3.87 Released 1 September 1999                                       %
%%      This version was used for the final 1200dpi PS copy of my book  %
%%      ``Practical Foundations of Mathematics'' (Cambridge Univ Press) %
%%      see   http://www.PaulTaylor.EU/Practical_Foundations            %
%% 3.86 Released 1 September 1998                                       %
%%      New options hug and nohug in PostScript mode: [PS,nohug] uses   %
%%      PS for the arrows without rotating the labels, but the way of   %
%%      calculating the actual position of these horizontal labels on   %
%%      will remain subject to alteration for some period of time ---   %
%%      please send me examples if you feel that adjustment is needed.  %
%%                                                                      %
%       flushleft/leftflush with no value retains old one, not 0pt      %
%       Suppress indentation of following text (due to LaTeX change)    %
%       inserted \global before \@ignoretrue                            %
%       Mangle \left@label and \right@label (conflict with Elsevier).   %
%%      midvshaft and snake for vertical arrows                         %
%       labels on verticals are now inside the lower \vbox              %
%%      New option [gap=width] (default=shortfall) to use instead of    %
%%      ~{\;} on horizontals and PS diagonals, as this caused ^ and _   %
%%      labels to be moved too far away from the shaft.                 %
%       Corrected position of hook in \dInto (see \shifthook).          %
%       Added 2pt space separating labels from vertical arrows.         %
%       Corrections to \lhtriangle \dhtriangle \newarrowtail{boldhook}  %
%%      Added >-> and <-< heads and tails, same as >> and << but the    %
%%      shaft goes *through* the extra arrowhead.                       %
%       Identify the cell in which a second-pass error occurs.          %
%       Corrected dot spacing with [dotted] option.                     %
%       (It was using \hfdot or \vfdot not \rf:. or \df:.)              %
%% 3.85 Released 20 August 1997                                         %
%%      New option [crab=distance] shifts horizontals and PS diagonals  %
%%      transversally by the specified distance (positive=upward).      %
%%      New option [snake=distance] shifts midshaft horizontals and     %
%%      PS diagonals longitudinally by the specified distance.          %
%       Set \catcode of :;!? as babel package makes them \active.       % 
%       \dblvert for ``Practical Foundations''                          %
%       Moved pullback symbols slightly further away.                   %
%       Fixed uneven \pile spacing.                                     %
%       Treat empty row as \noalign{\advance\prevdepth-\baselineskip}   %
%       Unknown PostScript translator names recognised.                 %
%       Parse space in $A\rTo^a _b B$ correctly.                        %
%       Big \LaTeX arrowheads with [thick] option.                      %
%%      New option [leftflush], like [flushleft] but reckons alignment  %
%%      from multiple verticals, or from text if there's no vertical.   %
%       Crude implementation of nohug.                                  %
%%      Most of the history has been suppressed from the user version.  %
%  3.84 Released 2 September 1996                                       %
%       Fixed undefined control sequence in \luOnto[dotted,PS]          %
%       moved \let\fill@dot\hfdot from \Horizontal@Map to \@setup@horiz %
%       Use \AtEndDocument to give once only warnings.                  %
%       Report unknown grid correctly.                                  %
%       Provided \NWclck etc 2-cell arrows.                             %
%% 3.83 Released 18 May 1995                                            %
%%      "dotted" option (set dot filler on maps)                        %
%       repositionpullbacks moved 0.25em horizontally                   %
%       fixed bug when \v@grid is longer than required                  %
%       added \relax in \over@print to avoid premature expansion        %
%       (to fix bug with repositionpullbacks \NWpbk and \SWpbk)         %
%       Fixed bug with interaction with amslatex/equation.              %
%       reported by Bruce Pollack; caused by \everycr.                  %
%%      Parallel maps (\pile) outside diagrams stretch correctly.       %
%       Added test \ifinpile to glue in horizontal maps.                %
%       Avoid stepped lines in PostScript by restricting the slopes.    %
%       Define \default@max@fraction=\default@size/5\pixel@size.        %
%       Rightmost width now calculated correctly.                       %
%       \reoutput@cell had spurious \box\cd@cell in it.                 %
%       Fewer "arrow too short" errors (the l> option for eliminating   %
%       birds' feet arrows is only applied in text, l>.5em in diagrams).%
%       Setting \dimen2 in \@setup@horiz, \default@args, \calc@horiz.   %
%       Recovery from "\rTo_\hbox{a}" no longer loops.                  %
%       Match TeX's inserted { with \eegroup instead of \egroup.        %
%       "midshaft" option now works; "midvshaft" ignored.               %
%%      Option "LaTeXeqno" uses LaTeX's equation number and style       %
%%      for "eqno";  LaTeX's \label command picks this up.              %
%%      Suppress warnings & 2nd pass errors with "silent" option.       %
%       Warning if extra material in \pile cell.                        %
%       Recover from square brackets mis-interpreted as options.        %
%  3.82                                                                 %
%% 3.81 Second alpha release 18 July 1994                               %
%       Fixed displaced parenthesis instead of hook tails in manual p8. %
%       By changing \box0 to \box3 in \raisehook (LaTeX2e \boldmath).   %
%       Parentheses and braces (not quite right): see end of source.    %
%%      \overprint{text} sets text in maths and overprints it in the    %
%%      current cell, centered in the column irrespective of other stuff%
%%      "repositionpullbacks" option uses this for \SEpbk etc           %
%%      \newdiagramgrid declaration, grid option and pentagon grid.     %
%% 3.80 Alpha release for adjusted diagonals 15 July 1994.              %
%       Some options can now take (x,y) values.                         %
%       Position during input as (\cd@row,\cd@cell); top left is (1,1). %
%       Name of DVI->PS translator as argument to PostScript option.    %
%       Preliminary code for stretchable diagonals and overprints:      %
%       \missive#1(x,y) anywhere in the diagram overprints #1 at (x,y). %
%       The extra boxes are added to the left of each cell, delimited   %
%       by \penalty-9990; this caused the paragraph builder to discard  %
%       the \hfil\kern(shortfall) on the left, so added \null.          %
%       Improved recovery from missing {} in labels.                    %
%       Recovers from \rTo~\rTo,  \rTo^\hat,  \rTo^\macro,  {\rTo^},    %
%       \rTo^ {&, ...                                                   %
%       Removed error message from \across since this works now.        %
%       Set \boxmaxdepth=\maxdimen for interaction with an old LaTeX.   %
%       Loading after \begin{document} in LaTeX2e possible.             %
%       (By testing whether \DeclareOption has been disabled (yuck).    %
%       Loading before \documentstyle or \documentclass possible.       %
%       (By defaulting \MapBreath and \default@mapbreadth to 0.4pt;     %
%       the latter is \edef'd in \size@dependencies.                    %
%       Equilateral triangle or regular hexagon size options.           %
%       \mathon and \mathoff correctly matched now, it seems.           %
%       Corrected Morse code for "P" (Ralph Loader)                     %
%       Changed all \new@if to \if@blah@. Added \if@in@matrix@.         %
%      Introduced landscape and portrait options.                      %
%       Define PS commands once for each (outermost) diagram needing    %
%       them; previously they were defined for every map.               %
%       Don't hide width of vertical middle components.                 %
%       (Changed \make@vert@part to \hbox in \newarrowmiddle.)          %
%       Negative stretchability in right half of horizontal arrows.     %
%       Added "." map qualifier to set dot filler.                      %
%       Only set \@diagonals@used@ for those set on first pass.         %
%       Parse []-options during label processing.                       %
%       Signal midhshaft with extra \penalty1 just before bomb.         %
%       Made midhshaft work; always set it for single-row diagrams.     %
%       Rewrote \widen@horiz, changing tests for space and handling of  %
%       through and centred horizontals.                                %
%       Maintain distance of each row from the top as \ht\cd@row on     %
%       rows which have been reformatted; used to calculate height of   %
%       diagonals.                                                      %
%       \diagramstyle may be used within diagrams.                      %
%       (Continuation, \after@opt@arg, not set, so did \@@@diagram.)    %
%       \objectwidth reduced from 3em to 1em; was destroying fixed      %
%       diagonals.                                                      %
%       Fixed "very" thick lines by changing \cds@thick.                %
%       All inter-row glue contributes to space.                        %
%       Vertical maps targetted at labels of horizontals avoid them.    %
%       Wide object on right no longer causes "increase width" warning. %
%       (Initialise \far@end@cell=1000 on right, don't complain about   %
%       insufficient space between objects if it still has this value.) %
%       Make these warnings more accurate and informative.              %
%       Fixed decapitated arrows (I think!).                            %
%       Now use \wd\cd@donat for \column@placing ie x-coord of centre.  %
%      Diagonals adjusted to meet their endpoints, at last!!!!         %
%       \min@map@length=0pt inside diagrams (?).                     %
%       Option showfirstpass[=depth].                                   %
%       Fixed intermittent "lower part of vertical too short" errors:   %
%       wasn't collecting the vertical glue below missives.             %
%       Missive aimed at horizontal map caused huge \right@donated: was %
%       overwriting \dimen2; moved most of the code within an \hbox.    %
%  3.29 Released 11 March 1994                                          %
%       Corrected error message when "&" or object is inserted before   %
%       horizontal maps etc outside diagram.                            %
%       \last@map@type initialised to \empty, when we just say "before".%
%       Also when label missing after <>^_~.                            %
%       Switch to centredisplay if flushleft doesn't fit on the page.   %
%       The code was ok when the diagram didn't fit at all, but not in  %
%       the case where it would fit in centredisplay mode.              %
%       Added Y head & tail from St. Mary Rd. font (not yet adjusted).  %
%       First attempt to support LaTeX2e \usepackage options.           %
%       Fixed bug (missing \endgroup and no arrow) with \rTo[opt][opt]. %
%       (The continuation, \after@opt@arg, had got overwritten.)        %
%       Set \mathsurround=0pt for everything within our code.           %
%       Already set in \inner@environment and in \make@horiz@part but   %
%       not when \math@on & math@off are (re)made in \size@dependencies.%
%       Also set it in \default@args for horiz maps outside diagrams.   %
% 3.28 Released 30 November 1993                                       %
%       Fixed bug causing diagram to disappear in vert mode in LaTeX    %
%       caused by \everypar overwriting \box0 - use \box2 instead.      %
%      Peter Freyd's \puncture symbol provided.                        %
%  3.27 Released 26 March 1993                                          %
%       Fixed bug which forced LaTeX slopes on PostScript diagonals.    %
%       Got \max@fraction wrong: moved to condition in \exec@diagonal.  %
%       Renamed \put@PS@horiz as \exec@PS@diagonal. Made \exec@horiz    %
%       exclusively horizontal, moving "extra text" test there.         %
%       Call \calc@horiz and \label@horiz from \exec@diagonal instead.  %
%       Restored \max@fraction{255} to PostScript arrows.               %
%  3.26 Released 11 February 1993                                       %
%       Added [defaultsize=] to set \default@size, used if size unset.  %
%       Added 1pt space between label (strut) and horizontal shaft.     %
% 3.25 Released 30 January 1993                                        %
%       Resolution-dependent fudge (dpi) applied to horizontal arrows.  %
%       Removal of glue from before to after applied to display as well %
%       as textflow, but didn't deal with spurious space after diagram. %
%       Fixed extra height in \rhla.                                    %
%       Fixed \HmeetV vertical profile - bug caused by pixel fudge.     %
%       Defined \if@ignore outside LaTeX, use to control \ignorespaces  %
%       at end of diagram: to cure spurious space in text after         %
%       notextflow diagram.                                             %
%       Added \kern-\displayindent inside $$/$$ to over-ride prevailing %
%       paragraph indentation: to cure shift and over-full \hbox in     %
%       itemized diagram.                                               %
%       Added \make@end@at@line after \egroup in \output@diagram so that%
%       "too wide for page" and "flushleft in $$" can give line numbers.%
%      LaTeX heads made default (unless \tenln undefined, when vee)    %
%       and set (by new \set@default@arrowhead) in horiz outside cd too.%
%       Also cures zero-length shafts of arrows in text in footnotes.   %
%       Made \labelstyle and \objectstyle available as options.         %
%       Diagram options and output as new section; some reorganisation. %
%       New display options give warning if used within maths.          %
%       Catch missing bracket at end of label and misplaced (but not    %
%       missing) bracket at end of \pile.                               %
%       Small adjustments on some heads and tails. hbox option.         %
%       Braces and parentheses as arrows (bits from cmex) commented out.%
%       Bits of double vert arrows use cmex not \Vert\Uparrow\Downarrow %
%      Circle, cross, little vee, little black triangle heads.         %
%       Fixed spaces before & after diagram in display and textflow.    %
%       Catch em-braced arrow commands.                                 %
%       Adjusted hook tails yet again (some theory behind horizontals!).%
%       Smashed height of \rhla \lhla \rtla and \ltla.                  %
%       Default \MapBreadth as TeXbook p447; pixel round on input.      %
%       Apply pixel rounding to \make@vert@part and \shifthook.         %
%      First-use warning when defaulted diagonal components are used.  %
%       Warning if diagonals used & columns stretched significantly.    %
%       Warning if diagonals with repeating components are too short.   %
%       Added \@use@TPIC@false to diagonal dot repeater.                %
%       Changed setup of diagonal maps; now \+To gets immediate control,%
%       sets defaults, calls \rTo (having changed \Horizontal@Map) and  %
%       the test to use PS is after the arguments have been read.       %
%       Local PostScript option (PS, noPS), disabled by noPostScript.   %
%       Collected all size-dependent initialisations in one macro, which%
%       is executed before \diagram, \diagramstyle or text arrows.      %
%       Allowed curly instead of square brackets in \diagramstyle.      %
%       Also \diagramsstyle.                                            %
%      AMSTEX emulation - works at least when amstex not present.      %
%       Check for \diagram options changed to \futurelet (the earlier   %
%       problem with this lay in using \next@token twice), so it now    %
%       catches a blank line after \diagram or \begin{diagram}.         %
%       Fixed \HmeetV yet again.                                        %
%       Added Morse Code signature to every 20th suitable horizontal.   %
%       Position horizontal labels using strut rather than \baselineskip%
%       Change definitions of default components from \def to \let.     %
%       This brought lower \scriptstyle labels closer to horizontals.   %
%       Use \boldmath for littlevee and hooks, if available. (DUBIOUS)  %
%       Vertical position of labels on diagonals had been unset!        %
%       Increased interim assumed \objectheight from .5ex to 1.8ex and  %
%       isolated \interim@shortfall.                                    %
%       Removed \outer from \diagramstyle.                              %
%       Lots of adjustments to bits of arrows (drives me mad!).         %
%% 3.24 Release 7 Sept 1992 advertised to users.                        %
%       Continued fractions, sine, cosine & pythagorean sum.            %
%       \newarrow etc also define \+To \-To \nwTo                       %
%       Rewrote LaTeX diagonal code:                                    %
%       uses continued fractions to find nearest slope and selects      %
%       character; diagonals touch a square around the (maths axis)     %
%       centre of the endpoints; middles; through diagonals.            %
%       \lq and \rq (instead of ` and ') for catcodes and octals.       %
%       Made it consistent with texinfo - for loading, at least.        %
%      PostScript option introduced:                                   %
%       \Rising@Map and \Falling@Map choose the horizontal command and  %
%       run \put@PS@horiz;                                              %
%       labels are rotated together with the arrow,                     %
%       which is set in the first pass                                  %
%       meets a circle and is not yet adjusted for its endpoints.       %
%      LaTeX, vee, curlyvee, triangle & blacktriangle heads & tails    %
%       provided and correctly adjusted; double heads & tails all made  %
%       with \make@double@head.                                         %
%      TPIC option introduced as an alternative to \LaTeX@make@line.   %
%  3.23 (14.5.92) experimental release on 10 July 1992                  %
%       Fixed pilespacing, and horizontal positioning of verticals      %
%       (bugs which arose from Seely's challenge). Also made need extra %
%       message work. Discovered that \get@arg finds \end@cell, not &,  %
%       so removed {} from \tokcase and \catcase, so the \mathord{}s    %
%       disappeared.                                                    %
%       Fixed vmiddle positioning of one-row diagrams.                  %
%       Fixed catastrophic error of empty first cell in nested diagram  %
%       by using \bbgroup\eegroup around the diagram.                   %
%       Moved making of \math@on@box to inside \bombparameters because  %
%       it caused "math formula deleted - insufficient fonts" if loaded %
%       before \documentstyle. deleted \defaultarrowhead{vee} for same. %
%  3.22 (14.5.92) experimental release                                  %
%  3.21 (1.5.92)                                                        %
%       Extra line of paragraph, to contain profile information.        %
%       Implemented \shift (\cd@hshift).                                %
%       Use \wd\cd@donat for column widths.                             %
%       New reformatting program.                                       %
%       Re-arranged the code.                                           %
%       Optional arguments on \diagram, maps and \diagramstyle.         %
%       Horizontal \shift; tight cell width and height (option).        %
%       top, vmiddle, bottom positioning - aligns chosen maths axes     %
%       origin, balance, nobalance horizontal positioning               %
%       Made \PileSpacing between verticals local.                      %
%       Fixed \HonV and \HmeetV profile. Included verticals in width.   %
%       Piles vertically centered ignoring outer labels.                %
%       Labels on horizontal maps positioned using \baselineskip 1.3ex. %
%       Extra .2ex spacing around labels removed, .2em reduced to .1em  %
%       midshaft option to centre labels in horizontal arrow shaft.     %
%       Through horizontals and verticals.                              %
%       \@and\sp\sb\space in \switch@arg; local catcode &,$             %
%       Re-wrote mangletex to substitute our internal command names.    %
%       \CellSize=default on entry, in case the font size is different. %
%       \across adds its with to \cd@hshift                             %
%       Fixed unterminated verticals and cross profiles.                %
%       Move labels away from wide vertical arrow middles.              %
%       Added strut in \get@label to stop verts hitting middle labels.  %
%       Re-wrote \newif to make it manglable.                           %
%  3.20 (29.4.92) early release of version 4                            %
%  3.19 (9.4.92)                                                        %
%       Ensure \enddiagram occurs only at correct {}-level              %
%       by using \aftergroup.                                           %
%       Blank line and \par within diagram =\enddiagram.                %
%       Clashing (horizontal) arrows detected at first pass             %
%       using an automaton;                                             %
%       "&" (etc) inserted, with error & help messages.                 %
%       \Pythagorean@sum.                                               %
%      Postscript arrows (basic code).                                 %
%      Implemented \newarrow \newarrowhead etc.                        %
%       Corruption-sensitive characters avoided wherever possible.      %
%       Reloading prevented.                                            %
%      Horizontal arrows outside diagram can stretch by wordspacing.   %
%  3.18 (18.12.90) bugfix                                               %
%       Diagonals (other than basic ones) moved to extra-diagonals.tex. %
%       Changed \lt and \gt to \lessthan and \greaterthan for Roy Crole.%
%      Added < and > for labels on left and right of arrow;            %
%       also [] for optional arguments on arrows (not used yet);        %
%       also displaced \catcase\bgroup (positional label) to speed up a %
%       bit as this is obsolete.                                        %
%  3.17 (10.9.90) bugfix                                                %
%       \offinterlineskip in \make@vert@part                            %
%       \endgraf instead of \par (because LaTeX changes it)             %
%       \leavevmode before diagram to fix LaTeX-interaction bug         %
%       \cong as a middle (problem was \mathpalatte within \edef)       %
% 3.16 (20.7.90) as mass mailed; only have mangled version             %
%       \DiagonalLineSegments=\ObsCount                                 %
%       \dmcornervert et seq commented out                              %
%  3.15 (1.7.90) numbered boxes for columns                             %
%       left part of horiz arrow in \box2 (\across not yet fixed)       %
%       bugfixes:                                                       %
%       spacing of \pile's                                              %
%       horizontal alignment of top of verticals - remove spurious space%
%       horizontal alignment of verticals - \make@vert@part             %
%       zero height & depth of vertical parts to not force lines apart  %
%  3.14 (1.7.90) bugfix:                                                %
%       parsing \across - remove spurious &                             %
%       horizontal alignment of bottom of multiple verticals.           %
%       \lhla arrow the right way round.                                %
%       add \MapShortFall and \MapCorner                                %
%  3.13 (2.6.90) A lot?                                                 %
%  3.11 (18.4.90)                                                       %
%       Catch obsolete parameters, rename some dimensions, added to     %
%       \bombparameters. Changed template.                              %
%  3.03 (18.4.90) re-arranged code; a lot of changes?                   %
%  3.02 (3-7.2.90)                                                      %
%  3.01 (9.1.90) vertical reformatting; only have mangled version       %
%% -- all following version numbers are post-facto --                   %
%%  3   (Jan 90) stretching vertical arrows                             %
%   2.8 (2.1.90) new reformatting                                       %
%   2.6 (30.12.89) added \pile                                          %
%%  2   (Sept 89) horizontals stretch to objects; "superscript" labels  %
%%  1   (1987) horizontal arrows stretch to edge of cell                %
%%  0   (1986) implementation of Knuth's TeXercise 18.46 for my thesis  %
%                                                                       %
%%======================================================================%

% BUGS
% mangle \@name

% "Commutative Diagram: "&*&" inserted between horizontal map and pile."
% in inline diagram

% Silvio Levy <levy@msri.org> 13 Sept 2006 - see examples
% width of diagram takes account of labels on arrows but not
% the width of the last row of objects

% signature on squashed arrow
% re-sort the obfuscation list, as Robin Houston has found the macros.

% missing } after \pile doesn't recover

% \across doesn't work with grid
% this code wasn't updated when we changed the use of \column@placing
% \ldTo^~p
% \begin{diagram} ended by \end{displaymath} causes havoc!

% When a diagram is immedately followed by a footnote, there is no
% space between the bottom of the diagram and the footnote rule.

% \begin{diagram}[htriangleheight] with default \DiagramCellHeight
% - Volker Schubert <volli@tunix.mathematik.uni-stuttgart.de> 5 Feb 1997

% midshaft on objects in a \pile

% $R:X\rEmbed[heads=littlevee,l>=1.5em] Y$ is not very pretty:
% \verb/$R:X\rEmbed[heads=littlevee,l>=1.5em] Y$/.

% make the rule in \verb/\upperBrace/ thicker and shorter;
% the vertical brace is also ugly.

% switch to balance within flushleft doesn't work

% make bottom right of negative gradient diagonals 2pt less shortfall

% doesn't insert } correctly in
% \uInto<{b_!={!_L^*} \adjoint \dOnto>{b^*}
   
% TO DO THIS TIME
% -     locate option to define origin of coordinates for diagonals
% -     text in the middle of right triangles
% -     diagonal pullback symbols
% -     handle \verb/\qed/

% -     \verb/vtriangle/ is too narrow (or too tall).
% -     we really ought to have curved arrows!
% -     define \verb/\Nanti/ and \verb/\Sclck/ 3/8-circle little arrows
% -     do ``\verb/=/'' middle using two ruled lines.
% -     wavy diagonal lines.

% -     check interaction of landscape with other positioning options
% -     option to set left or right width of object, rather than the shift
%       2-cells near vertices, offset annotation of vertices.
% -     annotation on arrowheads and XYpic adjustable positioning of labels
% -     Font sizes (line10) & \CellSize for slitex and 11pt/12pt (scaling?)
%       default rule breadth in slitex.
% -     give co-ordinates of cells (their line numbers?) in error messages

% TO DO NEXT TIME

% DIAGONALS
% -     steep \rdTo_u places the label very low down
% -     dashed diagonal should perhaps be dotted outside PS
% -     with shallow LaTeX diagonals, measure the width, not the height
% -     option to link diagonals to corners of objects instead of
%       aiming at the centres of the cells.

% OUTPUT OPTIONS
% -     argument to origin option
% -     re-calculate \prevgraf based on height of diagram and \baselineskip
% -     allow for short line before displayed diagram
% -     \output@cell doesn't take account of everything that sticks out.
% -     textflow diagram disappears immediately after displaymath envt.
% -     some rows remain unreformatted: one-line diagram enclosed in
%       \begin{diagram} \end{displaymath} in ptbook.sty.
% -     textflow generating horizontal space in paragraph (manual, page 3)

% BITS OF ARROWS
% -     make test file for all arrow styles and measure shortfall
% -     LaTeX diagonal double tails need to be brought in a bit
% -     option for shaft to go through double arrowhead; use difference in
%       width of head and tail to choose spacing of double heads
% -     curved corners on \HmeetV and half arrows; jumps and solders.
% -     loops on vertices: see Pino's bits
% -     electronic components
% -     \nwarrow etc as (1,1) LaTeX diagonals
% -     horizontal shaft one pixel too low for LaTeX heads and one pixel
%       too high for curlyvee, at 300dpi
% -     pixel adjustment on LaTeX diagonals
% -     move the dots closer together

% DIAGNOSTICS
% -     count number of lines since last & (\end@cell is more accurate)
%       we do this (\cell@at@line), but what for?
% -     make manual a LaTeX2e document.
% -     "maps must never be enclosed in braces" from shifted diagonal
% -     decide and document how much unterminated arrows stretch
% -     lower unterminated downward verticals
% -     allow unterminated maps to stretch to their natural width
% -     classified summary of options in manual; list of errors,
%       shift labels in options description to right
% -     option not to load error messages (ask how many users care about this)
% -     new display options should detect $$ not $ (probably useless in latex)
% -     missing \endcsname in various places:
%       in LaTeX2e \usepackage[flushleft=\mainindent]{diagrams}
%       in zed.sty from <> in diagrams.tex and \newarrow{blah}---->

% IDEAS
% -     make midvshaft work
%       all of the labels on a system of parallel verticals must align
% -     parametrise size of pullback symbols and crosses
% -     rewrite amscd.sty
% -     half arrows
% -     adjunction environment
% -     time bomb
% -     Lamstex & xypic fonts
% -     private version of \def with option to check re-definition; also
%       re- & \global loading - with the aim of doing it on first use
% -     \protect to arrows in section headings
% -     more space around labels on in-text arrows if in \displaystyle


% UNREPEATABLE BUGS
% -     \pile{text\rTo\\text\rTo} doesn't stretch correctly
%       seems to work.
% -     missives addressed to empty cells are lost - give error message
%       they appear to be handled ok.

% COMPLAINTS AND WISHES
% -     \hidewidth in objects causes arrows to overprint
% -     \rTo{}{} puts struts in both labels - forces \pile apart (obsolete)
% -     can't catch runaway argument to \pile
% -     multi-line labels with embedded arrays
%       this would have same problem as \pile in catching missing closing brace
%       long objects doing this automatically (paragraph?)
%       set up complete environment for labels
%       allow Sb and Sp environments for label? can't see any way!
% -     LaTeX center environment is unrestricted horizontal
%       may want restricted horizontal mode behaviour there.
% -     could \catcode`\&=\active etc and re\catcode (for texinfo)
% -     write size information to .aux? what?
% -     draft mode - what should(n't) it do?
% -     strings, Feynman diagrams, ...
% -     curved lines: see /home/leonardo/tex/contrib/Gnu/gs23/escher.ps
%       sorry, this doesn't work with dvips because it does ``bind def''
% -     \diagram[notextflow]..\enddiagram\begin{something}..\end{something}
%       makes \end{something} do \ignorespaces.
% -     prevent pagebreak before textflow diagram? penalties seem ok
% -     Dusko wants automatic hidden line elimination
% -     option to set the width of each column individually using missives
%       (grid option does this ok, I think)
% -     (probably) cannot work with TeX-XeT because of extra whatits
% -     macros as diagram options (Volker Schubert)
%
%%======================================================================%
%%                                                                      %
%%      (1) CORRUPTION-SENSITIVE HACKS                                  %
%           AND PROGRAMMING FEATURES                                    %
%%                                                                      %
%%======================================================================%

%%                      CORRUPTION & \catcode WARNING

%% BITNET (IBM) machines may corrupt certain important characters
%% in transmission by electronic mail:
%%        0123456789=digits, abcdefghijklmnopqrstuvwxyz=lowers,
%%        ABCDEFGHIJKLMNOPQRSTUVWXYZ=uppers, @=at (internal names),
%%        {}=curly braces (grouping), \=backslash (keywords),
%%        %=percent (comment), #=hash/sharp (argument), +=plus, -=minus,
%%        <>=angle brackets (relations \ifnum,\ifdim), ==equals,
%%        ,=comma, .=dot, :=colon, ;=semicolon,  =space
%% $=dollar (maths) is only used in the "bits of maps" section

%% The following characters are marked by a comment including the word "ASCII",
%% except in comments and messages:
%%        &=and (alignment), ~=tilde, |=vertical, []=square brackets,
%%        ^=caret (superscript), _=underline (subscript),
%%        "=double quote (hex), ()=round brackets,
%%        /=slash, ?=query, !=pling/bang, 
%% The following are no longer flagged:
%%        `=grave/backquote (catcodes), '=acute/single quote (octal),

% check by the command:
%       sed -e 's/.*%ascii.*//' -e 's/%.*$//' < diagrams.tex |\
%       grep -n '[][&()*?|~^_/\!\"']

%       Andrew Molitor <amolitor@wesleyan.earn> 27.3.91 says:
%       caret became a space or was eaten entirely, not sure which,
%       and tilde became a caret.

% changed \lq and \rq back to ` and ' 15.10.2008 (v3.93)
% as part of the adaptation to XeTeX proposed by
% Apostolos Sypopoulos <ijdt.editor@gmail.com>

%% The \catcode's marked * are assumed for reading this file:
%%          \=0* {=1* }=2* $=3 &=4 return=5* #=6 ^=7 _=8 ignored=9*
%%          space=10* letter=11* other=12 active=13 %=14* invalid=15
%% If you want to load this package inside Stallman's "texinfo", you must do
%% @catcode`@\=0 \catcode`\%=14 \input diagrams \catcode`\%=12 \catcode`\\=13
%% and then use @diagram @rTo @\ @enddiagram etc. (braces {} stay the same).
%% Also need @catcode`@&=4.

%%*** You *MUST NOT* use the internal commands (with names beginning \CD@)****
%! p \CD@
%! m \across@cells
% m \actually@braces@missing@around@macro@in@label
%! m \add@and
%! m \add@and@and
%! m \add@cr
%! m \add@dollar
%! m \add@empty@and
%! m \add@endpile@and
%! m \add@relax@before@square@bracket
%! m \@adjust@flush@left@false
%! m \@adjust@flush@left@true
%! m \after@diagram
%! m \after@name
%! m \after@names
%! m \after@opt@arg
%! m \amstex@diagram@setup
%! m \amstex@prefix
%! m \@and
%! m \and@in@pile
%! m \and@name
%! m \assign@at
%! m \assign@five
% m \at@
%! m \at@least
%! m \at@line
%! m \at@most
%! m \avoid@object
% m \axisheight
%! m \axis@profile
%! m \@back
%! m \bad@arrow
%! m \bad@end@label
%! m \bad@group@after@map
%! m \bad@pair@opt
%! m \bad@ps@prog
%! m \bbgroup
%! m \begin@at@line
%! m \@begin@cell
%! m \begin@cell
%! m \begin@maths
%! m \begin@pile
%! m \begin@square@name
%! m \better@use@ps
%! m \bgroup@name
%! m \body@
%! m \body@@
%! m \body@@@
%! m \@bomb
%! m \bomb@parameters
%! m \boxc@unt
% m \@brace
%! m \braced@label
% m \break@args
%! m \buffer@to@row
% m \@c
%! m \calc@horiz
% m \@catcode
%! m \@cd@a@false
%! m \cd@and
%! m \@cd@a@true
%! m \cd@balance
%! m \@cd@b@false
%! m \cd@bottom
%! m \cd@box@g
%! m \@cd@b@true
%! m \cd@cell
%! m \@cd@centre@display@false
%! m \@cd@centre@display@true
%! m \@cd@centre@hlabel@false
%! m \@cd@centre@hlabel@true
%! m \@cd@centre@vlabel@false
%! m \@cd@centre@vlabel@true
%! m \cd@cross
%! m \cd@diag@zer
%! m \cd@dim@a
%! m \cd@dim@b
%! m \cd@dim@g
%! m \cd@dim@h
%! m \cd@dim@k
%! m \cd@display
%! m \cd@display@box
%! m \cd@donat
%! m \cd@environment
%! m \cd@eqno
%! m \cd@error
%! m \cd@first@use
%! m \cd@fullwidth
%! m \@cd@g@false
%! m \cdgh@
%! m \@cd@g@true
%! m \cdgv@
%! m \@cd@hbox@false
%! m \@cd@hbox@true
%! m \cd@horiz@positioning
%! m \cd@hshift
%! m \@cd@landscape@false
%! m \@cd@landscape@true
%! m \cd@left
%! m \cd@left@donat
%! m \cd@left@margin
%! m \@cd@leqno@false
%! m \@cd@leqno@true
%! m \@cd@missive@false
%! m \@cd@missive@true
%! m \cd@mode@outside
%! m \cd@name
%! m \cd@num@a
%! m \cd@num@b
%! m \cd@num@c
%! m \cd@num@d
%! m \cd@num@g
%! m \cd@num@h
%! m \cd@obs@count
%! m \cd@obs@dim
%! m \cd@obs@dimq
%! m \cd@obs@msg
%! m \@cd@one@liner@false
%! m \@cd@one@liner@true
%! m \cd@opt@prefix
%! m \cd@penalty
%! m \cdps@  don't mangle any of these!
% m \cdps@Bechtolsheim
% m \cdps@Clark
% m \cdps@dvips
% m \cdps@dvitops
% m \cdps@dvitps
%! m \@cd@PS@horiz@false
%! m \@cd@PS@horiz@true
% m \cdps@IntegratedComputerSystems
% m \cdps@oztex
% m \cdps@RadicalEye
% m \cdps@Rokicki
% m \cdps@Trevorrow
%! m \cd@refmt@error
%! m \cd@right
%! m \cd@right@donat
%! m \cd@row
% m \cds@  don't mangle any of these!
% m \cd@shouldnt
%! m \cd@state
%! m \cd@switch@arg
%! m \cd@text@flow
%! m \@cd@text@flow@false
%! m \@cd@text@flow@true
%! m \@cd@through@false
%! m \@cd@through@true
%! m \@cd@tight@false
%! m \@cd@tight@true
%! m \cd@top
%! m \cd@top@height
%! m \@cd@use@PS@false
%! m \@cd@use@PS@true
%! m \cd@vbottom
%! m \cd@vcentre
%! m \cd@vert@positioning
%! m \cd@vmiddle
%! m \cd@vtop
%! m \cd@warning
%! m \cd@with@opt
%! m \cd@zerowidth
%! m \cell@at@line
%! m \cell@height@to@width
%! m \cell@missive
%! m \check@fated@enddiagram
%! m \check@horiz
%! m \check@part
%! m \check@vert
%! m \Climbingfalse
%! m \Climbingtrue
% m \@cmex
%! m \cmex@vert@part
%! m \column@placing
%! m \completed@depth
%! m \complete@horizontal
%! m \complete@last@row
%! m \@complete@vertical
%! m \complete@vertical
%! m \@complete@vspace
%! m \cont@frac@done
%! m \cont@frac@swap
%! m \co@ordinates
%! m \correct@for@width
%! m \crab@
%! m \cr@name
%! m \cross@names
%! m \cross@profile
%! m \cross@strut
%! m \@d
% m \d@brace
%! m \declared@at@cell
%! m \deepen@donations
%! m \default@args
%! m \default@diagonal
%! m \default@mapbreadth
%! m \default@max@fraction
%! m \default@profile
%! m \default@size
%! m \def@name
%! m \def@ps@turn
%! m \denominator@
%! m \diag@is@horiz
%! m \diag@is@vert
%! m \diagonal@box
%! m \@diagonals@used@false
%! m \@diagonals@used@true
%! m \@@@diagram
%! m \@@diagram
%! m \@diagram
%! m \diagram@cr
% m \diagram@help@messages
%! m \diagram@name
%! m \@di@dah
%! m \dim@in@pts
%! m \div@cclvi
%! m \div@dii
%! m \divide@
%! m \do@after@opt@arg
%! m \do@case
%! m \do@cont@frac
%! m \do@fated@enddiagram
%! m \dollar@name
%! m \do@message@at@end@doc
%! m \do@opt@arg
%! m \do@opt@arg@then
%! m \do@pile@row
%! m \do@set@dot@filler
%! m \dot@filler
%! m \double@LaTeX
% m \d@parenth
% m \eat@space
%! m \edef@name
%! m \eegroup
%! m \egroup@missing@label
%! m \egroup@name
%! m \@em
%! m \empty@filler
%! m \empty@name
%! m \empty@parts
%! m \end@at@line
%! m \end@cell
%! m \@enddiagram
%! m \@enddiagram@endpile
%! m \enddiagram@endpile
%! m \end@diagram@name
%! m \@end@diagram@ok@false
%! m \@end@diagram@ok@true
%! m \end@get@csname
%! m \@end@label
%! m \end@label
%! m \end@maths
%! m \end@mess
%! m \@end@pile
%! m \end@pile
%! m \end@square@name
% m \endswitch
%! m \exec@cross
%! m \exec@diagonal
%! m \execDiagonalLine
%! m \@exec@diagram
%! m \exec@diagram
%! m \exec@horiz
%! m \exec@LaTeX@diagonal
%! m \exec@map
%! m \exec@missive
%! m \exec@PS@diagonal
%! m \exec@vert
%! m \exit@diagram
%! m \expanded@ps@special
%! m \expanded@tpic@special
%! m \far@end@cell
%! m \fated@enddiagram
%! m \@filla
%! m \@fillb
% m \fill@dot % don't mangle as we \let@names{fill@dot}{}
%! m \@filler
% m \@fillh
% m \@fillv
%! m \finish@pile
%! m \first@occur
%! m \firstpass@showboxdepth
%! m \@first@positional@false
%! m \@first@positional@true
%! m \five@args
%! m \found@end@diagram
%! m \gdef@name
%! m \get@arg
%! m \@getcoords
%! m \get@csname
%! m \get@interrow@glue
%! m \@get@label
%! m \get@label
%! m \get@mand@value
%! m \@@getoptarg
%! m \get@opt@arg@list
%! m \get@opt@value
%! m \get@profile@info
% m \get@round@pair
% m \get@square@arg
%! m \glet
%! m \glet@names
% m \greaterthan
%! m \group@after@map
%! m \g@tmp
%! m \@h
%! m \handle@at
%! m \handle@at@
%! m \handle@matrix@row
% m \hbox@maths
%! m \@head
%! m \help@and
%! m \help@and@in@pile
%! m \help@bad@group
%! m \help@endlabel
%! m \help@hext
%! m \help@hpile
%! m \help@newarrow
%! m \help@pilecr
%! m \help@pile@enddiagram
%! m \help@undef@map
%! m \help@vext
%! m \help@vpile
% m \h@grid
%! m \horiz@add
%! m \horiz@extra
% m \horizhtdp
% m \Horizontal@Map
% m \Horizontal@Map
%! m \horizontal@name
%! m \horiz@repeater
%! m \horiz@state
%! m \@hug@false
%! m \@hug@true
%! m \if@adjust@flush@left@
%! m \if@cd@a@
%! m \if@cd@b@
%! m \if@cd@centre@display@
%! m \if@cd@centre@hlabel@
%! m \if@cd@centre@vlabel@
%! m \if@cd@g@
%! m \if@cd@hbox@
%! m \if@cd@landscape@
%! m \if@cd@leqno@
%! m \if@cd@missive@
%! m \if@cd@one@liner@
%! m \if@cd@PS@horiz@
%! m \if@cd@text@flow@
%! m \if@cd@through@
%! m \if@cd@tight@
%! m \if@cd@use@PS@
%! m \if@diagonals@used@
%! m \if@end@diagram@ok@
%! m \if@first@positional@
%! m \if@hug@
%! m \if@in@matrix@
%! m \if@need@PS@lib@
%! m \@@ifoptarg
%! m \@ifoptarg
%! m \if@reformatting@
%! m \if@use@TPIC@
%! m \if@was@pair@
% m \ignore@false
% m \ignore@true
% m \incommdiagfalse
% m \incommdiagtrue
%! m \info@at@end
%! m \@in@matrix@false
%! m \@in@matrix@true
%! m \inner@environment
%! m \inner@pile
%! m \intended@breadth
%! m \interim@shortfall
%! m \inter@row
%! m \iterate@
%! m \iterate@@
%! m \iterate@@@
%! m \@junk
%! m \@l
%! m \label@eat@space
%! m \label@egroup
%! m \label@egroups
%! m \label@horiz
%! m \label@optional
%! m \last@map@type
%! m \LaTeX@arrow@char
%! m \@@LaTeX@diagonal
%! m \LaTeX@dot@filler
%! m \LaTeX@line@char
%! m \LaTeX@make@line
%! m \LaTeX@name
%! m \LaTeX@NE
%! m \LaTeX@SW
% m \l@brace
%! m \left@donated
%! m \left@label
%! m \left@LaTeX@tail
%! m \left@over
%! m \left@part
%! m \left@width
% m \lessthan
%! m \let@names
%! m \lift@map@part
%! m \lift@map@parts
%! m \line@char
%! m \line@font
%! m \loop@on@cells
%! m \loop@on@maps
%! m \loop@on@rows
% m \lower@label
% m \l@parenth
% m \@m
%! m \make@diag@part
%! m \@make@double@head
%! m \make@double@head
%! m \@make@double@through@head
%! m \make@end@at@line
%! m \make@filler
%! m \make@found@end@diagram
%! m \make@horiz@part
%! m \make@line
%! m \makeline
%! m \make@old@fill
% m \make@pbk
%! m \make@profile
%! m \make@vert@part
%! m \math@off
%! m \math@off@box
%! m \math@on
%! m \math@on@box
%! m \maths@display
%! m \matrix@row@to@buffer
%! m \matrix@to@buffer
%! m \max@fraction
%! m \message@at@end@doc
%! m \@middle
% m \middle@label
%! m \min@map@length
%! m \misplaced@enddiagram
% m \missing@label
%! m \missive@diagonal
%! m \missive@outside
%! m \missive@to@cell
%! m \missive@to@row
%! m \mk@new@donat
%! m \modify@cell
%! m \monomial@
%! m \more@dim
%! m \more@donations
%! m \@morse
%! m \multiply@
%! m \multiply@@
% m \@name
%! m \name@prefix
%! m \need@extra
%! m \@need@PS@lib@false
%! m \@need@PS@lib@true
%! m \@new@arrow
%! m \newarrow@mmode
%! m \newarrow@name
%! m \new@arrow@part
%! m \new@diagonal
%! m \new@five@map
%! m \new@half@rpt@map
%! m \new@half@rule@map
%! m \new@help
%! m \new@horiz@map
%! m \new@if
%! m \new@line
%! m \new@map
%! m \new@rule@map
%! m \new@simple@map
%! m \new@slant@map
%! m \new@slope@map
%! m \new@thru@map
%! m \new@vector@map
%! m \new@vert@map
%! m \next
%! m \next@opt@arg
%! m \next@token
% m \no@cd@help
%! m \no@check@vert
%! m \no@error@context
%! m \nohcheck
%! m \no@make@line
%! m \@noptcmd
%! m \no@tenln
%! m \numerator@
% m \objectheight
%! m \object@profile
% m \objectwidth
%! m \obs@across
%! m \@obs@countq
%! m \obs@display
%! m \obs@positional
%! m \odef
%! m \old@horiz@fill
%! m \old@horiz@map
%! m \old@horiz@part
%! m \old@vert@fill
%! m \old@vert@map
%! m \one@sp
%! m \@optcmd
% m \optional@
% m \@outer@active
%! m \outer@empty
%! m \outer@environment
%! m \output@cell
%! m \output@diagram
%! m \outside@diagram
%! m \over@print
%! m \overprint@pbk
%! m \@p
%! m \pair@diagram@end
%! m \@par@enddiagram
%! m \par@enddiagram
% m \@parenth
%! m \par@name
%! m \par@not@allowed
%! m \@parse@opt@arg
%! m \parse@opt@arg
%! m \@parse@pair
%! m \pbk@osh
%! m \pbk@sh
%! m \pbk@shsh
%! m \pending@left
%! m \pending@right
%! m \@pile
%! m \pile@cr
%! m \pile@empty@row
%! m \pile@junk
%! m \pile@state
%! m \pixel@round
%! m \pixel@size
%! m \polar@to@rect
% m \positional@
%! m \PositiveGradientfalse
%! m \PositiveGradienttrue
%! m \ps@prog
%! m \push@queue
%! m \push@stack
%! m \put@cd@box
%! m \put@horiz
%! m \pyth@add@term
%! m \Pythagorean@sum
%! m \@pyth@sum
%! m \@r
% m \r@brace
%! m \reassign@filler
%! m \reassign@parts
%! m \receive@cell@type
%! m \reformat@cell
%! m \reformat@complex
%! m \reformat@empty
%! m \reformat@HmeetV
%! m \reformat@HonV
%! m \@reformat@horiz
%! m \reformat@horiz
%! m \reformat@matrix
%! m \reformat@object
%! m \reformat@pile
%! m \reformat@row
%! m \@reformatting@false
%! m \@reformatting@true
%! m \reformat@vert
%! m \reformat@VonH
%! m \reoutput@cell
%! m \resend@missive
%! m \reset@map@breadth
%! m \right@donated
%! m \right@label
%! m \right@LaTeX@tail
%! m \right@over
%! m \right@part
%! m \right@width
%! m \Rotated@Horizontal
%! m \rounded@breadth
%! m \row@depth
%! m \row@height
%! m \row@to@buffer
% m \r@parenth
% m \@rTo
%! m \rule@depth
%! m \rule@height
%! m \save@begin@at@line
%! m \save@cell@at@line
%! m \save@row@no
% m \@scriptaxis
% m \@scriptaxis
% m \script@axisheight
%! m \see@above
%! m \send@cell@type
%! m \separate@verticals
%! m \set@arrowhead
%! m \set@axis
%! m \set@cmex@axis
%! m \set@cmex@offset@axis
%! m \set@col@width
%! m \set@currentlabel
%! m \set@currentlabel@to@equation
%! m \@set@default@part
%! m \set@default@part
%! m \set@default@parts
%! m \set@dot@filler
%! m \set@fraction
%! m \set@h@grid
%! m \set@map@parts
%! m \set@max@fraction
%! m \set@mil
%! m \set@new@display
%! m \set@offset@axis
%! m \set@resolution
%! m \set@resultion
%! m \@setup@horiz
%! m \setup@pile
%! m \set@v@grid
%! m \showboxname
%! m \showname
%! m \show@prevgraf
%! m \showthename
%! m \@signature
%! m \signature@countdown
%! m \size@dependencies
%! m \skip@case
% m \Slant@Map
% m \Slant@Map
% m \Slope@Map
% m \Slope@Map
%! m \snake@
%! m \spAn
%! m \split@pile@row
%! m \square@fraction
% m \@ssaxis
% m \ss@axisheight
%! m \start@bomb@vlist
%! m \stretch@PS@diagonal
%! m \stretch@vert
%! m \@sub
% m \@super
% m \@super
% m \switch@arg
%! m \switch@label@arg
%! m \@szdep
%! m \@tail
%! m \test@loose@diagonals
%! m \test@signature
%! m \the@bomb
%! m \the@default@head
%! m \then
%! m \the@signature
%! m \this@map@type
% m \tmp
%! m \total@donated
% m \to@z
%! m \tpic@make@line
%! m \@u
% m \u@brace
%! m \unbraced@label
% m \undefined
% m \u@parenth
% m \upper@label
% m \Use@line@char
% m \Use@line@char
%! m \use@line@char
%! m \use@name
%! m \use@newarrow
%! m \@use@TPIC@false
%! m \@use@TPIC@true
%! m \using@ps
%! m \@v
%! m \@value
% m \Vector@Map
% m \Vector@Map
%! m \@vector@setup
%! m \verbatim@ps@special
%! m \vert@extra
% m \Vertical@Map
% m \Vertical@Map
%! m \vertical@name
%! m \vert@outside
%! m \vert@repeater
%! m \vert@wd@in@leftmost
% m \v@grid
%! m \@VonH
%! m \@was@pair@false
%! m \@was@pair@true
%! m \widen@hbox
%! m \widen@horiz
%! m \widen@pile
%! m \word@shrink
%! m \word@stretch
% m \@x % don't mangle as we \let@names{@x}{}
%! m \x@coord
%! m \xlc@ii
%! m \xlc@iv
%! m \x@offset
%! m \y@coord
%! m \y@offset

%! m \@pdf@false
%! m \@pdf@true
%! m \denom@@
%! m \div@@
%! m \do@eturn
%! m \if@pdf@
%! m \make@division
%! m \mk@@div
%! m \mnum@@
%! m \num@@
%! m \rotate@box@z
%! m \use@ps
%! m \dont@use@ps
%! m \use@pdf
%! m \undefined
%! m \cd@nonoPS
%! m \test@pdf
%! m \pdf@literal

%% don't load me twice!
% 19.9.2008 Terrence Bisson <bisson@canisius.edu>
% \undefined had been mangled to \CD@qK
% but in plain TeX, @=other, so got "@qK" in the output.
\ifx\diagram\isundefined\else\message
  {WARNING: the \string\diagram\space command is already defined and
  will not be loaded again}%
  \expandafter\endinput\fi

%% make @ letter, saving its old code to restore at the end of this file
%% look for this on the last line of the file if you think something's missing!
%% the other \catcode assignments are to make it work with texinfo.
\edef\cdrestoreat{%%
\noexpand\catcode`\noexpand\@=\the\catcode`\@%%
\noexpand\catcode`\noexpand\#=\the\catcode`\#%%
\noexpand\catcode`\noexpand\$=\the\catcode`\$%%
\noexpand\catcode`\noexpand\<=\the\catcode`\<%%
\noexpand\catcode`\noexpand\>=\the\catcode`\>%%
\noexpand\catcode`\noexpand\:=\the\catcode`\:%% Johannes L. Braams's
\noexpand\catcode`\noexpand\;=\the\catcode`\;%% Babel languages package
\noexpand\catcode`\noexpand\!=\the\catcode`\!%% makes these \active.
\noexpand\catcode`\noexpand\?=\the\catcode`\?%%
\noexpand\catcode`\noexpand\+=\the\catcode'53%% texinfo @+ is @outer@active
}\catcode`\@=11
\catcode`\#=6 \catcode`\<=12 \catcode`\>=12 \catcode'53=12
\catcode`\:=12 \catcode`\;=12 \catcode`\!=12 \catcode`\?=12

%% Change y to n if pool_size in your implementation of TeX is small.
%% This is reasonable if you have a small ("personal") computer, but if you
%% have a sun, dec, hp, ... workstation or a mainframe, complain to your local
%% system manager and get him/her to install a version of TeX with bigger
%% parameters. The "hash size" (number of command names) gets you next.
\ifx\diagram@help@messages\undefined\let\diagram@help@messages y\fi

%% The following macro is used to include literal PostScript commands in the
%% DVI file for rotation, etc.  Since this goes beyond standard TeX, it is
%% dependent on the convention used by your local DVI-to-PostScript translator.
%% Choose whichever line applies to the program used at your site, or, if
%% yours is not listed, consult the manual, experiment with this macro and
%% (please) tell me what is needed to make it work.
%%
%%
%% dvips (Tomas Rokicki, Radical Eye) labrea.stanford.edu /pub/dvips9999.tar.Z
%% CTAN: dviware/dvips
\def\cdps@Rokicki#1{\special{ps:#1}}%
\let\cdps@dvips\cdps@Rokicki
\let\cdps@RadicalEye\cdps@Rokicki\let\cdps@\cdps@Rokicki
\let\verbatim@ps@special\cdps@Rokicki\let\cdps@\cdps@Rokicki
%%
%% I'm not sure that the rest work.
%%
%% dvitps (Stephan Bechtolsheim, Integrated Computer Systems)
%% arthur.cs.purdue.edu /pub/TeXPS-9.99.tar.Z
\def\cdps@Bechtolsheim#1{\special{dvitps: Literal "#1"}}%% ASCII two dbl quotes
\let\cdps@dvitps\cdps@Bechtolsheim
\let\cdps@IntegratedComputerSystems\cdps@Bechtolsheim
%%
%% dvitops (James Clark)
%% CTAN: dviware/dvitops
\def\cdps@Clark#1{\special{dvitops: inline #1}}%%
\let\cdps@dvitops\cdps@Clark
%%
%% OzTeX (Andrew Trevorrow) cannot be used
\let\cdps@OzTeX\empty\let\cdps@oztex\empty\let\cdps@Trevorrow\empty
%%
%% dvi3ps (Kevin Coombes)
%% CTAN: dviware/dvi2ps/dvi3ps
\def\cdps@Coombes#1{\special{ps-string #1}}%
%\let@names{cdps@dvi3ps}{cdps@Coombes}%
%%
%% psprint (Trevorrow) CTAN: dviware/psprint
%% dvi2ps (Senn) CTAN: dviware/dvi2ps
%% psdvi (Elwell) CTAN: dviware/dvi2ps/psdvi

% there's also an expiry (and \endinput) message further down
\count@=\year\multiply\count@12 \advance\count@\month%%
\ifnum\count@>24300 %% (December 2024)
  \message{***********************************************************}%%ascii
  \message{! YOU HAVE AN OUT OF DATE VERSION OF COMMUTATIVE DIAGRAMS! *}%%
  \message{! it expired in December 2024 and is time-bombed for April *}%%
  \message{! You may get an up to date version of this package from *}%%ascii
  \message{! either www.ctan.org or www.PaulTaylor.EU/diagrams/ *}%%
  \message{***********************************************************}%%ascii
  \ifnum\count@>24303 %% (March 2025)
  \errhelp{You may press RETURN and carry on for the time being.}%
  \message{! It is embarrassing to see papers in conference proceedings}%
  \message{! and journals containing bugs which I had fixed years before.}%
  \message{! It is easy to obtain and install a new version, which will}%
  \errmessage{! remain compatible with your files. Please get it NOW.}%
\fi\fi

\def\glet{\global\let}\def\odef{\outer\def}%
% \let\@let\let\let\@edef\edef\let\@def\def
% \def\glet{\global\@let}%
% \def\odef{\outer\@def}%
% \@def\make@show@define#1{\expandafter\@let\csname\string#1\endcsname#1%
%       \@edef#1##1{\noexpand\message{\string#1\noexpand\string##1^^J}%
%               \csname\string#1\endcsname##1}}%
% \make@show@define\glet\make@show@define\let\make@show@define\def
% \make@show@define\gdef\make@show@define\edef\make@show@define\xdef
% \make@show@define\odef

%% safe names for braces, tab (&) and maths ($), as commands and for messages
{\escapechar\m@ne\xdef\bgroup@name{\string\{}\xdef\egroup@name{\string\}}%%
%%
%% three ASCII ampersands (ands) (&&&) appear on the next line
\catcode`\&=4 \glet\@and=&\xdef\and@name{\string\&}%%ascii three ands
%%
%% ASCII ^ and _ each appear twice on next line
%% six ASCII dollars ($$$$$$) appear on the next two lines.
\catcode`\$=3 \glet\begin@maths=$\glet\end@maths=$%%ascii three dollars
\xdef\dollar@name{\string\$}\gdef\maths@display{$$}%%ascii three dollars
%%
%% two ASCII underlines (__) appear on the next line.
\catcode`\_=8 \glet\@sub=_%%ascii two underlines
%%
%% eight ASCII carets (^^^^^^^^) appear on the next three lines.
\obeylines\catcode`\^=7 \glet\@super=^%%ascii two carets
\ifnum  \newlinechar=10 \gdef\new@line{^^J}%%ascii two carets
\else   \ifnum\newlinechar=13 \gdef\new@line{^^M}%%ascii two carets
\else   \ifnum\newlinechar=-1 \gdef\new@line{^^J}%%ascii two carets
\else   \glet\new@line\space
        \expandafter\message{! input error: \noexpand%ascii
        \newlinechar\space is ASCII \the\newlinechar, not LF=10 or CR=13.}%%
\fi\fi\fi}%%

%% avoid using <> (because I personally re-define them to mean \langle\rangle)
\mathchardef\lessthan='30474 \mathchardef\greaterthan='30476 

%% LaTeX line and arrowhead font
%% the "hit return" comments show up if the font is missing.
% size option?
\ifx\tenln\undefined%%
        \font\tenln=line10\relax%% Hit return - who needs diagonals?
\fi
\ifx\tenlnw\undefined
        \ifx\tenln\nullfont
                \let\tenlnw\nullfont
        \else%%
                \font\tenlnw=linew10\relax%% Hit return - who needs diagonals?
\fi     \fi%%

%% report line numbers in TeX3 only
% \newcount is \outer so cannot appear in skipped or definition text.
\ifx\inputlineno\undefined
        \csname newcount\endcsname\inputlineno\inputlineno\m@ne
        \message{***************************************************}%
        \message{! Obsolete TeX (version 2). You should upgrade to *}%
        \message{! version 3, which has been available since 1990. *}%
        \message{***************************************************}%
\fi

\def\cd@shouldnt#1{\cd@refmt@error{* THIS (#1) SHOULD NEVER HAPPEN! *}}%ascii

%% turn round- and square-bracketed arguments into curly-bracketed
\def\get@round@pair#1(#2,#3){#1{#2}{#3}}%%ascii round brackets ()
\def\get@square@arg#1[#2]{#1{#2}}%%ascii square brackets []
\def\get@opt@arg@list#1{%
    \@was@pair@false
    \let\next@opt@arg\@@getoptarg
    \@@getoptarg#1,],}%%ascii sq brackets
\def\begin@square@name{[}\def\end@square@name{]}%ascii
\def\commdiag#1{{\let\enddiagram\relax\diagram[]#1\enddiagram}}%ascii

%% ASCII open square bracket occurs on next line
\def\@@ifoptarg{{\ifx\next@token[%]%ascii
        \aftergroup\get@square@arg\aftergroup\@optcmd
\else
        \aftergroup\@noptcmd
\fi}}%%
% switch on presence of optional argument:
%   \@ifoptarg{\y}{\n}[arg]     does \y{arg}
%   \@ifoptarg{\y}{\n}          does \n
% are the braces actually necessary to avoid &?
\def\@ifoptarg#1#2{\def\@optcmd{#1}\def\@noptcmd{#2}%
\futurelet\next@token\@@ifoptarg}%

%% ASCII vertical bar (|) occurs on the next line
\def\vertical@name{|}%ascii

% idea: test & separately
% idea: use \meaning
% 14.5.92 DON'T GET & - GET \end@cell ANYWAY!
\def\cd@switch@arg{%% arguments to maps inside diagrams
\tokcase\end@cell:\@cd@a@false% no text between tip and &
                \break@args  ;%
\catcase\@super:\upper@label ;% superscript
\catcase  \@sub:\lower@label ;% subscript
\tokcase    {~}:\middle@label;%%ascii tilde
\tokcase      <:\left@label  ;%%ascii less-than
\tokcase      >:\right@label ;%%ascii greater-than
\tokcase      (:\co@ordinates;%%)%ascii open round bracket
\tokcase      [:\optional@   ;%%]%ascii open square bracket
\tokcase      .:\set@dot@filler;%%ascii dot 12.7.94
\catcase \space:\eat@space   ;% space (ignore)
\catcase\bgroup:\positional@ ;% obsolete positional labels
\default       :\@cd@a@true   % extra text between tip and &
                \break@args  ;% (anything else terminates labels)
\endswitch}

% Since maps are never bombed outside diagrams, glue compensation works
% and we don't have to abort through maps.
\def\switch@arg{%% arguments to horizontal maps outside diagrams
\catcase\@super:\upper@label ;% superscript
\catcase \@sub:\lower@label ;% subscript
\tokcase     [:\optional@   ;%%]%ascii open square bracket
\tokcase     .:\set@dot@filler;%%ascii dot 12.7.94 % ; was : before 15.6.97
\catcase\space:\eat@space   ;% space (ignore)
\catcase\bgroup:\positional@;% obsolete positional labels
\tokcase   {~}:\middle@label;%%ascii tilde (questionable!)
\default      :\@cd@a@false  % no need to allow for extra text
               \break@args  ;% (anything else terminates labels)
\endswitch}

%% That's as much as you get to read "in clear" - the rest is private!

%************************ program constructs *******************
%
\let\then\relax % makes \if...\then...\else...\fi more readable
\ifx\protect\undefined\let\protect\relax\fi
%
\ifx\AtEndDocument\undefined
   \def\message@at@end@doc{\cd@warning}%
   \def\info@at@end#1#2{}%
%
\else  % messages to output at the end of the run (28.7.95)
   \def\message@at@end@doc#1{%
      \edef\next{#1}%
      \expandafter\do@message@at@end@doc\next\end@mess}%
   \def\do@message@at@end@doc#1\end@mess{%
      \AtEndDocument{\typeout{\cd@name: #1}}}%
   \def\info@at@end#1#2{\gdef#1{#2}\AtEndDocument{#1}}%
\fi
% make warning to be given at first use only
\def\cd@first@use#1#2{%
   \def#1{\message@at@end@doc{#2\first@occur\at@line}%
   \glet#1\relax}}%
%
% TeX does not provide for nested loops in same scope!
% Warning: the \relax is needed in case the last command in the body reads
% ahead, for example "\advance\count@ 1".
%
% Why can't you put conditionals inside loops? Try with \toks.
%
\def\loop@on@rows#1\repeat{\def\body@{#1}\iterate@}%
\def\iterate@{\body@\relax\expandafter\iterate@\fi}%
\def\loop@on@cells#1\repeat{\def\body@@{#1}\iterate@@}%
\def\iterate@@{\body@@\relax\expandafter\iterate@@\fi}%
\def\loop@on@maps#1\repeat{\def\body@@@{#1}\iterate@@@}%
\def\iterate@@@{\body@@@\relax\expandafter\iterate@@@\fi}%
%
% as \newif, but simpler and manglable; initialised to false
\def\new@if#1#2#3{\def#2{\let#1\iftrue}\def#3{\let#1\iffalse}#3}%
%
% as \newhelp, but with a suppression option
\if y\diagram@help@messages
        \def\new@help#1#2{%
                \csname newtoks\endcsname#1%
                #1=\expandafter{%
                % I wanted to avoid the \ but it doesnt work
                %\expandafter\escapechar\expandafter\m@ne\expandafter\string
                \csname#2\endcsname}}%
\else
        \csname newtoks\endcsname\no@cd@help
        \no@cd@help{See the manual}%
        \def\new@help#1#2{\let#1\no@cd@help}%
\fi
%
% box definitions used during reformatting
\chardef\left@part=1
\chardef\right@part=2
\chardef\object@profile=5
\chardef\pending@right=6
\chardef\pending@left=7
\chardef\default@profile=9
\dimendef\right@donated=2
\dimendef\left@donated=3
\dimendef\left@width=4
\dimendef\right@width=5
\dimendef\total@donated=6
\dimendef\rule@height=8
\dimendef\rule@depth=9
\skipdef\completed@depth=1
\skipdef\inter@row=2
\skipdef\column@placing=3
\skipdef\horiz@extra=4
\skipdef\vert@extra=5
\skipdef\right@over=6
\skipdef\left@over=7
\skipdef\row@height=8
\skipdef\row@depth=9
\countdef\declared@at@cell=9
\countdef\far@end@cell=8
\countdef\across@cells=7
%
\def\sdef#1#2{\def#1{#2}}%
\def\after@name#1{\expandafter\aftergroup\csname #1\endcsname}%
\def\def@name#1{\expandafter\def\csname #1\endcsname}%
\def\gdef@name#1{\expandafter\gdef\csname #1\endcsname}%
\def\edef@name#1{\expandafter\edef\csname #1\endcsname}%
\def\let@names#1#2{\expandafter\let\csname#1\expandafter\endcsname
\csname#2\endcsname}%
\def\glet@names#1#2{\expandafter\glet\csname#1\expandafter
\endcsname\csname#2\endcsname}%
\def\use@name#1{\csname #1\endcsname}%
\def\showname#1{\expandafter\show\csname #1\endcsname}%
\def\showthename#1{\expandafter\showthe\csname #1\endcsname}%
\def\showboxname#1{\expandafter\showbox\csname #1\endcsname}%
%
\def\cd@name{Commutative Diagram}%
\edef\par@name{\string\par}%
\edef\diagram@name{\string\diagram}%
\edef\end@diagram@name{\string\enddiagram}%
\edef\cr@name{\string\\}%
\def\LaTeX@name{LaTeX}%
%
% LaTeX's switch to do \ignorespaces after an environment
% 11.10.97 inserted \global because LaTeX2e has changed the
% point at which \if@ignore\@ignorefalse\ignorespace\fi
% is executed. (Reported by Arthus Ogus ogus@math.berkeley.edu).
\ifx\@ignoretrue\undefined
    \expandafter\new@if\csname if@ignore\endcsname\ignore@true\ignore@false
    \def\@ignoretrue{\global\ignore@true}%
    \def\@ignorefalse{\global\ignore@false}%
\fi

%
%***************** aside on brace hacking (TeXbook p385) *****************
\def\bbgroup{{\ifnum0=`}\fi}\def\eegroup{\ifnum0=`{\fi}}%
% This is from latex.tex; it does \noalign{\hrule}, but if the next token
% is another \hrule it does \noalign{\hrule\vskip\hrule}.
% The reason why brace-backing is needed is that \ifx\@tempa\hline might
% encounter an & or \cr or \omit or \span. Our version of the same doesn't
% need this; it gets round it by putting the \ifx in braces.
% \def\hline{\noalign{\ifnum0=`}\fi\hrule \@height \arrayrulewidth \futurelet
%   \@tempa\@xhline}
%\def\@xhline{\ifx\@tempa\hline\vskip \doublerulesep\fi
%      \ifnum0=`{\fi}}
% there are other more complex examples for \\ commands for arrays, tables,
% etc. They need brace-hacking to protect \@ifstar - ie for the same reason.
%************************************************************************
% \hbox and \halign need {} or \bgroup\egroup, not \begingroup\endgroup
%************************************************************************
% 
%
% % % **** implement a case-switch construct ****
% % % Note that to protect & and \cr from recognition
% % % we have to em-brace them - \begingroup\endgroup doesn't work.
% % % This is probably the cause of the empty \mathord{} items.
% % % Also tried \def\catcase#1{\expandafter\eat@one{...}}\def\eat@one#1{}.
% % \def\catcase#1:{{%
% % \ifcat      \noexpand\next@token#1%
% % \then       \aftergroup\do@case
% % \else       \aftergroup\skip@case
% % \fi}}%
% % \def\tokcase#1:{{%
% % \ifx        \next@token#1%
% % \then       \aftergroup\do@case
% % \else       \aftergroup\skip@case
% % \fi}}%
% We never got & as \next@token anyway! The \mathord{}s have gone!
\def\catcase#1:{%
\ifcat  \noexpand\next@token#1%
\then   \expandafter\do@case
\else   \expandafter\skip@case
\fi}%
\def\tokcase#1:{%
\ifx    \next@token#1%
\then   \expandafter\do@case
\else   \expandafter\skip@case
\fi}%
\def\do@case#1;#2\endswitch{#1}%
\def\skip@case#1;{}%
\let\endswitch\relax
\def\default:#1;#2\endswitch{#1}% must come last
%
%idea
% \checklist<list><token>
% \def\checklist#1\expand\thenexttoken#2\endlist{%
% \def\rest{##2}%
% \ifx\rest\empty
% \then <not in list>
% \else <is in list>
% \fi}
%
% my initials in Morse code
%\def\@di@dah{\begin@maths{\cdot}{-}{\cdot}\;\;{-}\end@maths}%
%\def@name{rt:dah}{\rlap{\@di@dah}}%
%
%\edef\x{\meaning\year}\edef\y{\string\year} agree
%
% ***************** amstex emulation ***************
%
\ifx\at@\undefined\def\at@{@}\fi% amstex handling of @ defaults to letter
%\edef\amstex@prefix{pt@amstex@at@}%
\edef\amstex@prefix{\bgroup@name pt\egroup@name}%
\def@name{\amstex@prefix>}#1>#2>{\cd@and\rTo\sp{#1}\sb{#2}\cd@and}% horizontals
\def@name{\amstex@prefix<}#1<#2<{\cd@and\lTo\sp{#1}\sb{#2}\cd@and}%
\def@name{\amstex@prefix)}#1)#2){\cd@and\rTo\sp{#1}\sb{#2}\cd@and}%%ascii round
\def@name{\amstex@prefix(}#1(#2({\cd@and\lTo\sp{#1}\sb{#2}\cd@and}%%ascii brack
%
\def\amstex@diagram@setup{%
  \def\endCD{\enddiagram}%
  \def@name{\amstex@prefix A}##1A##2A{\uTo<{##1}>{##2}\cd@and\cd@and}%
  \def@name{\amstex@prefix V}##1V##2V{\dTo<{##1}>{##2}\cd@and\cd@and}%
  \def@name{\amstex@prefix=}{\cd@and\hEq\cd@and}%
  \def@name{\amstex@prefix\vertical@name}{\vEq\cd@and\cd@and}%
  \def@name{\amstex@prefix\string\vert}{\vEq\cd@and\cd@and}%
  \def@name{\amstex@prefix.}{\cd@and\cd@and}%
  \let\cd@and\@and
}%
%
\def\handle@at{%
   \let\tmp\handle@at@
   \ifcat     A\noexpand\next\else
   \ifcat     =\noexpand\next\else
   \ifcat\relax\noexpand\next\else
   \let\tmp\at@\fi\fi\fi
   \tmp}%
\def\handle@at@#1{\let@names{tmp}{\amstex@prefix\string#1}%
     \ifx\tmp\relax\def\tmp{\at@#1}\fi\tmp}%
%
\def\cd@and{}%
%
                                \begingroup\aftergroup
\def                            \aftergroup
    \assign@at                  \aftergroup
              {%
                                \aftergroup
               \def             \catcode`\@\active\aftergroup
                   @%
                                \endgroup
{\futurelet\next\handle@at}}%
%
%=======================================================================%
%                                                                       %
%       (2) DIMENSIONS AND COUNTS                                       %
%                                                                       %
%=======================================================================%
%
% define some scratch variables for our own use
% "gh" means global - use others and box/dimen 0...9 locally only
\newcount\cd@num@a\newcount\cd@num@b\newcount\cd@num@c\newcount\cd@num@d
\newdimen\cd@dim@a\newdimen\cd@dim@b
\new@if\if@cd@a@\@cd@a@true\@cd@a@false
\new@if\if@cd@b@\@cd@b@true\@cd@b@false
\newdimen\cd@dim@h\newdimen\cd@dim@k
\newcount\cd@num@g\newcount\cd@num@h
\newdimen\cd@dim@g\newbox\cd@box@g
\new@if\if@cd@g@\@cd@g@true\@cd@g@false
\newcount\numerator@\newcount\denominator@
%
% make #1 at least (resp at most) #2
\def\at@least#1#2{\ifdim#1<#2\relax#1=#2\relax\fi}%
\def\at@most #1#2{\ifdim#1>#2\relax#1=#2\relax\fi}%
%
\newdimen\one@sp\one@sp=1sp
\newdimen\@em\@em\z@
%
% check whether \@em has changed
% it was initialised to zero, and if "1em" is still zero
% that means there is no font loaded.
\def\size@dependencies{\ifdim\@em=1em\else\@szdep\fi}%
%
% if so, reset default arrowhead and \mathon & \mathoff
\def\@szdep{%
     \@em1em%
     \def\default@mapbreadth{\fontdimen8\textfont3 }%
     \set@arrowhead\set@max@fraction
     %
     % Can't see how to get \mathoff on its own without \null,
     % as it disappears at line breaks.
     % ! Math formula deleted: Insufficient symbol fonts
     \setbox0=\vbox{\bomb@parameters
        \noindent\begin@maths\null\penalty-9993\null\end@maths\null\endgraf
        \setbox0=\lastbox\unskip\unpenalty\setbox1=\lastbox
        \global\setbox\math@off@box=\hbox
                {\unhbox0\unskip\unskip\unpenalty\setbox0=\lastbox}%
        \global\setbox\math@on@box=\hbox
                {\unhbox1\unskip\unpenalty\setbox1=\lastbox}}%
}%
%
%\def\to@z{to\z@}%
%
% anticipate the pixel positioning
\newdimen\pixel@size\pixel@size=1true in \divide\pixel@size 300
%
% round #1 (a dimension or number) to pixels
\def\pixel@round#1{%
   \multiply#1\tw@
   \advance#1\ifnum#1<\z@-\else+\fi\pixel@size
   \divide#1\tw@
   \divide#1\pixel@size
   \multiply#1\pixel@size
}%
%
\def\MapBreadth{\afterassignment\reset@map@breadth\intended@breadth}%
\newdimen\intended@breadth % of ruled lines
\newdimen\rounded@breadth  % \intended@breadth rounded to pixels
\def\reset@map@breadth{%
   \rounded@breadth\intended@breadth
   \at@least\pixel@size{4\one@sp}% make sure we can divide by it
   \at@most\pixel@size\p@       % pixel smaller than point
   \pixel@round\rounded@breadth
   \ifdim\intended@breadth>\z@\at@least\rounded@breadth\pixel@size\fi
   \size@dependencies}%
\def\set@resolution#1{%
   \get@mand@value\count@
   \pixel@size#1%
   \ifnum\count@>\z@\divide\pixel@size\count@\fi
   \reset@map@breadth\set@max@fraction}%
\def\set@max@fraction{% 6 April 1995
   \dimen@\default@size
   \count@\dimen@\divide\count@ 5\divide\count@\pixel@size
   \edef\default@max@fraction{\the\count@}%
   %\expandafter\message
   %{max fraction=\default@max@fraction=\the\dimen@/5x\the\pixel@size}%
   }%
%
% set up for rule centred on maths axis
\def\set@axis{\set@offset@axis\z@}%
\def\set@offset@axis#1{%
   \rule@height\axisheight
   \advance\rule@height#1\relax
   \advance\rule@height-.5\rounded@breadth
   \pixel@round\rule@height
   \rule@depth-\rule@height
   \advance\rule@height\intended@breadth
}%
%
% transverse and longitudinal offset for arrows
\newdimen\crab@\crab@\z@\newdimen\snake@\snake@\z@
%
% set up for rule used with cmex parts (on baseline) 17.7.94
\def\set@cmex@offset@axis#1{%
   \rule@depth#1\relax
   \rule@height\rule@depth
   \advance\rule@height\intended@breadth\relax
}%
%
\def\horizhtdp{height\rule@height depth\rule@depth}%
\def\axisheight{\fontdimen22\the\textfont\tw@}% maths axis from symbols family
\def\script@axisheight{\fontdimen22\the\scriptfont\tw@}% script axis ditto
\def\ss@axisheight{\fontdimen22\the\scriptscriptfont\tw@}% scriptscript axis
\def\default@mapbreadth{0.4pt}%
\def\word@stretch{\fontdimen3\textfont\z@}%
\def\word@shrink{\fontdimen3\textfont\z@}%
%
%
\newdimen\PileSpacing
\newdimen\cd@left@margin        \cd@left@margin\z@
%\newdimen\min@map@length
\def\min@map@length{\ifincommdiag 1.3em\else 2em\fi}%
\newdimen\cd@top@height
%
\def\CellSize{\afterassignment\cell@height@to@width\DiagramCellHeight}%
\newdimen\DiagramCellHeight     \DiagramCellHeight-\maxdimen
\newdimen\DiagramCellWidth      \DiagramCellWidth-\maxdimen
\def\cell@height@to@width{\DiagramCellWidth\DiagramCellHeight}%
%
\def\default@size{3em}%
%
\newdimen\MapShortFall
\def\MapsAbut{\MapShortFall\z@\objectheight\z@\objectwidth\z@}%
%
\newdimen\cd@hshift\cd@hshift\z@ % amount to shift object right in cell
%
% %% this is a mega-hack for extracting as text the value of a \dimen in points
% {\catcode`p=12 \catcode`0=12 \catcode`.=12 \catcode` t=12 
% \gdef\rem@z#1.0.#2,{#1}%
% \gdef\dim@sans@uni#1pt{\rem@z#1.0.,}}%
% \def\dim@in@pts#1{\expandafter\dim@sans@uni\the#1 }
%\def\axis@height@in@pts{\dim@in@pts\axisheight}%
%
%------------------------------------------------------------------------
% 25 Aug 2006: PS & PDF switches moved here
%
% test whether \ifUglyObsoleteDiagrams has been defined and set to \iftrue
%
%\showname{ifUglyObsoleteDiagrams}%
\new@if\if@cd@use@PS@\@cd@use@PS@true\@cd@use@PS@false
\expandafter
   \ifx\expandafter\iftrue\csname ifUglyObsoleteDiagrams\endcsname
        \@cd@use@PS@false
   \else\@cd@use@PS@true
   \fi
\let@names{ifUglyObsoleteDiagrams}{relax}%
\newif\ifUglyObsoleteDiagrams
\def\use@ps{\@cd@use@PS@true\UglyObsoleteDiagramsfalse}%
\def\dont@use@ps{\@cd@use@PS@false\UglyObsoleteDiagramstrue}%
\if@cd@use@PS@\use@ps\else\dont@use@ps\fi
%
%
% are we using PDF-TeX?
\new@if\if@pdf@\@pdf@true\@pdf@false\@pdf@false
% 
% On Fri, 11 Jul 2003, Volodymyr Lyubashenko wrote:
% it seems that version 2002/03/15 v3.89 is incompatible with
% latex commands like
%    \usepackage[dvips]{graphics}
% or \usepackage{color}
% which also uses package `graphics'. It mistakes latex for pdflatex.
% This is ... MiKTeX 2.2 (preloaded format=latex 2000.11.28)
% ! Missing number, treated as zero.
% ! Missing = inserted for \ifnum.
% ! Illegal unit of measure (pt inserted).
% -- so I tried testing for \pdfoutput=\relax
%
\def\test@pdf{%
 \ifx\pdfoutput\undefined\else
 \ifx\pdfoutput\relax\else
 \ifnum\pdfoutput>\z@\use@pdf
 \fi\fi\fi
}
\def\use@pdf{%
   \global\@pdf@true
   \global\@cd@use@PS@true
   \global\UglyObsoleteDiagramsfalse
   \global\let\better@use@ps\empty
   \global\let\dont@use@ps\relax
   \global\let\use@pdf\relax
   \global\let\test@pdf\relax
}%
%\def\pdf@literal#1{\message{pdf: literal #1}\special{pdf: literal #1}}%
\def\pdf@literal#1{\special{pdf: literal #1}}%
\ifx\pdfliteral\undefined\else
\ifx\pdfliteral\relax\else
\let\pdf@literal\pdfliteral
\fi\fi
%
% are we running under XeTeX?
\ifx\XeTeXrevision\undefined\else
   \ifx\XeTeXrevision\relax\else
       \ifdim\XeTeXrevision pt<.996pt
           \expandafter\message{! XeTeX version \XeTeXrevision\space
           does not support PDF literals, so diagonals will not work!}%
       \else
           \expandafter\message{RUNNING UNDER XETEX \XeTeXrevision}%
           \use@pdf
\fi\fi\fi
%
% are we running under pdftex? (this is repeated in the first diagram)
\test@pdf
%
%=======================================================================%
%                                                                       %
%       (2) MAKE ARROW PARTS                                            %
%                                                                       %
%=======================================================================%
%
% \newarrowhead{name}{right}{left}{down}{up}
%                #5     #6    #7    #8   #9
%
\def\newarrowhead  {\new@arrow@part h\make@horiz@part\make@vert@part>}%
\def\newarrowtail  {\new@arrow@part t\make@horiz@part\make@vert@part>}%
\def\newarrowmiddle{\new@arrow@part m\make@horiz@part\hbox@maths\empty}%
\def\newarrowfiller{\new@arrow@part f\horiz@repeater \vert@repeater -}%
%                                  #1   #2              #3          #4
% 12.7.94 removed \make@vert@part from vertical middle,
% because it was hiding the width of wide middles (eg transitors).
%
% idea: []-option to set something instead of #4
% idea: check whether #5 is already defined
\def\new@arrow@part#1#2#3#4#5#6#7#8#9{%
  \def@name{r#1:#5}{#2{#6}}%
  \def@name{l#1:#5}{#2{#7}}%
  \def@name{d#1:#5}{#3{#8}}%
  \def@name{u#1:#5}{#3{#9}}%
 \edef@name{-#1:#5}{\expandafter\noexpand\csname-#1:#4\endcsname
    \noexpand\default@diagonal}%
 \edef@name{+#1:#5}{\expandafter\noexpand\csname+#1:#4\endcsname
    \noexpand\default@diagonal}%
% \let@names{+#1:#5}{+#1:#4}%
% \let@names{-#1:#5}{-#1:#4}%
}%
\cd@first@use\default@diagonal{\LaTeX@name\space diagonals are used unless
    PostScript is set}%
%
% ****************** choose default components *****************
%
% 32 arrow parts in 16 boxes
\def\defaultarrowhead#1{\edef\the@default@head{#1}\set@arrowhead}%
\def\set@arrowhead{%
   \set@default@parts       \the@default@head <>ht%       single arrowheads
  %\set@default@parts{double\the@default@head}{<<}{>>}ht% double heads
   \set@default@parts       \the@default@head <>th%       single tails
  %\set@default@parts{double\the@default@head}{<<}{>>}th% double tails
}%
%
% 8 arrow parts in 4 boxes
\def\set@default@parts#1#2#3#4#5{% #1=choice #2=tailname #3=headname #4=h #5=t
  \set@default@part{r#4}{#3}{l#5}{#2}{r#4:#1}%
  \set@default@part{r#5}{#2}{l#4}{#3}{l#4:#1}%
  \set@default@part{d#4}{#3}{u#5}{#2}{d#4:#1}%
  \set@default@part{d#5}{#2}{u#4}{#3}{u#4:#1}%
}%
%
% do:   if \#1+:#2 is not defined then \newbox\#1+:#2 \fi
%       \def\#1:#2{\copy\#1::#2}
%       \def\#3:#4{\copy\#1::#2}
%       \setbox\#1::#2=\#5
%
\def\set@default@part#1#2#3#4#5{%
\begingroup
        %\expandafter\ifx\csname #1+:#2\endcsname\relax %ascii
        %       \after@name{newbox}\after@name{#1+:#2}%ascii
        %\fi
        \aftergroup\@set@default@part
\after@name{#1+:#2}\after@name{#1:#2}\after@name{#3:#4}\after@name{#5}%ascii
\endgroup}%
%
% use this code first to define the boxes and macros
\def\@set@default@part#1#2#3#4{% #1=boxname #2=partname #3=synonym #4=value
\csname newbox\endcsname#1%
\def#2{\copy#1}%
\def#3{\copy#1}%
\setbox#1=\box\voidb@x}%
%
\def\the@default@head{}%
\set@arrowhead% do it with empty boxes
%
% now re-define the macro so that it just sets the box
\def\@set@default@part#1#2#3#4{\setbox#1=#4}%
%
\ifx\tenln\nullfont
     \def\the@default@head{vee}%
\else\let\the@default@head\LaTeX@name
\fi
%
\def\make@double@head#1#2#3{%
\begingroup
   \aftergroup\@make@double@head\after@name{#1#2:#3#3}\after@name{#1#2:#3}%
   \aftergroup\@make@double@through@head\after@name{#1#2:#3-#3}\after@name{#1#2:#3}%
\endgroup}%
%
\def\@make@double@head#1#2{\def#1{\hbox{\rlap{#2}\kern.4\@em#2}}}%
\def\@make@double@through@head#1#2{%
    \def#1{\hbox{\rlap{#2}\kern.4\@em#2\kern-.4\@em}}}%
\make@double@head lh>%
\make@double@head rt>%
\make@double@head rh<%
\make@double@head rt<%
\def\@make@double@through@head#1#2{%
    \def#1{\hbox{\kern-.4\@em\rlap{#2}\kern.4\@em#2}}}%
\make@double@head rh>%
\make@double@head lh<%
\make@double@head lt>%
\make@double@head lt<%
%
\def\@make@double@head#1#2{%
\def#1{\vbox{\vbox to\z@{#2\vss}\nointerlineskip\kern.4\@em#2}}}%
\def\@make@double@through@head#1#2{%
\def#1{\vbox{\vbox to\z@{#2\vss}\nointerlineskip\kern.4\@em#2\kern-.4\@em}}}%
\make@double@head uh>%
\make@double@head dt>%
\make@double@head dh<%
\make@double@head dt<%
\def\@make@double@through@head#1#2{%
\def#1{\vbox{\kern-.4\@em\vbox to\z@{#2\vss}\nointerlineskip\kern.4\@em#2}}}%
\make@double@head dh>%
\make@double@head ut>%
\make@double@head uh<%
\make@double@head ut<%
%
% old version that did both together every time
% NB \csname undefined\endcsname=\relax LOCALLY - \aftergroup it's \undefined
%\def\@set@default@part#1#2#3#4{% #1=boxname #2=partname #3=synonym #4=value
%\ifx#1\undefined\csname newbox\endcsname#1\fi %if #1 is undefined \newbox#1 fi
%\def#2{\copy#1}\def#3{\copy#1}%
%\setbox#1=#4}%
%
%
% ******************* MAKE MAP PARTS ***********************
%
% idea: use \mathsurround
%
% Clip the margins off Computer Modern symbols.
\def\make@horiz@part#1{%
\hbox{\mathsurround\z@\offinterlineskip
        \begin@maths\mkern-1.5mu{#1}\mkern-1.5mu\end@maths
}}%
%
% Put vertical arrow part into a box, centering it.
% However since there's nothing we can do about the fact the
% reference point of \vrule width\intended@breadth is on the left,
% we make the other repeating boxes compatible with it,
% by centering them (smashed) in a box of the same width.
% 
\def\hbox@maths#1{\hbox{\begin@maths#1\end@maths}}%  17.7.94
\def\make@vert@part#1{\hbox to\intended@breadth{%
   \setbox0=\hbox{%
      \offinterlineskip
      \mathsurround\z@
      \begin@maths{#1}\end@maths % set the vertical arrow part
    }%
   \dimen0.5\wd0\advance\dimen0-.5\rounded@breadth
   \pixel@round{\dimen0}%
   \kern-\dimen0\unhbox0\hss}}%  
%
% version for use with cmex parts 17.7.94 
\def\cmex@vert@part#1{\hbox to2\intended@breadth{% don't understand "2"
   \hss
   \offinterlineskip
   \mathsurround\z@
   \begin@maths{#1}\end@maths % set the vertical arrow part
   \hss}}%  
%\def\cmex@vert@part#1{\hbox to\z@{\hss\begin@maths#1\end@maths\hss}}%
%
%\def\make@vert@part#1{%
%\hbox to\intended@breadth{% arrow-part: centered in 0 to \MapB
%\offinterlineskip\mathsurround\z@
%\hss\begin@maths%\kern\intended@breadth
%{#1}\end@maths\hss}}%
%\def\make@vert@part#1{%
%\hbox to\z@{% arrow-part
%\setbox0=\hbox{\offinterlineskip\mathsurround\z@\begin@maths{#1}\end@maths}%
%\count@\wd0\advance\count@-\intended@breadth\advance\count@\pixel@size
%\divide\count@2\divide\count@\pixel@size
%\dimen0\wd0\advance\dimen0.5\pixel@size\divide\dimen0\pixel@size
%\dimen1\intended@breadth\advance\dimen1.5\pixel@size\divide\dimen1\pixel@size
%\advance\dimen0-\dimen1\divide\dimen0 2\count@\dimen0%
%\kern-\count@\pixel@size\box0\hss}}%
%
\def\make@diag@part#1{\hbox{\mathsurround\z@\begin@maths{#1}\end@maths}}%
%
\def\horiz@repeater#1{\hbox{\kern-.15\@em\begin@maths{#1}\end@maths
        \kern-.15\@em}}%
%
\def\vert@repeater #1{%
  \vbox{\offinterlineskip
    \kern-.2ex%
    \make@vert@part{#1}%
    %\hbox to\intended@breadth{\hss\begin@maths{#1}\end@maths\hss}%
    \kern-.2ex}}%
%
% also dot filler
%
\def\@fillh{\xleaders\vrule\horizhtdp}% default rule filler
\def\@fillv{\xleaders\hrule width\intended@breadth}%
\let@names{rf:-}{@fillh}\let@names{lf:-}{@fillh}%
\let@names{df:-}{@fillv}\let@names{uf:-}{@fillv}%
%
% ****************** empty components *****************
%
% empty arrowhead and middle
\let@names{rh:}{null}\let@names{rm:}{null}\let@names{rt:}{null}%
\let@names{lh:}{null}\let@names{lm:}{null}\let@names{lt:}{null}%
\let@names{dh:}{null}\let@names{dm:}{null}\let@names{dt:}{null}%
\let@names{uh:}{null}\let@names{um:}{null}\let@names{ut:}{null}%
\let@names{+h:}{null}\let@names{+m:}{null}\let@names{+t:}{null}%
\let@names{-h:}{null}\let@names{-m:}{null}\let@names{-t:}{null}%
%
% empty filler (nontrivial size, to avoid division by zero in \xleaders)
% 17.7.94 changed from \def to \let
% 4.7.97 \empty@filler and \empty@parts
\def\empty@filler{\hbox{\vrule height 1pt depth-1pt width 1pt}}%
\def@name{rf:}{\empty@filler}\let@names{lf:}{rf:}\let@names{+f:}{rf:}%
\def@name{df:}{\empty@filler}\let@names{uf:}{df:}\let@names{-f:}{df:}%
\def\empty@parts{\assign@five\null\empty@filler\null\empty@filler\null}%
%
%
%=======================================================================%
%                                                                       %
%       (3) NEW ARROW                                                   %
%                                                                       %
%=======================================================================%
%
% define a family of arrow commands
% \newarrow{Name}{tail}{filler}{middle}{filler}{head}
%
% idea: \catcode`\\ to catch non-text names
% idea: \renewarrow etc, also synonyms & head/tail synonyms
% idea: optional argument to list directions, eg [r,l,d,u] or [nw,ne,sw,se]
%
\edef\newarrow@name{\string\newarrow}% do this now because it's \outer
%
% ******************* \newarrow *******************************
%
\def\newarrow#1#2#3#4#5#6{%
\begingroup
%               ----- components and defaults -----
%
  \edef\@name{#1}%
  \edef\@tail{#2}\edef\@filla{#3}%
  \edef\@middle{#4}\edef\@fillb{#5}\edef\@head{#6}%
  \let\@h\new@horiz@map
  \let\@v\new@vert@map
  \let\@x\new@vector@map   % LaTeX vector
%
%               ----- normalise the components -----
%
% if the tips are the same as the corresponding fillers
% make them empty instead
  \ifx\@tail\@filla\let\@tail\empty\fi
  \ifx\@head\@fillb\let\@head\empty\fi
%
% if the head is empty and the tail isn't (funny!), swap everything around
  \def\@r{r}\def\@l{l}\def\@d{d}\def\@u{u}\def\@p{+}\def\@m{-}%
%  \ifx\@head\empty\ifx\@tail\empty\else
%       \let\@r\@filla          % wrong way round, so switch components
%       \let\@filla\@fillb
%       \let\@fillb\@r
%       \let\@head\@tail        % \@head was \empty anyway
%       \let\@tail\empty
%       \def\@r{l}\def\@l{r}\def\@d{u}\def\@u{d}\def\@p{-}\def\@m{+}%
%  \fi\fi
%
  \ifx\@filla\@fillb
%
%                ----- same filler fore and aft -----
%
%    normalise middle to empty if also same
     \ifx\@middle\@filla\let\@middle\empty\fi
%
     \ifx\@head\empty
        \ifx\@filla\horizontal@name
           \let\@x\new@slant@map % LaTeX \line
        \else
           \let\@x\new@slope@map % unrestricted
     \fi\fi
%
  \else\edef\@back{\@filla\@tail}%
     \ifx\@back\empty
%
%                ----- half-length maps -----
%
         \ifx\@middle\@fillb\let\@middle\empty\fi % normalise middle if same
        %\let\@h\new@half@horiz
        %\let\@v\new@half@vert
  \fi\fi
%
%            ----- are the components actually there? -----
\ifmmode
  \aftergroup\newarrow@mmode
\else
  \@cd@a@true
  \check@part rh{head\space\space}\@head
  \check@part rf{filler}\@filla
  \check@part rm{middle}\@middle
  \ifx\@fillb\@filla\else
     \check@part rf{filler}\@fillb
  \fi
  \check@part rt{tail\space\space}\@tail
%
  \if@cd@a@
%
%             ----- yes - output the definitions -----
%
       \@h % make horizontals
       \@v % make verticals
       \@x % make diagonals
%
        \new@diagonal l-2+2{lu}{nw}\NorthWest   % \diagonal@setup
        \new@diagonal r+2+2{ru}{ne}\NorthEast
        \new@diagonal l-2-2{ld}{sw}\SouthWest
        \new@diagonal r+2-2{rd}{se}\SouthEast
  \else
%             ----- no - output an error message -----
%
        \aftergroup\bad@arrow\after@name{r\@name}%
\fi\fi
\endgroup % \aftergroup collects all the actual definitions here
}%
%
% ******************* \newarrow internals **************************
%
%
\def\new@horiz@map {\new@map\@r\@l rl\Horizontal@Map}%
\def\new@vert@map  {\new@map\@d\@u du\Vertical@Map}%
\def\new@vector@map{\new@map\@p\@m +-\Vector@Map}% LaTeX \vector
\def\new@slant@map {\new@map\@p\@m +-\Slant@Map}%  LaTeX \line
\def\new@slope@map {\new@map\@p\@m +-\Slope@Map}%  unrestricted
%\def\new@half@horiz{\new@half@map\@r r\setup@right@half
%                    \new@half@map\@l l\setup@left@half}%
%\def\new@half@vert {\new@half@map\@d d\setup@bottom@half
%                    \new@half@map\@u u\setup@top@half}%
%
%
%                ----- make one or two user arrow commands -----
%
\catcode`\/=\active %ascii            avoid clash in use of slash delimiter/
%
\def\new@map#1#2#3#4#5{%
\@new@arrow#1#3#5t:\@tail/f:\@filla/m:\@middle/f:\@fillb/h:\@head//%ascii
\@new@arrow#2#4#5h:\@head/f:\@fillb/m:\@middle/f:\@filla/t:\@tail//}%ascii
%
%\def\new@half@map#1#2#3{\@new@arrow#1#2#3m:\@middle/f:\@fillb/h:\@head//}%
%
% internals:
% #1=name prefix, #2=argument prefix, #3=direction command, #4=arguments
\def\@new@arrow#1#2#3#4//{%ascii                        slash is \active here/
\edef\name@prefix{#2}%
\aftergroup\sdef\after@name{#1\@name}\aftergroup{%
        \aftergroup#3%        % setup
        %\after@name{#1\@name}% give it its name (?)
        \after@names#4//%ascii% arguments                    slash is \active/
\aftergroup}}%
%
\def\after@names#1/{%ascii /-separated, //-terminated list   slash is \active/
\edef\next@token{#1}%
\ifx    \next@token\empty
\else   \after@name{\name@prefix#1}%
        \expandafter\after@names%
\fi}%
%
\catcode`\/=12 %ascii                                         restore slash/
%
%                   ----- make a user diagonal command -----
%
% #1=orthogonal direction to use for rotation
% (#2#3,#4#5) vectorial form of direction
% #6 #7 direction prefix for user command name
% #8 direction setup
% do: \def\#6name{\#2name \signGradient \#1name  (#3,#5)}
\def\new@diagonal#1#2#3#4#5#6#7#8{%
  \aftergroup\sdef\after@name{#6\@name}\aftergroup{% \def\#6name
        \after@name{#2\@name}%  diagonal map command eg \+To
        \if#2#4%
             \aftergroup\PositiveGradienttrue
        \else\aftergroup\PositiveGradientfalse
        \fi
        \after@name{#1\@name}%  orthogonal map to rotate eg \rTo
%% ASCII round brackets and comma (,) appear on the next line
        \aftergroup(\aftergroup#3\aftergroup,\aftergroup#5\aftergroup)%ascii
  \aftergroup}%
}%
%
% do: \def\#6name{\diag@setup #7 \#1name \#2name (#3,#5)}
%\def\new@diagonal#1#2#3#4#5#6#7#8{%
%  \aftergroup\sdef\after@name{#6\@name}\aftergroup{% \def\#6name
%       \if#2#4%
%            \aftergroup\Rising@Map
%       \else\aftergroup\Falling@Map
%       \fi
%       %\aftergroup\Diagonal@Map\aftergroup#7%   % \Diagonal@Map #7
%       \after@name{#1\@name}\after@name{#2\@name}% \#1name \#2name
% % ASCII round brackets and comma (,) appear on the next line
%       \aftergroup(\aftergroup#3\aftergroup,\aftergroup#5\aftergroup)%ascii
%  \aftergroup}%
%}%
%
%                    ----- existence of components -----
\def\check@part#1#2#3#4{%
\expandafter\ifx\csname #1#2:#4\endcsname\relax
        \@cd@a@false\cd@warning{arrow#3 "#4" undefined}%ascii
\fi}%
%
\new@help\help@undef@map{All five components must be defined before an arrow.}%
\new@help\help@newarrow{\newarrow@name, unlike \string\HorizontalMap, is a
declaration.}%
%
\def\bad@arrow#1{\cd@error{Arrows \string#1 etc could not be defined}%
\help@undef@map}%
%
\def\newarrow@mmode{\cd@error{misplaced \newarrow@name}\help@newarrow}%
%
%
%=======================================================================%
%                                                                       %
%       (3A) NEW GRID                                                   %
%                                                                       %
%=======================================================================%
%
\def\newdiagramgrid#1#2#3{%
    \def@name{cdgh@#1}{#2,],}%% ASCII close square bracket
    \def@name{cdgv@#1}{#3,],}}%% ASCII close square bracket
%
%=======================================================================%
%                                                                       %
%       (4) HORIZONTAL STATE CHECKING AND ARROW SETUP                   %
%                                                                       %
%=======================================================================%
%
% We use \cd@donat (during the first pass, locally to each cell) to hold a
% "horizontal map state".  Each map type inserts the missing text (giving an
% appropriate error message) shown for each state and changes to the new state.
%
% donated half maps?
%
%                  end of \rTo or                \VonH or
% state              cell   \pile    \dTo   \HonV \HmeetV
% 0 outside diagram     -   ($) 0  forbid  forbid  forbid
% 1 space donated       1       5       3       4       4
% 2 arrow donated       1   {}& 5       3       5       4
% 3 verticals   (in)    1     & 5       3     & 4     & 4
% 4 junction   (this)   1     & 5     & 3     & 4     & 4
% 5 horizontal (cell)   2  &{}& 5     & 3     & 4     & 4
% 6 pile              } 2       7    }& 3    }& 4    }& 4
% 7 pile horizontal   } 2    \\ 7    }& 3    }& 4    }& 4
%
% initial states outside diagram, inside diagram and inside \pile
% signal we're outside \commdiag
\new@if\ifincommdiag\incommdiagtrue\incommdiagfalse
\new@if\if@in@matrix@\@in@matrix@true\@in@matrix@false % 12.7.94
\newcount\cd@donat
\cd@donat=0
\def\pile@state{\cd@donat6 }%
% idea: check number of rows and columns
% assign to \cd@num@g in case the first cell is empty, so \end@cell
% (and hence \send@cell@type) is not called.
% changed to \empty (and initialised as such) from {left edge} 27.12.93
\def\cd@state{\cd@donat1 \global\cd@num@g1 \glet\last@map@type\empty}%
\def\last@map@type{}%
%
% The automaton for horizontal maps; also used by \pile.
% #1="horizontal map" or "pile".
\def\check@horiz#1{\relax
\end@label % in case of missing close brace at end of label
\edef\this@map@type{#1}%
\begingroup
\if@cd@PS@horiz@\else
\ifcase\cd@donat\ifmmode\else%  0% 0 in maths outside diagram ok
   \modify@cell\add@dollar 0\fi%0% 0 outside maths
\or\horiz@state                 5% 1 accept space donation ok
\or\modify@cell\add@empty@and   5% 2 empty object between two horizontals
\or\modify@cell\add@and         5% 3 new cell after vertical
\or\modify@cell\add@and         5% 4 new cell after junction
\or\modify@cell\add@and@and     5% 5 two horizontals (perhaps \pile intended?)
\or\horiz@state                 7% 6 in pile ok
\or\modify@cell\add@cr          7% 7 new row of pile after horizontal
\fi\fi\endgroup         % save up commands to here with \aftergroup
\xdef\last@map@type{#1}}%
%
% The automaton for verticals; also used by \HonV, \VonH and \HmeetV.
% #1=least state requiring insertion, #2=usual new state, #3=exceptional one,
% #4=map type text, #5=command (will do no-op with error in forbidden case).
\def\check@vert#1#2#3#4#5{\relax
\end@label % in case of missing close brace at end of label
\xdef\this@map@type{#4}%
\begingroup
\ifnum  \cd@donat<#1
        \expandafter\horiz@state\ifcase\cd@donat0\or#2\or#3\else#2\fi%
\else   \ifnum  \cd@donat<6
        \then   \modify@cell\add@and            #2%
        \else   \modify@cell\add@endpile@and    #2%
\fi     \fi
\endgroup               % \aftergroup saves up commands to do here
\glet\last@map@type\this@map@type
\ifincommdiag
        \let\exec@map#5%
\else   \let\exec@map\vert@outside
\fi}%
%
% idea: compare with a global variable to check for (wrongly) em-braced maps.
% idea: count no. of rows & columns to check for overflow
%
% Pass the new horizontal state across cell boundary using global variable;
% this is picked up and assigned to \cd@donat in the next template.
\def\send@cell@type{\global\cd@num@g=\ifnum\cd@donat<5 1\else2\fi\relax}%
\def\receive@cell@type{\cd@donat\cd@num@g}%
%
% Set the new state (after \endgroup).
\def\horiz@state#1{\aftergroup\cd@donat\aftergroup#1\aftergroup\relax}%
%
% skip the check ("time nlatex manual")
% with check: 24.7u 1.0s 0:31 83% 0+1568k 0+13io 0pf+0w
% without:    24.6u 0.9s 0:30 83% 0+1572k 0+13io 0pf+0w
\def\nohcheck{%
\def\check@horiz##1{\relax}%
\let\check@vert\no@check@vert
\let\pile@state\relax
\let\cd@state\relax
\let\send@cell@type\relax
\let\receive@cell@type\relax
}%
\def\no@check@vert#1#2#3#4#5{%
\ifincommdiag
        \let\exec@map#5%
\else   \xdef\this@map@type{#4}\let\exec@map\vert@outside
\fi}%
%
% Do insertion, with error message (then change state), after \endgroup.
% [Remember that insertion of & or \\ within #1 causes a lot of extra commands
%  like \begin@cell \end@cell to be executed.
%  We are careful to ensure that conditionals are completed with our own cell.
%  Note sure why, but it does at least mean that the user does not see \fi in
%  the error context.]
\def\modify@cell#1{\aftergroup#1\aftergroup\relax\horiz@state}%
%
% The insertion commands.
\def\add@and{\horiz@add\and@name\help@and\@and}%
\def\add@endpile@and{\horiz@add{\egroup@name\and@name}\help@vpile%
  \end@pile\@and}%
% How can we tell (in the next case) whether there is already an object in
% the cell, so it's just a & which is missing? Perhaps test whether \next@token
% is the first of \check@horiz? [\relax is too common for this]
\def\add@empty@and{\horiz@add{*\and@name}\help@hpile\clubsuit\@and}%ascii
\def\add@and@and{\horiz@add{\and@name*\and@name}\help@hpile\@and\clubsuit%ascii
 \@and}%
\def\add@cr{\horiz@add\cr@name\help@pilecr\\}%
\def\add@dollar{\horiz@add\dollar@name\help@hext\begin@maths}%
\def\vert@outside{\cd@error{\this@map@type\space ignored \outside@diagram}%
  \help@vext}%
%
% Within the $..$ of diagram & pile cells we assign \bad@group@after@map
% to \group@after@map, but make it \empty again in the diagram and pile
% environments. Then \aftergroup\group@after@map at the end of the arrow
% command (in \break@args) causes an error if the next end-of-group occurs
% strictly within the $; the $ itself is supposed to be the end-of-group.
\def\group@after@map{}%
\def\bad@group@after@map{\cd@error{maps must never be enclosed in braces}%
   \help@bad@group}%
%
% This version also complains if you do ${\rTo}$ in text.
%   \def\group@after@map{\ifmmode\expandafter\bad@group@after@map\fi}%
% but I had the following example in my book:
%   $$\denote{\Gamma\rTo^{[f:=\hat g]}(f:(\hat A\to\hat B))}= ... $$
% which seems a reasonable use of braces around arrows in text.
% The only effect is to prevent them stretching with the paragraph.
%
% Help messages
\def\outside@diagram{outside diagram}%
\def\cross@names{\string\HonV, \string\VonH\space and \string\HmeetV}%
\new@help\help@and{The way that horizontal and vertical arrows are terminated
  implicitly means\new@line that they cannot be mixed with each other or with
  \cross@names.}%
\new@help\help@vpile{\string\pile\space is for parallel horizontal arrows;
  verticals can just be put together in\new@line a cell. \cross@names\space
  are not meaningful in a \string\pile.}%
\new@help\help@hpile{The horizontal maps must point to an object, not each
  other (I've put in\new@line one which you're unlikely to want).
  Use \string\pile\space if you want them parallel.}%
\new@help\help@pilecr{Parallel horizontal arrows must be in separate layers
  of a \string\pile.}%
\new@help\help@hext{Horizontal arrows may be used \outside@diagram s, but must
  still be in maths.}%
\new@help\help@vext{Vertical arrows, \cross@names\space\outside@diagram s
  don't know where\new@line where to terminate.}%ascii
\new@help\help@bad@group{This prevents them from stretching correctly.}%
%
% The actual message.
% Before 27.12.93 this tested \ifincommdiag.
\def\horiz@add#1{\cd@error{"#1" inserted %ascii
\ifx\last@map@type\empty
        before  \this@map@type
\else   between \last@map@type
        \ifx    \last@map@type\this@map@type s%
        \else   \space and \this@map@type
        \fi
\fi}}%
%
\count@=\year\multiply\count@12 \advance\count@\month
\ifnum\count@>24307 \message{because this one expired in July 2025!}%
\expandafter\endinput\fi
%
%=======================================================================%
%                                                                       %
%       (5) SYNTAX OF ARROW COMMANDS                                    %
%                                                                       %
%=======================================================================%
%
%
% ************************* MAP SETUP ********************************
%
% The following are available when \exec@map is called, except:
% * indicates \set@map@parts does the assignment
%
% @cd@a@      = there's text between the last argument and the end of the cell
% @cd@through = whether \@filla and \@fillb agree
% \exec@map   = command to execute
% \dimen 1    = left or lower shortfall
% \@head      = leading tip (macro)
%*\box   1    = leading tip (set)
% \@filler    = default filler against which to test for rule
% \@filla     = leading filler: box or rule leaders (empty for right half map)
%*\box   2    = leading repeater, or void for rule
% \dimen 2    = minimum length of arrow (tip-to-tip)
% \skip  2    = glue for leading filler
% \box   3    = middle
% \cd@penalty = penalty code value
% \@fillb     = trailing (right or lower) filler
%*\box   4    = trailing repeater, or void if rule
% \skip  4    = glue for trailing filler
% \@tail      = trailing tip (macro)
%*\box   5    = trailing tip (set)
% \dimen 5    = right or upper shortfall
% \box   6    = leading label or void
% \box   7    = trailing label or void
%
% diagonals only:
% \x@coord    = number of cells through which to pass horizontally
% \DiagramCellWidth = width of current column
% \y@coord    = number of cells through which to pass vertically
% \DiagramCellHeight = height of current row
%
% \rTo ->  \Horizontal@Map \rt: \rf:- \rm: \rf:- \rh:>
% \five@args picks up the five components and calls \get@arg,
% which parses the labels and options and calls \exec@horiz
%
\def\Horizontal@Map{%
\check@horiz{horizontal map}%   % avoid clashes
\default@args\@setup@horiz      % default parameters
%\let\fill@dot\hfdot % 12.7.94; moved to \@setup@horiz 28.7.95
\five@args}%
%
\def\@setup@horiz{%
\cd@penalty-9999                % \penalty code for default horizontal
\let\exec@map\exec@horiz        % continuation for \get@arg
\ifincommdiag
%       \baselineskip 1.4ex     % for positioning of labels in diagrams
%       \lineskip      .3ex
%       \lineskiplimit .3ex
\else   \size@dependencies
%       \dimen2=\min@map@length% min tip-to-tip arrow len 15.4.95
%       \baselineskip  .6ex     % much closer in text
%       \lineskip      .2ex
%       \lineskiplimit .2ex
   \ifinpile\else
        \skip2\z@
          plus 1.5\word@stretch % whole map stretches like three words
          minus .5\word@shrink % but shrinks like one
        \skip4\skip2
\fi\fi
\let\@filler\@fillh
%\let\fill@dot\hfdot % 28.7.95
\let@names{fill@dot}{rf:.}% 30.7.98
}%
%
% \ruTo -> \+To \PositiveGradienttrue \rTo (2,2)
% \+To  -> \Vector@Map \+t: \+f:- \+m: \+f:- \+h:>
% \@vector@setup sets \max@fraction and collects the five diagonal parameters.
% then \rTo is run with an altered definition of \Horizontal@Map
%
%\def\Rising@Map#1#2{\PositiveGradienttrue
%   \if@cd@use@PS@\@cd@PS@horiz@true\expandafter#1\else\expandafter#2\fi}%
%\def\Falling@Map#1#2{\PositiveGradientfalse
%   \if@cd@use@PS@\@cd@PS@horiz@true\expandafter#1\else\expandafter#2\fi}%
\def\Vector@Map{\@vector@setup 4}%
\def\Slant@Map {\@vector@setup{\if@use@TPIC@255\else6\fi}}%
\def\Slope@Map {\@vector@setup\default@max@fraction}% 7.4.95
%
% #1=maxfraction #2=tail #3=filler #4=middle #5=filler #6=head followed by
% gradient assignment and horizontal map to use in PostScript mode
\def\@vector@setup#1#2#3#4#5#6{%
  \default@args
  \def\x@coord{2}\def\y@coord{2}% coordinates for diagonals
  \def\x@offset{1}\def\y@offset{1}% diagonalbase
  %\global\@diagonals@used@true 12.7.94 moved to \exec@diagonal
  \let\Horizontal@Map\Rotated@Horizontal
  \def\max@fraction{#1}%
  \def\reassign@parts{\assign@five#2#3#4#5#6}%
}%
%
\def\Rotated@Horizontal{%
\@setup@horiz
\@cd@PS@horiz@true
\let\exec@map\exec@diagonal
\five@args}%
%
\new@if\if@cd@missive@\@cd@missive@true\@cd@missive@false\@cd@missive@true
\def\cds@missives{\@cd@missive@true}%
\def\exec@diagonal{%
   \if@cd@use@PS@
        \let\max@fraction\default@max@fraction
        \calc@horiz
        % attach labels to horizontal arrow if hug option
        \if@hug@\label@horiz\fi  % hug option 4.7.97
        \setbox0\hbox{\incommdiagfalse\put@horiz}%
        \if@cd@missive@
             % use missives to stretch the arrow in second pass
             % (\box0 and the labels are sent as the data)
             \exec@missive
        \else\global\@diagonals@used@true % 12.7.94
             % set the PS diagonal here on the first pass
             % (only uses \box0, so no labels unless they're in \box0)
             \exec@PS@diagonal
        \fi
        \ifvoid6 \ifvoid7 \@hug@true\fi\fi
        \if@hug@\else
             % 4.7.97 lazy implmentation of nohug option
             % assign empty parts to a LaTeX diagonal arrow
             \empty@parts
             \global\@diagonals@used@true
             \let\make@line\no@make@line % hack!
             \exec@LaTeX@diagonal
        \fi   
   \else\reassign@parts
        \reassign@filler
        \global\@diagonals@used@true % 12.7.94
        \exec@LaTeX@diagonal
   \fi}%
%
%
% default labels etc appropriate to all kinds of arrows
\def\default@args{%
\begingroup             % 
\dimen1=\MapShortFall   % leading shortfall
%\dimen2.5em            % min tip-to-tip arrow len within diagrams 15.4.95 
\dimen2=\min@map@length% minimum tip-to-tip length of arrow
\dimen5=\MapShortFall   % trailing shortfall
\setbox3=\box\voidb@x   % middle label
\setbox6=\box\voidb@x   % upper or left label
\setbox7=\box\voidb@x   % lower or right label
\@first@positional@true   % haven't done \positional@ yet
\mathsurround\z@        %
\skip2\z@ plus1fill minus 1000pt% amount to fill on left
\skip4\skip2            % and right
\@cd@through@false}%
%
\new@if\if@cd@through@\@cd@through@true\@cd@through@false
%
\def\assign@five#1#2#3#4#5{%
\let\@tail#1\let\@filla#2\let\@middle#3\let\@fillb#4\let\@head#5%
\@cd@through@false\ifx\@filla\@fillb\@cd@through@true\fi}%
%
\def\five@args#1#2#3#4#5{\assign@five#1#2#3#4#5\get@arg}%
%
%
%\def\front@args#1#2#3{%
%\let\@tail#3\let\@filla#2\setbox3=#1\let\@fillb\empty\let\@head\null\get@arg}%
%
%\def\back@args#1#2#3{%
%\let\@tail\null\let\@filla\empty\setbox3=#1\let\@fillb#2\let\@head#3\get@arg}%
%
%
% \dTo ->  \Vertical@Map \dt: \df:- \dm: \df:- \df:>
% \five@args picks up these five parameters and calls \get@arg
% which calls \exec@vert
%
\def\Vertical@Map{%
\check@vert433{vertical map}\exec@vert
\default@args
\cd@penalty-9995
\let\@filler\@fillv
%\let\fill@dot\vfdot % 12.7.94
\let@names{fill@dot}{df:.}% 30.7.98
\five@args}%
%
\def\break@args{%
     % If \get@arg happens to be called again,
     % make it do its continuation straight away.
     \def\get@arg{\exec@map}%
     \exec@map          % do the continuation
   \endgroup            % close the map environment
  \aftergroup\group@after@map}% check for enclosing braces
%
\def\set@map@parts{%
\setbox1=\@tail\setbox5=\@head
\ifvoid3 \ifx\@middle\null\else\setbox3=\@middle\fi\fi
\make@filler 2\@filla
\make@filler 4\@fillb
}%
%
%
\def\lift@map@parts#1{%
% lift all map parts by #1
\ifvoid 1\else\lift@map@part 1#1\fi
\ifvoid 2\else\lift@map@part 2#1\fi
\ifvoid 3\else\lift@map@part 3#1\fi
\ifvoid 4\else\lift@map@part 4#1\fi
\ifvoid 5\else\lift@map@part 5#1\fi
}
%
% lift map part #1 by #2
\def\lift@map@part#1#2{\setbox#1\vbox{%
\offinterlineskip
\box#1%
\dimen@\prevdepth
\advance\dimen@-#2\relax
\setbox0\null\dp0\dimen@\ht0-\dimen@
\box0}}%
%
\def\make@filler#1#2{%
\ifx#2\@filler
   \setbox#1=\box\voidb@x
\else
   \setbox#1=#2%
   \def#2{\xleaders\box#1}%
\fi}%
%
%
% ****************** OLD-STYLE MAP SETUP *****************
%
\cd@first@use\use@newarrow{\string\HorizontalMap, \string\VerticalMap\space
and \string\DiagonalMap\new@line are obsolete - use \newarrow@name\space
to pre-define maps}%
%
\def\HorizontalMap#1#2#3#4#5{%
\use@newarrow
\check@horiz{old horizontal map}% avoid clashes
\default@args
\@setup@horiz
\def\@tail{\old@horiz@part{#1}}% left tip, eg \rthookb
\old@horiz@fill\@filla{#2}% filler
\def\@middle{\old@horiz@part{#3}}% middle
\old@horiz@fill\@fillb{#4}% filler
\def\@head{\old@horiz@part{#5}}% right tip, eg \rhvee
\get@arg}%
%
\def\VerticalMap#1#2#3#4#5{%
\use@newarrow
\check@vert433{vertical map}\exec@vert
\default@args
\cd@penalty-9995
\let\@filler\@fillv
\def\@tail{\make@vert@part{#1}}% upper tip, eg \dthooka
\old@vert@fill\@filla{#2}% filler
\def\@middle{\make@vert@part{#3}}% middle
\old@vert@fill\@fillb{#4}% filler
\def\@head{\make@vert@part{#5}}% lower tip, eg \dharrow
\get@arg}%
%
\def\DiagonalMap#1#2#3#4#5{%
\use@newarrow
\default@args
\def\max@fraction{4}%
\let\@filler\undefined
\let\exec@map\exec@LaTeX@diagonal
\def\x@coord{2}\def\y@coord{2}% coordinates for diagonals\default@args
\def\x@offset{1}\def\y@offset{1}% diagonalbase
\def\@middle{\make@diag@part{#3}}%
\ifPositiveGradient
     \let\mv\raise
     \def\@tail{\make@diag@part{#5}}%
     \def\@filla{\make@diag@part{#4}}%
     \def\@fillb{\make@diag@part{#2}}%
     \def\@head{\make@diag@part{#1}}%
\else\let\mv\lower
     \def\@tail{\make@diag@part{#1}}%
     \def\@filla{\make@diag@part{#2}}%
     \def\@fillb{\make@diag@part{#4}}%
     \def\@head{\make@diag@part{#5}}%
\fi
\get@arg}%
%
% \vertical@name was in the "corruption-sensitive" section
\def\horizontal@name{-}\def\empty@name{\empty}%\def\vertical@name{|}
\def\old@horiz@fill{\make@old@fill\horiz@repeater\horizontal@name\@fillh}%
\def\old@vert@fill {\make@old@fill\vert@repeater \vertical@name  \@fillv}%
%
\def\make@old@fill#1#2#3#4#5{\def\next{#5}%
\ifx    \next#2%
        \let#4#3%        rule filler
\else   \let#4\null %    empty filler
\ifx    \next\empty\else
\ifx    \next\empty@name
\else   \let#4\next%     other filler
\fi\fi\fi}%
%
\def\old@horiz@part#1{%
\hbox{\mathsurround\z@\offinterlineskip
        \def\next{#1}%
        \ifx\next\empty\else\ifx\next\empty@name\else
        \begin@maths\mkern-1.5mu{\next}\mkern-1.5mu\end@maths
        \fi\fi
}}%
%
%
%=======================================================================%
%                                                                       %
%       (5A) LABELS                                                     %
%                                                                       %
%=======================================================================%
%
% \get@arg -> \switch@arg -> various -> \break@args -> \exec@map
% ^_<>~    -> \left@label etc -> \get@label -> \@get@label ->
%   \switch@label@arg -> \(un)braced@label -> \@end@label -> \get@arg
%
% Pick up following label and assign it appropriately.
% idea: force expansion of #3 before we read it (but this may execute & or \cr)
% idea: ensure that \box3 (in particular) doesn't shrink
% (\exec@horiz does this)
% vertical positioning of labels with descenders?
%
\def\get@label#1#2{% put label #3 in box #1 (#2 is ^_<>~-)
  \setbox#1=\hbox\bgroup
    \setbox0=\hbox{\begin@maths\labelstyle()\end@maths}%% ASCII round brackets
    \setbox1=\null\ht1\ht0\dp1\dp0\box1
    \kern.1\@em%
    \begin@maths
       \bgroup       % matches user's close brace (\begingroup wouldn't)
          \labelstyle
                                \aftergroup\@end@label
                                \@get@label}%
          %
          %#3%
       %\egroup supplied by the user or in \unbraced@label
                                \def\@end@label{%
    \end@maths
    \kern.1\@em%
  \egroup
    % We used to do the following to the finished box:
    %  \dimen0=\ht#1\advance\dimen0.4ex\ht#1=\dimen0
    %  \dimen0=\dp#1\advance\dimen0.4ex\dp#1=\dimen0
  \get@arg      % continue processing of further arguments
}%
%
% The text of the label is read in the same way as is that of a footnote
% (TeXbook page 363), ie we look at the next token, swallowing it if it is
% an open brace, and use \aftergroup to regain control after the close.
% At various places we do \end@label just in case the closing brace has been
% omitted; this is \empty outside the label text, but causes an error and
% inserts the closing brace inside it. We choose \empty rather than \relax
% because the latter would inhibit correct expansion of \cr\enddiagram.
%
\def\@get@label{\futurelet\next@token\switch@label@arg}%
%
\def\switch@label@arg{%% qualifiers on label arguments
\catcase\bgroup:\braced@label;% label text enclosed in {}
\catcase\egroup:\missing@label;% 
\catcase\space:\label@eat@space;% ignore space
\tokcase     [:\label@optional;%%]%ascii close square bracket 
\default      :\unbraced@label;% single token label text without {}
\endswitch}%
%
%\def\@get@label{%
%  \ifcat\bgroup\noexpand\next@token
%       \expandafter\braced@label
%  \else\expandafter\unbraced@label
%  \fi}%
%
\def\braced@label{%
    \let\end@label\bad@end@label      
    \let\next % pick up and discard user's opening brace (cf \footnote)
    }%
%
%\def\unbraced@label#1{\labelstyle#1\@end@label}% before 28.12.93
%
\def\unbraced@label#1{%
    \let\label@egroup\egroup
    {%
     \let\actually@braces@missing@around@macro@in@label\outer@empty
     \let\end@label\egroup@missing@label
     \let\label@egroup\label@egroups
     #1%
     \actually@braces@missing@around@macro@in@label
    }%
    \label@egroup
}%
\def\actually@braces@missing@around@macro@in@label{\let\next=}%
\def\missing@label{\egroup\cd@error{missing label}\help@endlabel}%
\def\egroup@missing@label{\egroup\missing@label}%
\outer\def\outer@empty{}%
% 14.4.94
% normally, \eat@egroup does nothing and
%    \label@egroup expands (once) to \egroup matching \bgroup above
% if #1 is \egroup, \eat@egroup eats following }, then
%    \label@egroup matches { and then \bgroup (no error message)
% if #1 is \rTo (or some other diagram command beginning \end@label)
%    then \end@label matches { and \bgroup with "missing label" error;
%    later \eat@egroup eats the following } and \label@egroup does nothing.
% if #1 is a macro it takes \missing@braces@around@label@macro as its first
%    argument; however as this is \outer there is an error message;
%    the } prevents the macro from taking \label@egroup as a second
%    argument (it gets \par instead)
%    then } matches { and \label@egroup matches \bgroup.
% if TeX inserts { after #1 (as it does e.g. for \hat), the } matches this
%    and \label@egroup inserts an explicit } token (as many as TeX inserted })
%    until it becomes \egroup, which matches the \bgroup above.
% (If we had assigned \egroup\label@egroup to \label@group the first time,
% the final (empty) \label@egroup would be left to be parsed as the next
% label argument and would fall through \switch@arg.)
% Unfortunately this doesn't pick up the *real* macro arguments,
% and TeX's error recovery is rather messy, but at least doesn't loop.
\def\label@egroup{}%
\def\label@egroups{\eegroup\label@egroup}% 15/4/95 changed from \egroup
%
\def\end@label{}%
%
\def\label@optional% 12.7.94
{\let\after@opt@arg\@get@label\get@square@arg\get@opt@arg@list}%
%
\new@help\help@endlabel{The text which has just been read is not allowed
  within map labels.}%
\def\bad@end@label{\egroup
  \cd@error{missing \egroup@name\space inserted after label}\help@endlabel}%
%
% OLD VERSION
% Catch missing label before closing bracket. ?When can this happen?
% TeX would insert \par for the missing argument, which would then become
% \enddiagram. Perhaps we should just redefine \par locally instead.
% Come to think of it, such a closing bracket has no business to be there
% anyway.
% Other cases can look after themselves by inserting \end@label.
% Could recognise (any kind of) \bgroup and change it to
% \bgroup\aftergroup\end@label to allow label environments.
% \def\@get@label{%
% \ifcat        \next@token\egroup
%       \expandafter\label@is@egroup
% \else \expandafter\@@get@label
% \fi}%
%\def\@get@label#1{#1\end@label}% was \@@get@label
%\def\label@is@egroup{\cd@error{arrow commands must not be em-braced}
%\help@brace
%  \end@label}%
%\new@help\help@label{A closing bracket followed \string
%                           ^, \string
%                              _, \string
%                                 <, \string
%                                    > or \string~.}%
%
% ******************* arrow argument parsing ********************
%
%            ----- Fetch particular labels -----
%
%   \hbox6 gets first/upper/left label & disables positional assignment to it
\def\upper@label {\@first@positional@false\get@label6}%
%   \hbox7 gets second/lower/right label label & disables all positional
\def\lower@label {\def\positional@{\@cd@a@true\break@args}\get@label7}%
\def\middle@label{\get@label3}% \hbox3 is (middle of arrow or) middle label
\new@if\if@first@positional@\@first@positional@true\@first@positional@false
%
\def\left@label{%
\ifPositiveGradient
\then   \expandafter\upper@label
\else   \expandafter\lower@label
\fi}%
\def\right@label{%
\ifPositiveGradient
\then   \expandafter\lower@label
\else   \expandafter\upper@label
\fi}%
\def\positional@{\cd@warning{labels as positional arguments are obsolete}%
\if@first@positional@
\then   %\@first@positional@false
        \expandafter\upper@label
\else   %\let\positional@\break@args % third positional argument terminates
        \expandafter\lower@label
\fi-}% provide dummy second argument (^_<>~) to \getlabel
%
%
%             ----- other argument parsing subroutines -----
%
% Get following token, perform case analysis and repeat or do \exec@map.
\def\get@arg{\futurelet\next@token\switch@arg}%
%
% discard following space and re-read token
\def\eat@space{\afterassignment\get@arg\let\next@token= }%
\def\label@eat@space{\afterassignment\@get@label\let\next@token= }%
%
% get a pair of coordinates, and an optional argument
\def\co@ordinates{\get@round@pair\@getcoords}%
\def\@getcoords#1#2{\def\x@coord{#1}\def\y@coord{#2}\get@arg}%
\def\optional@{\let\after@opt@arg\get@arg\get@square@arg\get@opt@arg@list}%
\def\set@dot@filler.{\do@set@dot@filler\get@arg}% 12.7.94
\def\do@set@dot@filler{% 13.11.94
     \let\@filla\fill@dot\let\@fillb\fill@dot % horizontals or verticals
     \def\reassign@filler{\let\@filla\dfdot\let\@fillb\dfdot}}% diagonals
\def\reassign@filler{}%
%
%=======================================================================%
%                                                                       %
%       (6) OPTIONAL ARGUMENTS                                          %
%                                                                       %
%=======================================================================%
%
%
% - width of each cell individually
%
% blobs:        define . o x O !
% poset (Hasse):size=2em,abut,blobs
% adjunction:
%
%\def\@@getoptarg#1,{%
%   \parse@opt@arg#1,%
%   \let\next\do@opt@arg@then
%   \ifx\@name\end@square@name
%       \let\next\after@opt@arg
%       \let\after@opt@arg\relax
%       \if@was@pair@\bad@pair@opt\fi
%   \fi
%   \next
%}%
%
%\def\do@opt@arg@then{\do@opt@arg\@@getoptarg}%
%
\def\@@getoptarg#1,{%
\parse@opt@arg#1,%
\begingroup
  \ifx\@name\end@square@name
     \if@was@pair@\aftergroup\bad@pair@opt\fi
     \aftergroup\do@after@opt@arg
  \else
        %\batchmode
        \expandafter\def\expandafter\@junk\expandafter{%
            \csname
            \@name%
            \endcsname}%
        %\scrollmode
        \expandafter\get@csname\@junk\end@get@csname
        \ifx\@junk\empty
             \aftergroup\do@opt@arg
             \expandafter\aftergroup\csname\cd@opt@prefix\@name\endcsname
             \expandafter\aftergroup\csname\cd@opt@prefix @\@name\endcsname
        \else
             \gdef\g@tmp{#1}%
             \cd@warning{\string\relax\space inserted before `[\g@tmp'}%
             \message{(I was trying to read this as a \cd@name\ option.)}%ascii
             \aftergroup\add@relax@before@square@bracket
        \fi
  \fi
\endgroup}%
%
\def\get@csname#1#2\end@get@csname{\def\@junk{#2}}%
\def\do@after@opt@arg{\let\next\after@opt@arg\let\after@opt@arg\relax\next}%
%
\def\add@relax@before@square@bracket#1],{%% ASCII close square bracket
  \do@after@opt@arg\relax
  \def\@junk{#1}%
  \ifx\@junk\empty
       \def\@junk{[\g@tmp]}%% ASCII open and close square bracket
  \else\def\@junk{[\g@tmp,#1]}%% ASCII open and close square bracket
  \fi
  \@junk}%
%
\def\do@opt@arg#1#2{%
%\expandafter\let\expandafter\next\csname\cd@opt@prefix @\@name\endcsname
% \next=#1=\csname cds@\@name\endcsname
% #2=\csname cds@@\@name\endcsname
\ifx#2\undefined
     \ifx#1\undefined
          % neither \cds@name nor \cds@@name is defined
          \cd@warning{option `\@name' undefined}%
     \else
          % \cds@name is defined but \cds@@name isn't: execute without pair
          #1%
     \fi
\else
     % \cds@@name#1#2 is defined - the command takes a pair value
     \if@was@pair@
         % this is the second half - execute and reset
         \expandafter#2\@value
         \@was@pair@false
     \else
         % this is the first half - set flag and wait
         \@was@pair@true
\fi  \fi
\next@opt@arg}%
%
\new@if\if@was@pair@\@was@pair@true\@was@pair@false
%
\def\parse@opt@arg#1,{%
   \if@was@pair@
      \ifx\@value\undefined\bad@pair@opt\else
            \expandafter
        \@parse@pair
            \@value
            ,#1,(,),(,)[]%%ASCII 5commas two pairs round, pair square
   \fi\fi
   \if@was@pair@ % tries again if parsing as a pair failed
   \else\@parse@opt@arg#1==,%
   \fi
}%
\def\bad@pair@opt{%
   \cd@warning{option `\@name' needs (x,y) value}%
   \@was@pair@false
   \let\@name\empty}%
%
\def\@parse@opt@arg#1=#2=#3,{%
    \def\@name{#1}\def\@value{#2}\def\@junk{#3}%
    \ifx\@junk\empty\let\@value\undefined\fi
}%
%% ASCII 2commas 2pair round, pair square on next line
\def\@parse@pair#1(#2,#3)#4,(#5,#6)#7[]{%ascii
    \def\@value{{#2}{#3}}%
    \def\@junk{#1#4#5#6}%
    \ifx\@junk\empty
         \def\@junk{#7}%
         \ifx\@junk\empty\bad@pair@opt\fi
    \else\bad@pair@opt
    \fi
}%
%
\def\cd@opt@prefix{cds@}\let\after@opt@arg\relax
%
%
%
\def\get@mand@value#1{%
\ifx\@value\undefined
        \cd@warning{option `\@name' needs a value}%
\else
        #1\@value\relax
\fi}%
%
\def\get@opt@value#1#2{%
\ifx\@value\undefined
        #1#2\relax
\else
        #1\@value\relax
\fi}%
%
\def\cds@@showpair#1#2{\message{x=#1,y=#2}}%
\def\cds@@diagonalbase#1#2{\edef\x@offset{#1}\edef\y@offset{#2}}%
%
\def\ps@prog#1{%
    \def\next{#1}%
    \let@names{@x}{cdps@#1}%
    %\message{PostScript translator `#1` requested.}%
    \ifx\next\empty\bad@ps@prog\next{cannot be used}%
    \else\ifx\next\relax % \csname undefined\endcsname = \relax
         \bad@ps@prog\next{unknown}%
    \else\let\verbatim@ps@special\@x
    \fi\fi
}%
\def\bad@ps@prog#1#2{% 24.8.2003 pass name as #1 instead of \@value
   \cd@warning{PostScript translator `#1' #2}}%
   %\dont@use@ps\let\cds@PS\empty\let\cds@noPS\empty}% removed 30.12.07
%
%
\def\obs@display{}%
\def\set@new@display{\@cd@hbox@false\edef\obs@display{\noexpand
  \cd@refmt@error{\@name\space ignored within maths}}}%
%
\def\diagramstyle{%
  \size@dependencies
  \let\after@opt@arg\relax % 13.7.94
  \@ifoptarg\get@opt@arg@list\get@opt@arg@list}%
\let\diagramsstyle\diagramstyle
%
% ********************** THE ACTUAL OPTIONS *************************
%
%
\new@if\if@cd@text@flow@\@cd@text@flow@true\@cd@text@flow@false
\new@if\if@cd@one@liner@\@cd@one@liner@true\@cd@one@liner@false
\new@if\if@cd@leqno@\@cd@leqno@true\@cd@leqno@false
\new@if\if@cd@centre@display@\@cd@centre@display@true\@cd@centre@display@false
\@cd@centre@display@true
\new@if\if@cd@centre@hlabel@\@cd@centre@hlabel@true\@cd@centre@hlabel@false
\new@if\if@cd@centre@vlabel@\@cd@centre@vlabel@true\@cd@centre@vlabel@false
\new@if\if@use@TPIC@\@use@TPIC@true\@use@TPIC@false
\new@if\if@cd@PS@horiz@\@cd@PS@horiz@true\@cd@PS@horiz@false
\new@if\if@cd@hbox@\@cd@hbox@true\@cd@hbox@false
\new@if\if@cd@landscape@\@cd@landscape@true\@cd@landscape@false % 10.7.94
\new@if\if@need@PS@lib@\@need@PS@lib@true\@need@PS@lib@false % 10.7.94
%
\def@name{cds@ }{}\def@name{cds@}{}% spaces are no-ops
\def@name{cds@1em}{\CellSize1\@em}\def@name{cds@1.5em}{\CellSize1.5\@em}%
\def@name{cds@2em}{\CellSize2\@em}\def@name{cds@2.5em}{\CellSize2.5\@em}%
\def@name{cds@3em}{\CellSize3\@em}\def@name{cds@3.5em}{\CellSize3.5\@em}%
\def@name{cds@4em}{\CellSize4\@em}\def@name{cds@4.5em}{\CellSize4.5\@em}%
\def@name{cds@5em}{\CellSize5\@em}\def@name{cds@6em}{\CellSize6\@em}%
\def@name{cds@7em}{\CellSize7\@em}\def@name{cds@8em}{\CellSize8\@em}%
\def\cds@abut{\MapsAbut\dimen1\z@\dimen5\z@}%
\def\cds@alignlabels{\@cd@centre@hlabel@false\@cd@centre@vlabel@false}%
\def\cds@amstex{%
  \ifincommdiag
       \amstex@diagram@setup
  \else\def\CD{\diagram[amstex]}%%ascii square brackets []
  \fi
  \assign@at\catcode`\@\active
}%
\def\cds@b{\let\cd@vert@positioning\cd@vbottom}%
\def\cds@balance{\let\cd@horiz@positioning\cd@balance}%
\let\cds@bottom\cds@b
\def\cds@center{\cds@vcentre\cds@nobalance}%
\let\cds@centre\cds@center
\def\cds@centerdisplay{%
  \@cd@centre@display@true\set@new@display\cds@balance}%
\let\cds@centredisplay\cds@centerdisplay
\def\cds@crab{\get@opt@value\crab@{.5\PileSpacing}}%
\def@name{cds@crab-}{\crab@-.5\PileSpacing}%
\def@name{cds@crab+}{\crab@.5\PileSpacing}%
\def@name{cds@crab++}{\crab@1.5\PileSpacing}%
\def@name{cds@crab--}{\crab@-1.5\PileSpacing}%
\def\cds@defaultsize{\get@opt@value{\let\default@size}{3em}\set@max@fraction}%
\def\cds@displayoneliner{\@cd@one@liner@false}%
\let\cds@dotted\do@set@dot@filler
\def\cds@dpi{\set@resolution{1truein}}%
\def\cds@dpm{\set@resolution{100truecm}}%
\let\cd@eqno\undefined
\def\cds@eqno{%
  \let\cd@eqno\@value
  \let\set@currentlabel\empty}%
\def\cds@fixed{\@cd@missive@false}%
\new@if\if@adjust@flush@left@\@adjust@flush@left@true\@adjust@flush@left@false
\def\cds@flushleft{%
  \@adjust@flush@left@false % 15.6.97
  \@cd@centre@display@false\set@new@display\cds@nobalance
  \get@opt@value\cd@left@margin\cd@left@margin}%
\def\cds@gap{\set@axis%
  \setbox3=\null\ht3=\rule@height\dp3=\rule@depth 
  \get@opt@value{\wd3=}\MapShortFall}
\def\cds@grid{%
  \ifx\@value\undefined
      \let\h@grid\relax\let\v@grid\relax
  \else
      \let@names{h@grid}{cdgh@\@value}%
      \let@names{v@grid}{cdgv@\@value}%
      \ifx\h@grid\relax
          \cd@warning{unknown grid `\@value'}%
      \else\@cd@tight@true
  \fi\fi}%
\let\h@grid\relax\let\v@grid\relax
\def\cds@gridx{\ifx\@value\undefined\else\cds@grid\fi
  \let\next\h@grid\let\h@grid\v@grid\let\v@grid\next}%
\def\cds@h{\get@mand@value\DiagramCellHeight}%
\def\cds@hcenter{\let\cd@horiz@positioning\cd@fullwidth}%
\let\cds@hcentre\cds@hcenter
\def\cds@heads{%
  \get@opt@value{\let\the@default@head}\the@default@head
  \set@arrowhead
  \if@cd@use@PS@\else\ifx\the@default@head\LaTeX@name\else
        \default@diagonal
  \fi\fi
}%
\let\cds@height\cds@h
\let\cds@hmiddle\cds@balance
\def\cds@htriangleheight{\get@opt@value\DiagramCellHeight\DiagramCellHeight
   \DiagramCellWidth1.73205\DiagramCellHeight}%
\def\cds@htrianglewidth{\get@opt@value\DiagramCellWidth\DiagramCellWidth
   \DiagramCellHeight.57735\DiagramCellWidth}%
\new@if\if@hug@\@hug@true\@hug@false\@hug@true
\def\cds@hug{\@hug@true}
\def\cds@inline{\@cd@hbox@true\let\obs@display\empty}%
\def\cds@inlineoneliner{\@cd@one@liner@true}%
\def@name{cds@l>}{\get@mand@value{\let\min@map@length}\dimen2=\min@map@length}%
\def\cds@labelstyle{\get@mand@value{\let\labelstyle}}%
\def\cds@landscape{\@cd@landscape@true}% 10.7.94
\def\cds@large{\CellSize5\@em}%
\let\set@currentlabel\empty
\def\set@currentlabel@to@equation{%
   \refstepcounter{equation}%
   \def\cd@eqno{\hbox{\@eqnnum}}}%
\def\cds@LaTeXeqno{\let\set@currentlabel\set@currentlabel@to@equation}%
\def\cds@lefteqno{\@cd@leqno@true}%
\def\cds@leftflush{\cds@flushleft\@adjust@flush@left@true}% 15.6.97
\def\cds@leftshortfall{\get@mand@value{\dimen1 }}%
% \def\cds@locate
\def\cds@lowershortfall{\ifPositiveGradient\cds@leftshortfall\else
        \cds@rightshortfall\fi}%
\def\cds@loose{\@cd@tight@false}%
\def\cds@midhshaft{\@cd@centre@hlabel@true}%
\def\cds@midshaft{\@cd@centre@hlabel@true}%
\def\cds@midvshaft{\@cd@centre@vlabel@true}%
%\def\cds@midvshaft{\cd@warning{midvshaft option doesn't work}}%
\def\cds@moreoptions{\@cd@a@true}% tested in \@@@diagram
\let\cds@nobalance\cds@hcenter
\def\cds@nohcheck{\nohcheck}%
\def\cds@nohug{\@hug@false}
\def\cds@nooptions{\def\@@diagram{\exec@diagram}}%
\let\cds@noorigin\cds@nobalance
\def\cds@nopixel{\pixel@size 4\one@sp\size@dependencies}%
\def\cds@UO{\dont@use@ps\global\let\better@use@ps\empty}%
\def\cds@UglyObsolete{\cds@UO\let\cds@PS\empty}% \let\cds@noPS\empty}% 30.12.07
\def\cd@nonoPS#1{\cd@warning{option `#1' renamed as `UglyObsolete'}}% 30.12.07
\def\cds@noPostScript{\cd@nonoPS{noPostScript}}% 30.12.07
\def\cds@noPS{\cd@nonoPS{noPostScript}}% 30.12.07
\def\cds@notextflow{\@cd@text@flow@false}%
\def\cds@noTPIC{\@use@TPIC@false}%
\def\cds@objectstyle{\get@mand@value{\let\objectstyle}}%
\def\cds@origin{\let\cd@horiz@positioning\cd@zerowidth}%
\def\cds@p{\get@mand@value\PileSpacing}%
\let\cds@pilespacing\cds@p
\def\cds@pixelsize{\get@mand@value\pixel@size\reset@map@breadth}%
\def\cds@portrait{\@cd@landscape@false}% 10.7.94
\def\cds@PostScript{\use@ps\global\let\better@use@ps\empty
        \get@opt@value\ps@prog\empty}%
\def\cds@PS{\use@ps\global\let\better@use@ps\empty}%
\info@at@end\better@use@ps{\typeout{\cd@name: try the PostScript option for better results}}%
\def\cds@repositionpullbacks{%
  \let\make@pbk\overprint@pbk\let\pbk@sh\pbk@osh}% 14.11.94
\def\cds@righteqno{\@cd@leqno@false}%
\def\cds@rightshortfall{\get@mand@value{\dimen5 }}%
\def\cds@ruleaxis{\get@mand@value{\let\axisheight}}% 17.7.94
\def\cds@cmex{\let\make@vert@part\cmex@vert@part
\let\set@offset@axis\set@cmex@offset@axis}%
\def\cds@s{\cds@height\DiagramCellWidth\DiagramCellHeight}%
\def\cds@scriptlabels{\let\labelstyle\scriptstyle}%
\def\cds@shortfall{\get@mand@value\MapShortFall
        \dimen1\MapShortFall\dimen5\MapShortFall}%
\def\cds@showfirstpass{\get@opt@value{\let\firstpass@showboxdepth}\z@}%
\def\cds@silent{\def\cd@refmt@error##1{}\def\cd@warning##1{}}%
\let\cds@size\cds@s
\def\cds@small{\CellSize2\@em}%
\def\cds@snake{\get@opt@value\snake@\z@}% 4.7.97
\def\cds@t{\let\cd@vert@positioning\cd@vtop}%
\def\cds@textflow{\@cd@text@flow@true\set@new@display}%
\def\cds@thick{\let\line@font\tenlnw
   \intended@breadth\default@mapbreadth
   \get@opt@value\MapBreadth{2\intended@breadth}%
   \set@arrowhead}% 15.6.97
\def\cds@thin{\let\line@font\tenln
   \get@opt@value\MapBreadth{\default@mapbreadth}%
   \set@arrowhead}% 15.6.97
\def\cds@tight{\@cd@tight@true}%
\let\cds@top\cds@t
\def\cds@TPIC{\@use@TPIC@true}%
\def\cds@uppershortfall{\ifPositiveGradient\cds@rightshortfall\else
        \cds@leftshortfall\fi}%
\def\cds@vcenter{\let\cd@vert@positioning\cd@vcentre}%
\let\cds@vcentre\cds@vcenter
\def\cds@vtriangleheight{\get@opt@value\DiagramCellHeight\DiagramCellHeight
   \DiagramCellWidth.577035\DiagramCellHeight}%
\def\cds@vtrianglewidth{\get@opt@value\DiagramCellWidth\DiagramCellWidth
   \DiagramCellHeight1.73205\DiagramCellWidth}%
\def\cds@vmiddle{\let\cd@vert@positioning\cd@vmiddle}%
\def\cds@w{\get@mand@value\DiagramCellWidth}%
\let\cds@width\cds@w
%
%
%=======================================================================%
%                                                                       %
%       (7) THE DIAGRAM - OPTIONS AND OUTPUT                            %
%                                                                       %
%=======================================================================%
%
%
% The following macros are preparatory to the diagram, picking up optional
% arguments and beginning the main \vbox.
%
% \diagram -> \@diagram -> \@@diagram [-> \@@@diagram] -> \exec@diagram
% -> \@exec@diagram -> \enddiagram=\@end@diagram -> \after@diagram
% (\matrix@to@buffer, \reformat@matrix) -> \output@diagram -> \exit@diagram
%
\def\diagram{\relax\protect\@diagram}%
\def\enddiagram{\protect\misplaced@enddiagram}% real one in \inner@environment
%
\def\diagraminline{\diagram[inline,moreoptions]}%
\def\enddiagraminline{\enddiagram}%
%
\def\@diagram{%
\bbgroup        % {} closed in \exit@diagram
  \save@begin@at@line   % line number for reformatting error messages
  \incommdiagtrue
  \edef\save@row@no{\the\cd@row}% save row number
  \global\cd@row\z@
    %
    % LaTeX pre 15/12/87 had \maxboxdepth\z@; this found its way into
    % a journal style with which Richard Kennaway had a problem.
  \boxmaxdepth\maxdimen % added 3 June 1994
    %
    % amslatex's equation environment sets \everycr;
    % reported by Bruce Pollock <pollock@newton.rutgers.edu> 5 April 1995
  \everycr{}%
    %
    % test for (active) pdftex
  \test@pdf
    %
    % pdfsync package also sets these: 3 Jan 2006
    % Hubert.Flenner@ruhr-uni-bochum.de  Fri May 14 14:31:36 2004
    % Arthur Ogus <ogus@Math.Berkeley.EDU> Tue Jan  3 17:21:02 2006
  \everymath{}%
  \everyhbox{}%
    %
    % That was not enough.  See email 25--30 Jan 2008 with
    % jerome.laurens@u-bourgogne.fr  (author of pdfsync)
    % and Bernd Strieder <strieder@informatik.uni-kl.de> (user).
  \ifx\pdfsyncstop\undefined\else\pdfsyncstop\fi
%  \futurelet\next
  \@@diagram}%
  %
  \def\@@diagram{%
        \@cd@a@false
        \let\after@opt@arg\@@@diagram
   \@ifoptarg\get@opt@arg@list\exec@diagram}%
  %
%  \def\@@diagram{%             % do we have options?
%     \ifx[\next
%       \expandafter\cd@with@opt        % yes
%     \else
%       \expandafter\exec@diagram       % no
%     \fi
%  }%
%  %
%  \def\cd@with@opt{%
%       \@cd@a@false
%       \let\after@opt@arg\@@@diagram
%       \get@square@arg\get@opt@arg@list}% read and execute options
  %
  \def\@@@diagram{%
  \if@cd@a@                     % did we ask for more options?
        \expandafter\@@diagram          % yes (\cds@moreoptions)
  \else \expandafter\exec@diagram       % no
  \fi}%
  %
  \def\exec@diagram{%
   % \next may have been &, which is a dangerous thing to have around
  \let\next@token\relax
  %
  \if@cd@landscape@\if@cd@use@PS@\else % 10.7.94
        \if@pdf@\else % won't be needed when we're finished
       \cd@refmt@error{landscape ignored without PostScript}%
       \@cd@landscape@false
  \fi\fi\fi
  \set@currentlabel
  %
  \setbox2=\vbox\bgroup % avoid \box0 since overwritten by \everypar
     \inner@environment
     \@exec@diagram
     }%
     % \@exec@diagram is in the next section; it eventually calls
     %
     \def\output@diagram{%
     %
     % having provided the following positioning statistics:
     %     \expandafter\message{%
     %       interaxis=\the\dimen1, %
     %       topheight=\the\cd@top@height, %
     %       fullheight=\the\completed@depth, %
     %       bottomdepth=\the\row@depth, %
     %       dimen0=\the\dimen0, %
     %       dimen2=\the\dimen2, %
     %       dimen7=\the\dimen7, %
     %       right over=\the\right@over, %
     %       left over=\the\left@over%
     %       }%
     %
     %  \dimen0:        distance between leftmost and rightmost centres
     %  \dimen1:        distance between top and bottom axes
     %  \dimen2:        right width of rightmost column
     %  \rule@height :  axis height
     %  \cd@top@height: height of top row
     %  \completed@depth :      height from last baseline to top
     %  \right@over :   from centre of leftmost to far edge of rightmost
     %  \left@over :    left width
     %  \row@depth :    depth of bottom row
     %  \cd@top:        number of rows
     %  \cd@right:      number of columns
     %  \vert@wd@in@leftmost: left width of (last) vertical system in column 1
     %                   or \undefined if none (15.6.97)
     %
     %
     % The commands \cd@horiz@positioning and \cd@vert@positioning are assigned
     % by the positioning options to routines which adjust these statistics.
     %
     \if@cd@landscape@ % 10.7.94
          \cd@vtop
     \else\cd@vert@positioning
     \fi
     \cd@horiz@positioning
     %
     % Now force our box to have the required depth and right width.
     \nointerlineskip
     \setbox0=\null\ht0-\row@depth\dp0\row@depth\wd0\right@over
     \box0
     %
     \global\cd@dim@g\left@over % save left width
     \global\cd@num@g\cd@top    % and number of rows
     %
     % alignment adjustment on left (15.6.97)
     \ifx\vert@wd@in@leftmost\undefined
         \global\cd@dim@h\left@over % no verticals - use edge of text
     \else
         \global\cd@dim@h\vert@wd@in@leftmost % width of multiple verticals
     \fi
     %
  \egroup               % end of \setbox2=\vbox\bgroup in \exec@diagram
  \make@end@at@line     % 
  %
  % The following are now available:
  %  \box2:     the completed diagram, with its left width smashed
  %  \cd@dim@g: the left width
  %  \cd@dim@h: the left width alignment adjustment
  %  \cd@num@g: number of rows
  %  mode:      as in the text outside
  %
  \if@cd@landscape@ % 10.7.94
        \setbox2=\hbox to\dp2{%
          %\dp2=\cd@dim@g\ht2\wd2% replaced with vrule 6.10.2001
          \vrule height\wd2 depth\cd@dim@g width\z@
          \global\cd@dim@g\ht2%
          \ht2\z@\dp2\z@\wd2\z@
          \if@pdf@ 
              \pdf@literal{q 0 1 -1 0 0 0 cm}%
          \else
              \global\@need@PS@lib@true
              \verbatim@ps@special{0 1 bturn}%
          \fi
          \box 2%
          \do@eturn %\verbatim@ps@special{eturn}%
          \hss}%
        \@cd@one@liner@false
  \fi
  %
  \ifnum\cd@num@g=1 \else\@cd@one@liner@false\fi
  %
  \global\@ignorefalse
  %
  % decide what to do with the finished diagram
  %
  \if@cd@hbox@\leavevmode\fi
  %
  \ifvmode
     % vertical mode:
     % ie page \vbox or \vadjust, but \ifinner isn't a reliable indication
     % of which it is, as it is \iftrue in \vbox and also \vadjust.
     % This makes it difficult to see how we could handle floats.
     %
     % We must begin a paragraph.  This is because LaTeX uses \trivlist for
     % numerous purposes (center for instance). This sets a flag (\if@newlist)
     % which is cleared (globally) in \everypar. It claims that there is a
     % "missing item" if it finds it true at the end, ie if no paragraph has
     % been created in the meantime.
     %
     % The usual way of forcing a paragraph is \leavevmode or \noindent,
     % but \cd@display uses $$..$$ and LaTeX seems to be happy with this.
     %
     \cd@display
     %
  \else
     \ifmmode           % maths mode
        %\ifinner\else  % can't distinguish $/$$ within \bbgroup\eegroup
           \obs@display
        %\fi
        \put@cd@box
  %
     \else                      % horizontal mode
        \if@cd@one@liner@\@cd@hbox@true\fi
        \ifinner\@cd@hbox@true\fi
        %
        \if@cd@hbox@     \put@cd@box     % hbox or one-liner option
        \else\if@cd@text@flow@
                        \cd@text@flow   % --- flow
             \else      \cd@display     % --- display
        \fi\fi
  \fi\fi
  %
  \exit@diagram}%
  %
  \def\exit@diagram{%
  %
  \global\cd@row\save@row@no\relax % restore row number
  %
  \if@end@diagram@ok@ % was \enddiagram deliberate or anticipated?
         \global\@end@diagram@ok@false  % deliberate
  \else\aftergroup\do@fated@enddiagram  % antipated - give error message
  \fi
  %
  \if@ignore\aftergroup\ignorespaces\fi % ignore spaces after display
  %
\eegroup % main {} begun in \@diagram
\ignorespaces%
}% and go home!
% That's REALLY the end of the diagram as far as we are concerned,
% although LaTeX will do further processing if \end{diagram} has been used;
% in particular it will do \ignorespaces conditionally on \if@ignore.
%
% ***************** positioning options ********************
%
%   VERTICAL
\def\cd@vtop{\advance\row@depth\dimen1\relax}%
\def\cd@vmiddle{\advance\row@depth.5\dimen1\relax}%
\def\cd@vbottom{}%
\def\cd@vcentre{\cd@vtop\advance\row@depth\cd@top@height\divide\row@depth 2
   \advance\row@depth-\axisheight\relax}%
%
%   HORIZONTAL
\def\cd@fullwidth{}%
\def\cd@zerowidth{\left@over\z@}%
%
\def\cd@balance{%
\ifdim  \dimen2>\left@over 
        \left@over \dimen2
\else   \dimen2\left@over 
        \right@over \dimen0
        \advance\right@over \dimen2
\fi}%
%
% ***************** output manipulation ********************
%
\def\cd@text@flow{%
   %
   % Remove all positive glue from before the diagram and save it.
   % same as LaTeX's \@bsphack \@esphack
   \skip0\z@\relax
   \loop   \skip1\lastskip
   \ifdim  \skip1>\z@
           \unskip
           \advance\skip0\skip1
   \repeat
   %
   \vadjust{%
        % Insert glue and penalties as if TeX
        %   had created the display itself.
        \prevdepth\dp\strutbox
        \penalty\predisplaypenalty
        \vskip\abovedisplayskip
        \cd@display@box
        \penalty\postdisplaypenalty
        \vskip\belowdisplayskip
   }%
   %
   \ifdim\skip0=\z@\else        % if there was any glue before the diagram,
        \hskip\skip0            % put it back afterwards and
        \global\@ignoretrue     % do \ignorespaces after \end{diagram}
   \fi
}%
%
% Our own display output when we have a single
% diagram to contribute to the horizontal list.
% ideas:
% What if preceding line of text is short (\predisplaysize)?
% Calculate \prevgraph based on height of diagram?
%
\def\cd@display{%
  \maths@display        % $$
    \kern-\displayindent% undo any prevailing paragraph indentation
    \cd@display@box     % output the box
  \maths@display%       % $$
  \global\@ignoretrue   % do \ignorespaces after \end{diagram}
}%
%
\def\cd@display@box{\hbox to\hsize{%
  %
  % if [leftflush], adjust alignment (15.6.97)
  \if@adjust@flush@left@\ifdim\cd@dim@h=\z@\else
      \advance\cd@dim@g-\cd@dim@h
      \setbox2=\hbox{\kern\cd@dim@h\box2}%
  \fi\fi
  %
  % make the equation number
  \setbox1=\hbox{\ifx\cd@eqno\undefined\else\begin@maths\cd@eqno\end@maths\fi}%
  % insert it on the left if required
  \if@cd@leqno@
     \if@cd@centre@display@\else
        \advance\cd@dim@g\wd1
     \fi
     \wd1\z@
     \box1
  \fi
  % check that the diagram will fit on the page
  \dimen0\wd2
  \advance\dimen0\wd1
  \advance\dimen0-\hsize
  % does it fit on the page with the specified indentation? 2.3.94
  \ifdim\dimen0>-\cd@left@margin
      % no - switch from flushleft to centredisplay
      \@cd@centre@display@true
  \fi
  % does it fit on the page at all?
  \advance\dimen0\cd@dim@g
  \ifdim\dimen0>\z@
      \cd@refmt@error{wider than the page by \the\dimen0 }%
      \@cd@centre@display@true
  \fi
  % space to the left of the diagram
  \if@cd@centre@display@
        \hss
  \else \at@least\cd@dim@g\cd@left@margin
  \fi
  % output the diagram itself
  \put@cd@box
  % space to the right
  \hss\kern-\wd1\box1   % right equation number (already void if left)
}}%
%
% Raw output used in maths, user display, \hbox (eg picture) and one-liner.
% 10.7.94 define PostScript commands here if needed
\def\put@cd@box{%
   \if@need@PS@lib@\if@in@matrix@\else
      \def@ps@turn
      \global\@need@PS@lib@false
   \fi\fi
   \kern\cd@dim@g\box2 }%
%
%
% ***************** notes ********************
%
% For some reason the usual \futurelet method gets tied up
% if the next token is &.
% (Try again: there was another bug, with \cd@state)
%\def\@diagram{\begingroup\@ifoptarg\cd@with@opt\@@diagram}%
%\def\@@diagram{{%
%       \aftergroup\exec@diagram
%       \ifcat  \next@token\@and
%               \aftergroup\replace@and
%       \fi
%}}%
%
%\def\replace@and{\omit\hskip 1sp plus1fil}\def\@@and{\@and}%
%
% nested diagram bug:
% $\begin{array}{ll}\begin{diagram}&A\\B\end{diagram}$
% causes: ! Emergency stop. <recently read> \endtemplate
% not fixed by \relax or by changing \begingroup\endgroup to \bgroup\egroup
% \@@diagram picks up $ (in right template of array) and the log file ends
% (interwoven alignment preambles are not allowed).  (11 July 1992)
% but it is fixed by changing to \bbgroup\eegroup
%
% idea: forbid a list of commands within diagram
%
%\edef\cd@mode@outside  {% code for external mode
%               \ifmmode\ifinner0%      $..$
%                       \else1\fi%      $$..$$  
%       \else   \ifhmode\ifinner2%      \hbox{..}
%                       \else3\fi%      paragraph (maybe in \vbox)
%       \else   \ifvmode\ifinner4%      \vbox{..} or \vadjust{..}
%                       \else5\fi%      current page
%       \fi\fi\fi}%
%
%=======================================================================%
%                                                                       %
%       (8) THE MATRIX                                                  %
%                                                                       %
%=======================================================================%
%
\new@if\if@diagonals@used@\@diagonals@used@true\@diagonals@used@false
%
\def\inner@environment{%
\size@dependencies
\ifdim\DiagramCellHeight=-\maxdimen\DiagramCellHeight\default@size\fi
\ifdim\DiagramCellWidth =-\maxdimen\DiagramCellWidth \default@size\fi
\global\@diagonals@used@false
\@in@matrix@true % 12.7.94
\let\group@after@map\empty
\let\cd@and\@and
\let\overprint\over@print
\let\@bomb\the@bomb             % pull out the pin!
\let\enddiagram\@enddiagram
\let\\\diagram@cr               % for LaTeX users
\let\par\par@enddiagram         % deal with spurious \par inside diagram
\let\end@label\empty            % we put these at the end
\let\switch@arg\cd@switch@arg   % allow &<>() arguments to maps too
\let\shift\cd@hshift            % shift objects
\baselineskip\DiagramCellHeight % minimum line spacing
\lineskip\z@                    % otherwise, just stretch as necessary
\lineskiplimit\z@               %
\mathsurround\z@                % no unnecessary space in cells
\tabskip\z@                     % or between them horizontally (ignored anyway)
\cd@state                       % set up automaton to check horizontal state
}%
%
%
\def\@exec@diagram{%
\penalty-123             % marker - checked in \matrix@to@buffer
\begingroup             % confine the following to the text of the diagram
\@cd@landscape@false    % don't rotate nested diagrams 12.7.94
\aftergroup\after@diagram% execute at corresponding \egroup
%\incommdiagtrue
%
\halign\bgroup          % begin the matrix (see below for template)
\global\advance\cd@row1 % maintain row number in matrix
\vadjust{\penalty1}%    % code below row picked up in \matrix@to@buffer
\global\cd@cell\z@      % initialise column number
\cd@state               % horiz state (\cd@donat) at left is space donation
\begin@cell##\end@cell  % template for leftmost cell
\@and\@and              % "&&" means repeat following indefinitely
\receive@cell@type      % recover horiz state from \send@cell@type
\begin@cell##\end@cell  % template for subsequent cells
\cr                     % end of template
}%
%
% insert the matrix between calling these two macros
%
\def\@enddiagram{%
\end@label              % catch missing close brace after label
\enddiagram@endpile     % ditto after \pile
\crcr                   % catch missing \cr
\egroup                 % end of \halign
\global\@end@diagram@ok@true% signal we meant
\endgroup               % to do \after@diagram (\aftergroup)
}%
%
%
%=======================================================================%
%                                                                       %
%       (8) CELLS                                                       %
%                                                                       %
%=======================================================================%
%
%
%***************************** the template ****************************
%
% The main purpose of the template is to recognise empty cells quickly.
% The \hbox'es produced by the various types of cell are:
% - empty or white:     \glue 1sp plus 1fil
% - \span (\across):    completely empty
% - object:             \hfil\mathon...\mathoff\hfil
% - arrow etc:          \hfil\mathon...\penalty...\mathoff\hfil
%
% \save@cell@at@line?
% do \futurelet and eager expansion advance \inputlineno? - yes
% (may be better to do it during previous \end@cell instead)
\def\begin@cell{%
%\save@cell@at@line
\global\advance\cd@cell 1
\futurelet\next@token\@begin@cell}%
%
% A hack for future reference:
% Without \end@cell, we'd pick up \endtemplate as \thefirsttoken
% however it's \outer, so the only way of testing for it is by \ifx
% with something obtained in the same way. Moreover \theendtemplate
% must be used before it's defined, because it's \outer.
% Knuth is devious, but we've got round him!
% \def\gettheendtemplate{\glet\theendtemplate\thenexttoken}
% \halign{\futurelet\thenexttoken\gettheendtemplate#\cr\cr}
%
%
\def\@begin@cell{%
\ifx    \next@token\end@cell
\then   \hskip 1sp plus 1fil \relax
        \let\end@cell\relax\save@cell@at@line
\else   \hfil\begin@maths\objectstyle
        \let\group@after@map\bad@group@after@map
\fi}%
%
%
% The \halign cell \hbox of an ordinary object cell is
%       \hfil
%       \mathon
%       (text)
%       \penalty -9993
%       \mathoff
%       \null
%       \kern -2\cd@hshift
%       \null
%
% Missing close brace between label and & will probably be picked up by
% TeX anyway.
%
\def\end@cell{%         % idea: deal with crosses in the same way
\end@label\relax        % in case of missing closing bracket
\send@cell@type         % save new horiz state globally across cell boundary
\save@cell@at@line
\global\cd@dim@g\cd@hshift% save object right shift across $
\penalty-9993           % split off profiling info as last line of paragraph
\end@maths\hfil\null    % $\hfil and protect following glue & penalties
%\penalty\profile@code  % profiling option
\kern-2\cd@dim@g        % balance to indicate right shift
\null                   % protect glue, kerns and penalties
}%
%
\def\diagram@cr{\cr}% optional argument? terminate horizontals?
% NB: vertical mode material in cells (\vadjust, \insert, \write) migrates
% when \cr is executed.
%
%************************ across several columns ***********************
%
% what happens if \across is used for all the the cells in some column?
% count cells
% \across must not follow verticals and crosses
%
% \mscount already defined by \multispan
%
% for some reason, \across3\cr doesn't work with the following definition,
% although \across2\cr, \across3 \cr and \across3& do work.
% \multispan appears to have a similar problem.
% \def\across{\span\omit\relax\afterassignment\spAns\mscount=}
% \def\spAns{\relax\loop\relax\ifnum\mscount>2 \spAn\repeat}
%
%\diagram
%      x&\rTo^{\xi}{}\across3&x'\\
%      \dTo^{u^x_y}{}&&&&\dTo_{u^{x'}_{y'}}\\
%      y&&&&y'\\
%      &\SE{\upsilon}{}&&\SW{}{\upsilon'}\\
%      &&y''\\
%\enddiagram
%       drives \rTo through x' and puts \xi near its right tip!
%
%\cd@first@use\obs@across{\string\across\space should be changed to multiple
%\and@name}%
\def\across#1{\span\omit\mscount=#1
\global\advance\cd@cell\mscount
\global\advance\cd@cell\m@ne
\loop@on@cells
\ifnum\mscount>2 \spAn\repeat
\ignorespaces}%
% use original plain TeX \sp@n? LaTeX version? count cells?
\def\spAn{\relax\span\omit\advance\mscount\m@ne}%
%
%\def\across#1{\message{%
%       ! diagrams Warning: \string\across\ must be changed to multiple &}%
%       \global\def\across#1{}}
%
% idea: back up one line (using \baselineskip\z@) or more (dunno)
%
%
%=======================================================================%
%                                                                       %
%       (8A) SIGNATURE                                                 %
%                                                                       %
%=======================================================================%
%
% Now test whether we have enough space to put our Morse Code signature on the
% stretching horizontal. Only do it in diagrams, where both fillers are "-",
% there is no middle, there is enough space and the rule breadth is positive.
% Do it on the 10th and then every 20th subsequent such occasion.
%
\def\test@signature{%
\ifincommdiag
   \ifx\@filla\@fillh
      \ifx\@fillb\@fillh
         \ifdim\dimen3>\z@\else
            \ifdim\dimen2>93\pixel@size % corrected 24.6.94 for P
            \ifdim\dimen2>18\p@ % added 24.6.94 for high resolution
               \ifdim\intended@breadth>\z@
                  \count@\signature@countdown
                  \advance\count@\m@ne
                  \ifnum\count@<\z@
                     \count@ 20%
                     \let\@signature\the@signature
                  \fi
                  \xdef\signature@countdown{\the\count@}%
\fi\fi\fi\fi\fi\fi\fi
%\showthe\skip2 %\expandafter\message{\signature@countdown}%
}%
% Dots, dashes and spaces are 2, 6 and 2 pixels wide, 1 pixel high.
% However at over 596 dpi resolution this unit is increased:
% \dimen2= 3pixels=0.17pt at 1270dpi, and 6pixels=.17pt at 2540dpi
\def\@morse#1{\vrule\horizhtdp width#1\dimen@\kern2\dimen@}%
%
% Paul Taylor =  .--. .- ..- .-..   - .- -.-- .-.. --- .-.
% Code for "P" corrected 24.6.94 (Ralph Loader)
\def\the@signature{\rlap{%
  \dimen@\pixel@size\at@least\dimen@{.182\p@}\pixel@round\dimen@
   \advance\rule@height\dimen@
   \@morse0\@morse0%                                       4
   \@morse2\@morse6\@morse6\@morse2\@morse0\@morse0%    P 28
   \@morse2\@morse6\@morse0\@morse0%                    A 16
   \@morse2\@morse2\@morse6\@morse0\@morse0%            U 20
   \@morse2\@morse6\@morse2\@morse2\@morse0\@morse0%    L 24
%   \@morse0\@morse0%                           space      4
%   \@morse6\@morse0\@morse0%                           T 12
%   \@morse2\@morse6\@morse0\@morse0%                   A 16
%   \@morse6\@morse2\@morse6\@morse6\@morse0\@morse0%   Y 32
%   \@morse2\@morse6\@morse2\@morse2\@morse0\@morse0%   L 24
%   \@morse6\@morse6\@morse6\@morse0\@morse0%           O 28
%   \@morse2\@morse6\@morse2\@morse0\@morse0%%          R 20
%   \@morse0\@morse0%                           space      4
   }}%
\def\signature@countdown{10}%
\def\@signature{}%
%
%=======================================================================%
%                                                                       %
%       (9) HORIZONTALS                                                 %
%                                                                       %
%=======================================================================%
%
% \dimen 0 = kern compensation for through-filler = \dimen5+\wd5
% \dimen 3 = half width of middle (exactly zero iff filler passes through)
% \skip  3 = glue compensation for through-filler - disappears at break
% \dimen 4 = fixed part of right glue
% \dimen 8 = height of rule filler (.5\rounded@breadth + \axisheight)
% \dimen 9 = depth  of rule filler (.5\rounded@breadth - \axisheight)
%
% what is depth of \vbox{\hrule\horizhtdp}?
%
\def\exec@horiz{%
%\show\if@cd@a@\show\if@cd@through@
\if@cd@a@\@cd@through@false\fi % if more text in cell, disable "through"
\calc@horiz\label@horiz\put@horiz}%
%
%\def\shortfall{\kern\MapShortFall}\def\unshortfall{\kern-\MapShortFall}%
%
% ***************** calculations for horizontal arrows ****************
%
% Calculate (unstretched) dimensions of components of horizontal arrow.
\def\calc@horiz{%
\set@offset@axis\crab@               % set \rule@height and \rule@depth
\set@map@parts
\ifdim\crab@=\z@\else\lift@map@parts\crab@\fi
%
% Half width of middle.
% If this is zero and \@filla=\@fillb, can go straight through
% [don't know what to do if it's negative].
\ifvoid3
        \setbox3=\null\ht3\rule@height \dp3\rule@depth 
\else   \at@least{\ht3}\rule@height\at@least{\dp3}\rule@depth
\fi
\dimen3=.5\wd3
\ifdim  \dimen3=\z@
        \if@cd@through@\else\dimen3-\one@sp\fi
\else   \@cd@through@false
\fi
%
% Find the greater length of labels;
% \dimen2 has been set to minimum arrow length.
\at@least{\dimen2}{\wd7}% extend to label widths
\at@least{\dimen2}{\wd6}%
%\at@least{\dimen2}{.5em}% 15.7.94 removed 15.4.95
%
\test@signature
%
\advance\dimen2-2\dimen3        % middle accounts for some of it
\dimen4.5\dimen2
\dimen2\dimen4                  % half each side
\advance\dimen2\snake@          % shift right for snake option 4.7.97
\advance\dimen4-\snake@         % doesn't work
\advance\dimen2-\wd1            % subtract tips
\advance\dimen4-\wd5
%
% make sure middle is as high and deep as the fillers
% and that leaders print at least one copy
\ifvoid2
\else   \at@least{\ht3}{\ht2}%
        \at@least{\dp3}{\dp2}%
        \at@least{\dimen2}{\wd2}%
\fi
\ifvoid4
\else   \at@least{\ht3}{\ht4}%
        \at@least{\dp3}{\dp4}%
        \at@least{\dimen4}{\wd4}%
\fi
% add stretchability to glue
\advance\skip2\dimen2
\advance\skip4\dimen4
%
% \dimen3=\z@ is a code to say that the filler can pass through.
% By manipulating glue, we make it stretch correctly whether or not the
% bomb explodes.
% (\total@donated, \left@donated and \right@donated are used like this
% during reformatting only)
%   <------------------\total@donated----------------->
%   short  tip  leaders-------------->---kern-->bomb
%   -fall               <-----negative glue-----
%                                          short
%                       middle glue-->tip  -fall
%   <----\left@donated----><--\right@donated--->
% If the bomb does not explode, the negative glue compensates for the kern
% and the right glue (remember that the middle has zero width). The arrow
% may be re-set to any required length as if none of these hacks were there.
%
% If the bomb does explode, the glue (being after the break) automatically
% disappears. The natural and stretched widths of the part to the right of
% the bomb are as expected (with the negative glue they would be zero).
% The width of the part to the left is that of the whole arrow.
% The kern ensuring that the leaders go up to the right tip; the right part is
% still stretched to the right width, so that the middle is correctly placed.
%
% Line-breaking cannot occur at these \xleaders and \kern's outside
% a diagram because they're part of a maths formula (TeXbook p96).
% Inside, the bomb is used (by \reformat@cell) to recognise and split
% the arrow, enabling the halves to be stretched by different amounts.
%
% Since these calculations cannot take account of anything which follows
% the arrow command in the cell, \switch@arg suppresses "through" if
% the arrow command is terminated by anything other than \end@cell.
%
\if@cd@through@
        % leaders can pass though - calculate compensating glue
        \advance\skip2\skip4    % add width+glue of right to left
        \dimen0\dimen5
        \advance\dimen0\wd5     % compensating kern
        \skip3-\skip4           % compensating glue
        \advance\skip3-\dimen0  %
        \let\@fillb\empty       % print nothing on the right
\else   \skip3\z@\relax         % otherwise no compenating glue or kern
        \dimen0\z@
\fi
%
}%
%
% ***************** Add sub & superscript (if any)  ****************
%
% Add to middle,
% retaining baseline and width (2\dimen3) of original middle.
% TeX does this as \vbox{[\kern]\hbox\kern\hbox\kern\hbox[\kern]}
%
\def\label@horiz{%
\offinterlineskip\lineskip.2\@em
\ifvoid6
\else   \setbox3=\vbox{%
                \hbox to2\dimen3{\hss\box6\hss}%
                \box3}%
\fi
\ifvoid7
\else   \setbox3=\vtop{%
                \box3
                \hbox to2\dimen3{\hss\box7\hss}}%
\fi}%
%
% ***************** Output unstretched horizontal ****************
%
\def\put@horiz{% make the horizontal cell - here as seen by paragraph builder
%\hfil\mathon(text)     % beginning of cell and text on left
\kern\dimen1            % space before
\box1                   % left tip
\@signature
\@filla\hskip\skip2     % filler: glue, leader or rule
\kern\dimen0            % kern compensation
\ifincommdiag
        \if@cd@centre@hlabel@\penalty1\fi % signal midhshaft 12.7.94
        \kern\dimen3
        \penalty\cd@penalty
        \hskip\skip3
        \null
        \kern-\dimen3
\else   \hskip\skip3
\fi
\box3                   % middle part of arrow
\@fillb\hskip\skip4     % filler
\box5                   % right tip
\kern\dimen5}%          % space on right
%(text)\penalty-9993
%  \mathoff\hfil\null\kern\z@\null
%\rightskip % text and \end@cell
%
% ***************** PostScript rotation of above ****************
%
%+++ INTERIM: ensure at least \objectheight or \objectwidth
\def\interim@shortfall{%
 \ifnum\numerator@>\denominator@
    \at@least{\dimen1}\objectheight
    \at@least{\dimen5}\objectheight
 \else
    \at@least{\dimen1}\objectwidth
    \at@least{\dimen5}\objectwidth
 \fi
}%
%
% Make the (diagonal) \kern needed on a line
% of length \dimen2 width \dimen7 and height \dimen6
% in order to intersect the edge of a rectangle
% of height \dimen8 and width \dimen9
\def\avoid@object{%
\begingroup
%\expandafter\message{line=(\the\dimen7,\the\dimen6)=\the\dimen2 \space
%  object=(\the\dimen9,\the\dimen8)}%
  \ifdim\dimen7=\z@
        \kern\dimen8 % vertical: use height
  \else\ifdim\dimen6=\z@
        \kern\dimen9 % horizontal: use width
  \else
        \dimen5\dimen6 % save height of line
        \dimen6\dimen9 % width of rectangle
        \set@fraction  % proportion of length
        \dimen4\dimen2 
        \multiply@{\dimen4}%
        \dimen6\dimen5 % restore height of line
        %
        \dimen7\dimen8 % height of rectangle
        \set@fraction  % proportion of length
        \divide@{\dimen2}%
        %
%\expandafter\message{kern=(\the\dimen2,\the\dimen4)}%
        \ifdim\dimen2<\dimen4
                \kern\dimen2 % hit left or right edge
        \else   \kern\dimen4 % hit top or bottom edge
  \fi\fi\fi
\endgroup   
}%
% Stretch a horizontal arrow in \hbox0
% as the diagonal of a rectangle of height \dimen6 and width \dimen7
% avoiding objects
%  above: 
%  below:
%
\def\stretch@PS@diagonal{%
\Pythagorean@sum % hypotenuse=\dimen2 x=\denominator@ y=\numerator@
\setbox\z@\hbox{%
    \lower\axisheight\hbox to\dimen2{%
    \if@reformatting@
        % profile of left object
        \ifPositiveGradient
             % lower left
             \dimen8\ht\object@profile 
             \dimen9\right@width
        \else% upper left
             \dimen8\dp3
             \dimen9\dimen1
        \fi
    \else
       \dimen8 \ifPositiveGradient\objectheight\else\z@\fi \dimen9\objectwidth
    \fi
    \advance\dimen8 \ifPositiveGradient-\fi\axisheight
    \avoid@object% 
    \unhbox\z@
    \if@reformatting@
        % profile of right object
        \ifPositiveGradient
             % upper right
             \dimen8\dp3
             \dimen9\dimen0
        \else% lower right
             \dimen8\ht\object@profile
             \dimen9\left@width
        \fi
    \else
       \dimen8 \ifPositiveGradient\z@\else\objectheight\fi \dimen9\objectwidth
    \fi
    \advance\dimen8 \ifPositiveGradient\else-\fi\axisheight
    \avoid@object%
}}}%
%
\def\exec@PS@diagonal{%
\dimen6 \y@coord\DiagramCellHeight
\dimen7 \x@coord\DiagramCellWidth
\stretch@PS@diagonal
%
\ifPositiveGradient
     \advance\dimen7-\x@offset\DiagramCellWidth
\else\dimen7 \x@offset\DiagramCellWidth
     \dimen6\z@
     %\multiply\numerator@\m@ne % \rotate@box@z does this now
\fi
\advance\dimen6-\y@offset\DiagramCellHeight
%
\rotate@box@z
%
\setbox0=\rlap{%
   \kern-\dimen7
   \lower\dimen6\box\z@}%
\ht0\z@\dp0\z@\raise\axisheight\box0
}%
%
\def\rotate@box@z{%
\setbox0\hbox{%
        \ht\z@\z@\dp\z@\z@\wd\z@\z@
        \if@pdf@  
           \expandafter\pdf@literal{q
              \denom@@\space\num@@\space\mnum@@\space\denom@@\space
              0 0 cm}%
        \else
           \global\@need@PS@lib@true
           \expanded@ps@special{%
           \the\denominator@\space
           \ifPositiveGradient\else-\fi\the\numerator@\space
           bturn}%
        \fi
      \box\z@
      \do@eturn}%
}%
%
% ***************** Complete reformatted horizontal ****************
%
% Initial processing of horizontal arrows at the point of declaration during
% reformatting is in the simple reformatting section.
%
% Output a completed horizontal arrow (see also \widen@pile).
% Result is appended to \box\cd@cell using \output@cell.
% Set up new horizontal donation to left.
%
% The pending horizontal arrow or space donation is saved in \box\pending@left
%  (and \box\pending@right).
%   space:              \box\pending@left  void (\box\pending@right  undefined)
%   \left@donated :     accumulating amount of (left) donation (cell--a)
%   single horizontal:  \hbox\pending@left  is left component,
%                       \hbox\pending@right  right component
%   pile:               \vbox\pending@left  is pile
%   \right@donated :            required right width of horizontals (a--b)
%   \declared@at@cell:  cell number where arrow was declared
%   \far@end@cell:      ditto for obstruction
%
\def\complete@horizontal{%
\advance\left@donated-\right@width 
\total@donated\left@donated\advance\total@donated\right@donated
%
\ifvoid\pending@left
        % no arrow, but check that there is some space between objects
        \ifdim\total@donated<.1em\ifnum\far@end@cell=\@m\else
                \more@dim h\total@donated<.1em:objects overprint:%
                        \cd@cell\far@end@cell
        \fi\fi
\else   \ifhbox\pending@left
                \widen@horiz
        \else   \widen@pile
        \fi
        \advance\total@donated\right@width 
        \output@cell{-\right@width}{\box\pending@left}{\total@donated}\z@
\fi
\left@donated -\left@width      % new space donation to left
                        % - \box\pending@left  is already void
\far@end@cell\cd@cell   % save our column number
\right@donated \z@
}%
%
% re-set single horizontal map, where
% \hbox\pending@left  is left part, width required to be \left@donated,
% cols \cd@cell to \declared@at@cell
% \hbox\pending@right  is right part, width \right@donated,
%  cols \declared@at@cell to \far@end@cell
% \total@donated=\left@donated+\right@donated
%
% before entry:
%   right: DO strip glue/penalty, restore \math@off and re-set naturally
%          DON'T restore \math@on
%   left:  DON'T strip glue/penalty, restore \math@off, or re-set
%          (already has \math@on anyway)
%
\def\widen@horiz{% reorganised 12.7.94
% reset parts to natural width, removing \rightskip & \penalty-9999
\setbox\pending@left=\hbox{\unhbox\pending@left\unskip\unpenalty}%
\setbox\pending@right=\hbox{\unhbox\pending@right\unskip\unpenalty}%
%\showbox\pending@left
%\showbox\pending@right
%
\setbox\pending@left=\hbox to\total@donated{%
        %
        % get the left part, saving its natural width
        \cd@dim@a\wd\pending@left
        \unhbox\pending@left
        %\showboxbreadth=999 \showlists
        %
        % 15.4.95: swapped \kern with midshaft \penalty
        % because penalties got lost at line breaks
        % save the \kern in \cd@dim@b and restore it
        %
        % test for through filler (\kern 0pt)
        \cd@dim@b\lastkern\unkern
        \ifdim  \cd@dim@b=\z@
                \@cd@through@true
                % calculate natural width of left part alone
                \advance\cd@dim@a-\wd\pending@right
        \else   \@cd@through@false
        \fi
        %
        % test for midhshaft (\penalty1)
        \ifnum\lastpenalty=\z@\else
                \@cd@centre@hlabel@true
                \unpenalty
        \fi
        \kern\cd@dim@b
        %
        %\expandafter\message{^^J%
        %       midshaft=\if@cd@centre@hlabel@ true\else false\fi,
        %       through=\if@cd@through@ true\else false\fi,^^J%
        %       natural  \the\cd@dim@a\space and  \the\wd\pending@right^^J%
        %       donated  \the\left@donated\space and  \the\right@donated}%
        %
        % if insufficient space on either side, set midshaft
        \ifdim\left@donated<\cd@dim@a\@cd@centre@hlabel@true\fi
        \ifdim\right@donated<\wd\pending@right\@cd@centre@hlabel@true\fi
        %
        % adjust right length for midshaft
        \if@cd@centre@hlabel@
                \right@donated\total@donated
                \advance\right@donated-\cd@dim@a
                \advance\right@donated\wd\pending@right
                %
                \ifdim\right@donated<2\wd\pending@right % not enough
                     \more@dim h\right@donated<2\wd\pending@right:%
                        arrow too short:\cd@cell\far@end@cell
                \fi
                %
                % give half of it to the right
                \divide\right@donated\tw@
                \left@donated\total@donated % don't need this
                \advance\left@donated-\right@donated
                %\expandafter\message{^^Jfinally
                %       \the\left@donated\space and \the\right@donated}%
        \fi
        %
        % if "through" expand left into right
        \if@cd@through@\kern-\right@donated\fi
        %
        \hbox to\right@donated{\unhbox\pending@right}%
        \math@off
}}%
%
%=======================================================================%
%                                                                       %
%       (10) PILES                                                      %
%                                                                       %
%=======================================================================%
%
%
% \hbox of cell containing \pile:
%       \glue(\hfil)
%       \mathon
%       \vbox
%               \hbox                   top line
%                   \glue\tabskip
%                   \hbox
%                   \glue\tabskip
%               \glue\baselineskip
%               \hbox                   second line
%               ...
%               \hbox                   bottom line
%       \penalty-9998
%       \rightskip                      added by paragraph builder
%       \mathoff                        from here is discarded
%       \glue(\hfil)
%
% uneven \pile separation, for example in
%      X & \pile{\rOnto^p\\\\\lInto~n\\\\\rTo_v} & Y
% because .5\PileSpacing is too little to accommodate the label ``n'',
% so \lineskip is used in the \vbox instead of \baselineskip.  
% Also, the empty line is
% \hss\kern\mathon\hfil\mathon\mathoff\kern\hss
%
%
%********************* phase 1 & 2 *****************************
%
% vertical position of pile?
% idea: optional argument to set width when outside diagram
% idea: get map labels and pass them to maps inside (eg adjunctions)
%
% It's not possible to catch a run-away argument to \pile.
% If we read it as an ordinary argument (#1), then if there is no matching
% closing brace anywhere before the end of the paragraph, the rest of the
% paragraph is lost and we get (a TeX error and) \par as the argument; this
% will expand to \enddiagram, which will at least close the \pile cleanly.
% On the other hand, if we do not read it as an argument, but leave the
% closing brace to TeX to parse later, it must end the \halign without giving
% us the opportunity to insert \crcr, and we can't regain control, because
% it is not possible to do \halign\bgroup\aftergroup.
%
% At various places we do \end@pile just in case the closing bracket has been
% put in too late. Since \pile{...\dTo...}\next translates into
% \begin@pile...\dTo...\end@pile\next we never see the original closing brace
% again, but \end@pile stands in for it. Since \dTo wants to force \end@pile,
% it inserts one and gives its own error message; the original becomes
% innocuous because (being no longer in the scope begun by \begin@pile) it is
% \empty. We choose this rather than \relax so that \\\enddiagram, which
% translates to \cr\end@pile\crcr\egroup, does not get an extra \cr.
% Perhaps these dummy \end@label and \end@pile commands should give error
% messages? Maybe, but it's quite likely that TeX or we have already given one.
% \let\end@label\empty
%
\new@if\ifinpile\inpiletrue\inpilefalse\inpilefalse
%
\def\pile{\protect\setup@pile\protect\@pile}%
\def\@pile#1{\begin@pile#1\end@pile}%
\def\setup@pile{%
\check@horiz{pile}%     % ensure correct horizontal state
\setbox0=\vtop\bgroup   % we want to know the height of the top level
\aftergroup\finish@pile % do this after the corresponding \egroup
%\incommdiagtrue                % signal we're NOT inside \commdiag
\inpiletrue
\let\group@after@map\empty
\let\pile\inner@pile    %
\let\end@pile\@end@pile %
\let\enddiagram@endpile\@enddiagram@endpile
\pile@state             % horiz state (\cd@donat) within \pile is either 6 or 7
\baselineskip.5\PileSpacing%
\lineskip.1\@em\relax   %
\lineskiplimit\lineskip %
\mathsurround\z@        % \m@th
\tabskip\z@             % \ialign
\let\\\pile@empty@row
}%
\def\begin@pile{%
\glet\last@map@type\empty% initialise horiz error message (27.12.93)
\halign\bgroup          % matrix of 1-column rows [\ifincommdiag\else to..\fi]
   \hfil
   \begin@maths
      \let\group@after@map\bad@group@after@map
      \let\\\pile@cr
      ##\end@label
   \end@maths
   \hfil
   \@and
   \and@in@pile##\cr% the template
}%
% idea: use second column to catch misplaced &
%
\new@help\help@and@in@pile{pile only allows one column.}%
\new@help\help@pile@enddiagram{you left it out!}%ascii
\def\and@in@pile{\end@pile\@and\relax
  \cd@error{missing \egroup@name\space inserted after \string\pile}%
  \help@and@in@pile}%
%
\def\@end@pile{\end@label\crcr\egroup\egroup}%
\def\enddiagram@endpile{\end@label}%
\def\@enddiagram@endpile{\end@label\relax\end@pile
   \cd@error{missing \egroup@name\space inserted between \string\pile\space
   and \end@diagram@name}\help@pile@enddiagram}%
%
% no point in warning about misplaced or anticipated \end@pile, because
% we've already got to that line and should have given some error message,
% since the argument to \pile is em-braced.
\def\end@pile{\end@label}%
%
% have the pile in \vbox0; do \vcenter without regard to outer labels
\def\finish@pile{%
\vbox  {\dimen1\dp0             % total height apart from this
        \unvbox0                % re-set \pile
        \setbox0=\lastbox       % get bottom layer
        \advance\dimen1\dp0     %
        \nointerlineskip
        \box0                   % restore bottom layer
        \nointerlineskip
        \setbox0=\null\dp0.5\dimen1\ht0-\dp0
        \box0}%                 % sink by half top-bottom axis distance
\ifincommdiag
\then   \penalty-9998           % flag this was a \pile
\fi
\xdef\last@map@type{pile}%
}%
%
% \\ inside \pile after some text
\def\pile@cr{\cr}%
%
% empty row in \pile (\\ at beginning of cell)
% fiddle the depth of the previous row
% to make \baselineskip or \lineskip do the work
\def\pile@empty@row{\noalign{%
   % this is really \advance\prevdepth-\baselineskip
   \skip@\prevdepth
   \advance\skip@-\baselineskip
   \prevdepth\skip@}}%
%
% Nested pile generates its own matrix in the same way, contributing the
% result to the main pile vertical list using \noalign (yes, this works).
%\def\inner@pile#1{\noalign\bgroup\begin@pile#1\end@pile}%
\def\inner@pile#1{#1}% I'm sure this will do!
%
% % \def\Atop#1#2{{%                     upper and lower parts
%   \setbox0\hbox{\strut\begin@maths#1\end@maths}\dp0\z@
%   \setbox1\hbox{\strut\begin@maths#2\end@maths}\ht1\z@
%   \vtop{\vbox{\kern-0.7ex\box0\hrule width\z@ height0.7ex depth0.93ex}
%     \nointerlineskip\box1}
% }}
% 
% The idea was to take apart (the definition of) the two arrows and
% re-assemble them. At the TeX end this wouldn't be very difficult to
% do, but it would have produced awful DVI (like visiting the houses
% in a street in numerical order, rather than going up the odds and down
% the evens). Experience has shown that all DVI drivers (it seems) are
% so careless with rounding DVI->pixel conversions that the result would
% be unspeakably ugly.
%
% \def\ExtractMapPartsA#1#2#3#4#5{%
% \def\mapA{#1}\def\tailA{#2}\def\headA{#3}\def\fillerA{#4}\def\middleA{#5}}
% \def\ExtractMapPartsB#1#2#3#4#5{%
% \def\mapB{#1}\def\tailB{#2}\def\headB{#3}\def\fillerB{#4}\def\middleB{#5}}
% 
% % eg "\ParallelMap\rTo\bot\lTo f g" or
% "\ParallelMap\uTo\adjoint\dTo f g" f-|g
% % \def\ParallelMap#1#2#3{%
% \expandafter\ExtractMapPartsA #1%     eg \rTo
% \setbox4=\hbox{\begin@maths#2\end@maths}%     middle bit, eg \bot or \adjoint
% \setbox5=\hbox{}\wd5=\wd4\ht5=\ht4\dp5=\dp4
% \expandafter\ExtractMapPartsB #3%     eg \lFrom
% \def\ke{\kern0.1\@em\copy5\kern0.1\@em}%
% \ifx\mapA\HorizontalMap\let\tbox\vcenter\else\let\tbox\hbox\fi
% \mapA{\tbox{\tailA\ke\tailB}}{\tbox{\headA\ke\headB}}%
%{\tbox{\fillerA\ke\fillerB}}
%{\tbox{\middleA\kern0.1\@em\box4\kern0.1\@em\middleB}}}
%
%
%********************* phase 4 *****************************
%
% \vbox\pending@left  contains the pile, as created by \halign above.
% \left@donated  is the required left width and \right@donated  the right width
% \total@donated is sum of these
% Result goes back in \box\pending@left . (\vcenter, \hbox or what?)
% \hbox3, \hbox4, \dimen0, \cd@dim@a, \skip0 scratch - local to \vbox
%
% When splitting the \vbox, we first put it on the stack (current vertical
% list) adding the following:
%       \penalty3 (stopper)
%       \hbox   (top map)
%       \baselineskip
%       ...
%       \baselineskip
%       \hbox (bottom map)
%
\def\widen@pile{%
\setbox\pending@left=\vbox{%
\unvbox\pending@left            % turn \vbox into a vertical list
\setbox1=\lastbox       % sinking box
\setbox0=\box\voidb@x   % accumulate new pile
%
\loop@on@maps % in the list
        \setbox\pending@left=\lastbox
\ifhbox\pending@left
        \do@pile@row
\repeat
\unvbox0                % put it back in the vertical list
\global\cd@dim@g\horiz@extra    % save extra cell width across closing braces
}%                      % complete \vbox
\horiz@extra\cd@dim@g}% % restore extra cell width
%
\def\do@pile@row{%
\if@cd@centre@hlabel@
        % unwrap box from \hbox{\tabskip\hbox{<-+->}\tabskip}
        \setbox\pending@left=\hbox{%
                \unhbox\pending@left
                \unskip
                \setbox\pending@left=\lastbox\unskip\unhbox\pending@left}%
        \ifdim\total@donated<\wd\pending@left 
                \more@dim h\total@donated<\wd\pending@left:%
                        arrow in pile too short:%
                        \cd@cell\far@end@cell
        \else   \setbox\pending@left =\hbox to\total@donated{\unhbox\pending@left}%
        \fi
\else   
        \split@pile@row
\fi
\setbox0=\vbox{% add the stretched row to the top of the completed pile
        \box\pending@left 
        \nointerlineskip
        \ifvoid0
        \then   \box1           % bottom layer - restore sinking box
        \else   \vskip\skip0    % restore interlayer glue
                \unvbox0
        \fi}%
\skip0=\lastskip\unskip % save \baselineskip above this row
}%
%
%  \box\pending@left =\hbox{
%       \tabskip
%       \hbox
%           (left part)
%           \penalty-9999
%           (right part)
%       \tabskip}
%
% Split each line of the pile, using the paragraph builder again, so
% the following is added to the stack (current vertical list):
%       FOR A MAP               FOR AN "OBJECT"
%       \parskip                \parskip
%       \baselineskip           \baselineskip
%       \hbox   (left part)     \hbox   (the object)
%       \baselineskip
%       \hbox   (right part)
%
%       \vbox0: completed pile
%       \box1   box to sink depth to do \vcenter without regard to labels
%       \hbox\pending@right : right part or object
%       \hbox\pending@left : row to be split, then left part, then result
%       \left@donated : the required left width
%       \right@donated : the required right width
%       \skip0: \baselineskip above it
%
\def\split@pile@row{%
\penalty7                       % mark the \parskip
\noindent
\unhbox\pending@left            % \tabskip\hbox\tabskip
\unskip                         % remove \tabskip
\setbox\pending@left=\lastbox   % get the \hbox (cell)
\unskip                         % remove \tabskip
\unhbox\pending@left            % split the box
\endgraf                        % using the paragraph builder
%
\setbox\pending@right=\lastbox\unskip% object or right part, and \baselineskip
\setbox\pending@right=\hbox{%
        \math@on
        \unhbox\pending@right
        \unskip\unskip\unpenalty % \parfillskip\rightskip\penalty10000
        }%
%
\ifcase\prevgraf\cd@shouldnt P% row of \pile contains wrong number of parts
%
% ONE line: a centered "object" between the maps
\or     \ifdim\total@donated<\wd\pending@right
                \more@dim h\total@donated<\wd\pending@left:%
                        object in pile too wide:%
                        \cd@cell\far@end@cell
                \setbox\pending@left =\hbox to\total@donated{\hss
                        \unhbox\pending@right
                        \hss}%
        \else
                \setbox\pending@left =\hbox to\total@donated{\hss
                        \kern\left@donated
                        \unhbox\pending@right
                        \kern\right@donated 
                        \hss}%
        \fi
%
% TWO lines: a map
\or     \setbox\pending@left=\lastbox\unskip  
                % get left part & discard \baselineskip
        \widen@horiz
                % re-set \hbox\pending@left using
                % \box\pending@right \right@donated
                % \box\pending@left  \left@donated  \total@donated
%
\else\cd@shouldnt Q\fi % row of \pile contains wrong number of parts
%
\unskip\unpenalty}% remove \parskip and marker (7)
%
%
%=======================================================================%
%                                                                       %
%       (11) VERTICALS                                                  %
%                                                                       %
%=======================================================================%
%
%
% idea: amount to fill? don't think it's worth the trouble
% at least ht & dp of other boxes
% idea: rotate text of labels
\def\exec@vert{%
\set@map@parts
\ifvoid3
        \setbox3=\null\ht3\axisheight\dp3-\ht3
        \dimen3.5\intended@breadth
\else   \dimen4\dp3
        \dimen3.5\wd3
        \setbox3=\make@vert@part{\box3}% re-center middle
        \dp3\dimen4                     % but preserve its depth
        \ifdim\ht3=-\dp3 \else\@cd@through@false\fi
\fi
%
\dimen0\dimen3                  % half original width of middle
\advance\dimen0-.5\intended@breadth
%
% attached labels to middle as overlaps
% preserving the size of \box3
% save widths for later phantom
\setbox0\null\ht0\ht3\dp0\dp3\wd0\wd3 % save size because we're reboxing
\ifvoid6\else
    \setbox6\hbox{\unhbox6\kern\dimen0\kern 2pt}\dimen0\wd6
\fi
\ifvoid7\else
    \setbox7\hbox{\kern 2pt\kern\dimen3\unhbox7}\dimen3\wd7
\fi
\setbox3\hbox{%
    \ifvoid6\else\kern-\dimen0\unhbox6\fi
    \unhbox3
    \ifvoid7\else\unhbox7\kern-\dimen3\fi
}%
\ht3\ht0\dp3\dp0\wd3\wd0
\if@cd@through@
        \dimen4=\ht\object@profile
        \advance\dimen4\dp5
        \advance\dimen4\dimen1  % lower tip plus shortfall
        \let\@fillb\empty       % lower filler is space
\else   \dimen4\ht3             % phantom middle
\fi
\setbox0\null
\ht0\dimen4
\offinterlineskip
%
\setbox8=\vbox spread2ex{%      % upper part with nominal extension
        \kern\dimen5            % shortfall above
        \box1                   % upper tip
        \@filla\vfill           % filler
        \if@cd@through@\else
            \kern\snake@        % user's adjustment
        \fi
        \box0}%                 % phantom middle provides baseline (depth zero)
        \ht8=\z@                % zero height so as not to force lines apart
\setbox9=\vtop spread2ex{%      % lower part with nominal extension
        \kern-\ht3              % top of box at baseline
        \kern-\snake@           % user's adjustment
        \box3                   % middle
        \@fillb\vfill           % filler [amount to fill?]
        \box5                   % lower tip
        \kern\dimen1}%          % shortfall below (\vbox would put \dp=0)
        \dp9=\z@                % zero depth so as not to force lines apart
%
\hskip\dimen0plus.0001fil       % phantom left label plus a tiny amount of glue
\box9                           % lower part
\kern-\intended@breadth         % backspace to overprint the two parts
\box8                           % upper part
\if@cd@centre@vlabel@\penalty2 \fi % code to say centre label vertically
\if@cd@through@\penalty1 \fi    % code to say filler goes through
\kern\PileSpacing               % code the locally required spacing
\kern-\PileSpacing              % and undo its effect
\kern-.5\intended@breadth       % centre penalty horizontally in shaft
\penalty\cd@penalty
\null
\kern\dimen3}%                  % phantom label (was \box7)
%
%
%********************* phase 3 *****************************
%
% \hbox\right@part  is rightmost, \hbox\left@part next,
% rest as lines of paragraph on current vertical list
% transfer them to \hbox\cd@donat
% calculate widths
%
% The format of each arrow \hbox is
%       \hfil
%       \mathon
%       \hbox(left label)
%       \kern
%       \vtop (lower part)
%       \kern (space adjustment)
%       \vbox (upper part)
%       \penalty2   \if@cd@centre@vlabel@ (midvshaft) 
%       \penalty1   \if@cd@through@ (filler goes through)
%       \kern\PileSpacing
%       \kern-\PileSpacing
%       \kern (space adjustment)
%       \penalty-9995
%       \rightskip
%
\def\reformat@vert{%
\ifhbox\cd@donat
        \cd@refmt@error{clashing verticals}%
        \ht\object@profile.5\dp\cd@donat
        \dp\object@profile-\ht5
        \complete@vertical
        \ht\object@profile\z@\dp\object@profile\z@
\fi
% save what will be our height
\dimen1\dp\cd@donat
%
% initialise accumulation of parts
\cd@num@d\prevgraf
\unvbox\cd@donat
\cd@num@c\lastpenalty\unpenalty % row number of top
\setbox\cd@donat=\null
%
% re-set rightmost part to natural width
%\setbox\right@part\hbox{\math@on\unhbox\right@part\math@off}% should be enough
\setbox\right@part =\hbox{%
        \math@on
        \unhbox\right@part 
        \unskip                 % \rightskip
        %\count@\lastpenalty    % code -9993
        \unpenalty
        %\setbox\junk\lastbox   % \hbox(right label)
        %\unkern                % 
        %\setbox\junk\lastbox   % \null
        \dimen0\lastkern\unkern % adjustment
        \unkern                 % un\PileSpacing
%\global\cd@dim@g\lastkern      % \PileSpacing
        \unkern
        \kern\dimen0            % replace adjustment
        \math@off
        }%
%
%
% and next-to-rightmost part, from which \rightskip and \penalty-9995
% have already been removed.
\setbox\left@part=\hbox{%
        \unhbox\left@part
        \dimen0\lastkern\unkern % adjustment
        \unkern                 % un\PileSpacing
\global \cd@dim@g\lastkern      % \PileSpacing
        \unkern
        \kern\dimen0            % replace adjustment
        }%
%
% copy all but leftmost & rightmost parts to donations box
\loop@on@maps
\ifnum  \cd@num@d>4
        \separate@verticals
\repeat
%
% remove \baselineskip and \parskip from vertical list
\unskip\unskip
%
% start by centering arrow system without regard to outermost parts
% (\left@width and \right@width initialised by \get@profile@info)
\advance\left@width.5\wd\cd@donat
\advance\left@width\wd\left@part
\advance\right@width.5\wd\cd@donat
\advance\right@width\wd\right@part 
%
% if this is the leftmost column of the diagram,
% remember how wide the system of verticals is (15.6.97)
\ifnum\cd@cell=\cd@left
    \cd@dim@a .5\wd\cd@donat
    \edef\vert@wd@in@leftmost{\the\cd@dim@a}%
\fi
%
% add outermost parts to donation, and codes for row numbers
\setbox\cd@donat=\hbox{%
        \kern-\left@width       % smash left width
        \box\left@part          % leftmost
        \unhbox\cd@donat        % middle
        \box\right@part         % rightmost
        \kern-\right@width      % smash right width
        \penalty\cd@num@c       % row number of top
        \penalty\cd@row}%       % row number of middle
%
% restore our height and depth, and the intercolumn width
\ht\cd@donat\dimen1
\dp\cd@donat\z@
\wd\cd@donat\column@placing
%
% use \left@width and \right@width  to obstruct horizontal
\complete@horizontal
}%
%
\def\separate@verticals{%
\ifdim\wd\left@part<\cd@dim@g
   \setbox\left@part=\hbox to\cd@dim@g{\math@on\unhbox\left@part}%
        % stretch to \PileSpacing apart
\fi
\advance\cd@num@d\m@ne
\setbox\cd@donat=\hbox{\box\left@part\unhbox\cd@donat}%
        % add back to donations box
\unskip                                 % remove \baselineskip
\setbox\left@part=\lastbox
\setbox\left@part=\hbox{%
        \unhbox\left@part
        \unskip                 % \rightskip
        %\count@\lastpenalty    % code -9995
        \unpenalty              %
        \dimen0\lastkern\unkern % adjustment
        \unkern                 % un\PileSpacing
\global \cd@dim@g\lastkern      % \PileSpacing
        \unkern
        \kern\dimen0            % replace adjustment
        }%
}%
%
%*************************** phase 4 ****************************
%
% Format of \box\cd@donat
%       either: space:  \vbox{  \penalty(row no. of upper obstruction)}
%       or:     arrows: \hbox{  \hbox(leftmost arrow)   -- see below
%                               ...
%                               \hbox(rightmost arrow)
%                               \hbox(right label)
%                               \penalty(row no. of upper obstruction)
%                               \penalty(row no. where declared)
%                               }
%
\def\complete@vertical{%
\dimen1\dp\cd@donat
\ifhbox\cd@donat
        \@complete@vertical
\else   \@complete@vspace
\fi
%
% make new space donation downwards
\setbox\cd@donat=\vbox{\penalty\cd@row}%save our row number
\dp\cd@donat-\dp\object@profile                         % amount of space
\wd\cd@donat\column@placing                       % intercolumn width to left
}%
%
\def\@complete@vspace{%
\unvbox\cd@donat
\cd@num@c\lastpenalty\unpenalty
\ifdim\dimen1<\ht\object@profile 
        \more@dim v\dimen1<\ht\object@profile:rows overprint:\cd@row\cd@num@c
\fi}%
%
\def\@complete@vertical{%
\dimen0=\ht\cd@donat    % height
%\dimen1=\dp\cd@donat   % depth
% vertical centering (questionable) - idea: make use of natural \ht & \dp
%\if@cd@centre@vlabel@
%        \advance\dimen0\dimen1
%        \dimen1.5\dimen0
%        \dimen0\dimen1
%\else  \cd@dim@b\z@
%\fi
%
\setbox\cd@donat=\hbox\bgroup
        \advance\dimen1-\ht\object@profile  %### forgot this in centre@vlabel!
        \unhbox\cd@donat
        \cd@num@d\lastpenalty\unpenalty % row number of middle
        \cd@num@c\lastpenalty\unpenalty % and of top
\global \cd@dim@h-\lastkern\unkern      % right width (local to \hbox)
        \setbox0=\lastbox               % right label (don't touch)
%
        \loop@on@maps
                \setbox\cd@donat=\hbox{\box0\unhbox\cd@donat}%
                \setbox0=\lastbox
        \ifhbox0
                \stretch@vert
        \repeat
\global \cd@dim@k-\lastkern\unkern      % left width
\global \cd@dim@g\vert@extra            % save extra cell height across \egroup
        \unhbox\cd@donat
\egroup
\vert@extra \cd@dim@g                   % restore extra cell height
\output@cell{\cd@dim@k}{\box\cd@donat}{\cd@dim@h}{\dimen1}}%
%
% local to \hbox:
% \hbox0:  upper part
% \dimen0: required height of upper part, depth \dimen2
% \hbox1:  lower part
% \dimen1: required depth of lower part, height \dimen2
% \dimen2: adjustment for midvshaft
% \dimen7: right adjustment
% \dimen6: left adjustment
%
\def\stretch@vert{%
\setbox0=\hbox to\wd0\bgroup
\unhbox0
\unskip\unpenalty       % \rightskip, \penalty-9995
\dimen7\lastkern\unkern % right adjustment
\ifnum  \lastpenalty=1
        \unpenalty
        \@cd@through@true
\else   \@cd@through@false
\fi
\ifnum  \lastpenalty=2
        \unpenalty
        \dimen2.5\dimen0\advance\dimen2-.5\dimen1\advance\dimen2-\axisheight
\else   \dimen2\z@
\fi
\setbox0=\lastbox       % upper part
\dimen6\lastkern\unkern % left adjustment
\setbox1=\lastbox       % lower part
%
% stretch upper part (\dp\z@ since ends in \hbox\dp\z@ or \kern)
\setbox0=\vbox{%
        \unvbox0
        \if@cd@through@
             \kern-\dimen1   % for filler to go through
        \else\ifdim\dimen2=\z@\else
             \kern\dimen2    % for midvshaft
        \fi\fi}%
\ifdim\dimen0<\ht0
        \more@dim v\dimen0<\ht0:upper part of vertical too short:%
                {\if@cd@through@\cd@row\else\cd@num@c\fi}\cd@num@d
\else   \setbox0=\vbox to\dimen0{\unvbox0}%
\fi
%
% stretch lower part
% NB (see TeXbook p81)
% \vbox would make \dp=0 (because ends \kern\MapShortFall) so \ht=total;
% but \vtop makes \ht=0 (because begins \box), so \dp=total.
\setbox1=\vtop{\unvbox1}%
\ifdim\dimen1<\dp1
   \more@dim v\dimen1<\dp1:lower part of vertical too short:\cd@row\cd@num@c
\else   \setbox1=\vtop to\dimen1{%
        \ifdim\dimen2=\z@\else
             \kern-\dimen2
        \fi
        \unvbox1
        }%
\fi
%
\box1                   % put lower part back
\kern\dimen6            % left adjustment
\box0                   % upper part
\kern\dimen7            % right adjustment
\math@off
\global\cd@dim@g\vert@extra     % save extra cell height neede across \egroup
\egroup                 % end of \hbox
\vert@extra\cd@dim@g\relax}%    %
%
%
%=======================================================================%
%                                                                       %
%       (12) TRANSFER TO BOX ARRAYS                                     %
%                                                                       %
%=======================================================================%
%
% TeX has 256 boxes, some (not, in fact, very many) of which are allocated
% (using \newbox and \newinsert)
% for specific purposes by plain.tex, latex.tex and other packages, including
% this one. Those from 10 to \boxc@unt have been allocated by \newbox and
% those from \insc@unt to 255 by \newinsert, but most of them are unused.
% We use those in between, allocated locally, as a scratch array for our
% reformatting. (\box0..\box9 are also used for scratch). By convention,
% the pointer to the loweset-numbered box in an allocation is to that box,
% whilst that to the highest is to the one above.
%
\countdef\boxc@unt=14 % [cf \insc@unt] number of last \box allocation
%
% \box0..9                                      available as scratch
% 10..\boxc@unt                                 allocated to various packages
% \cd@bottom=\boxc@unt+1..\cd@top-1             used for rows of matrix
% \cd@left@donat=\cd@top..\cd@right@donat       used for vertical donations
% \cd@right@donat+1..\cd@left-1                 unused
% \cd@left..\cd@right-1                         used for cells of current row
% \insc@unt=\cd@right..254                      allocated for footnotes etc
% 255                                           is the current page
%
\newcount\cd@bottom     % \box\cd@bottom is the bottom row
\newcount\cd@top        % \box{\cd@top-1} is top row
\newcount\cd@row        % \box\cd@row is current row
\let\cd@right\insc@unt  % \box{\cd@right-1} is rightmost cell of current row
\newcount\cd@cell       % \bot\cd@cell is current ditto
\newcount\cd@left       % \bot\cd@left is leftmost ditto
\let\cd@left@donat\cd@top% \box\cd@left@donat is leftmost vertical donation
%\cd@donat already defd % \box\cd@donat is current ditto
\newcount\cd@right@donat% \box{\cd@right@donat-1} is rightmost ditto
%
% After each row has been reformatted and output, its height \ht\cd@row
% is set to the current value of \completed@depth, ie the distance from
% the top of the diagram. (10.7.94)
%
% This is called just after we've finished building the vertical list
% which comprises the matrix. The rows of the matrix may be extracted
% one by one in reverse order (with glue between them), and then each
% row is similarly decomposed, also in reverse order.
% At the beginning this vertical list looks like this:
%          \penalty-123  % marker placed by \diagram
%          \hbox        % top row
%               \glue\tabskip
%               \hbox   % leftmost cell (see template and maps for format)
%               \glue\tabskip
%               \hbox   % second cell
%               ...
%               \glue\tabskip   
%               <<<<<<<<<<<<<<<<<<<<< \reformat@row is called here
%          \penalty 1   % code that this is a row, mot a missive
%          \glue\baselineskip
%          \hbox        % second row
%          \penalty 1   % code that this is a row, mot a missive
%          \glue\baselineskip
%          ...
%          \hbox        % bottom row
%          <<<<<<<<<<<<<<<<<<<<<<<<<< \reformat@matrix is called here
%
% reformatting goes from right to left in each row,
% top row to bottom row.
%
% IDEAS:
%  -    collect overprints and diagonals, adding them to the left of the
%       appropriate row boxes (making new ones void first if necessary)
%  -    similar use column widths to set vertical donations (as \wd\vbox)
%       void boxes for unspecied ones and warning for repeated specification
%
% MISSIVES:
% \vadjust{} called within a cell puts its material into the vertical list
% below the row (so it appears to \lastbox, \lastpenalty, etc before the row).
% Instead of the \hbox\penalty1 of the row, this is encoded as follows:
%           \hbox{missive material}
%           \penalty (column number; 1=leftmost)
%           \penalty (row number; 1=topmost)
%           \penalty (missive code number, >1)
% The missive material may contain overprints, diagonals, etc.  In the case of
% diagonals, the row and column numbers are those of the upper (and, for
% horizontals, leftmost) cell involved; the other end of the arrow is
% encoded as penalties contained in the missive material.
%
% \missive@to@row is called when such a \penalty is found whilst the vertical
% list produced by \halign is being taken apart. It appends the missive to the
% left of the \hbox containing the row to which it is addressed in the format
%           \hbox{missive material}
%           \penalty (column number)
%           \penalty (missive code)
% \missive@to@cell is called whilst the row \hbox is being taken apart.
% It appends the missive to the left of the cell \hbox in the format
%           \hbox{missive material}
%           \penalty (missive code)
%
%********************* transfer rows of matrix to array **********************
%
\new@if\if@reformatting@\@reformatting@true\@reformatting@false\@reformatting@false
%
\def\firstpass@showboxdepth{-1}%
%
\def\after@diagram{%
\ifnum\firstpass@showboxdepth<\z@\else % 15.7.94
    \begingroup
       \scrollmode % 17.7.94 %%% but this is now set globally 16/4/95
       \showboxdepth\firstpass@showboxdepth
       \showboxbreadth\maxdimen
       \showlists
    \endgroup
\fi
\@reformatting@true
\make@end@at@line
\cd@bottom=\boxc@unt            % allocate array from \boxc@unt upwards
\advance\cd@bottom1             % for bottom and other rows of matrix
\cd@top=\cd@bottom              %
% during the first pass, we counted the rows (globally) in \cd@row
% if only one row, center the labels on the horizontal maps 12.7.94
\ifnum\cd@row=1 \@cd@centre@hlabel@true\fi
\advance\cd@top\cd@row          % top
\dimen1\z@                      % height of previous row
\skip0\z@                       % interline space below this row
\count@=\insc@unt
\advance\count@\boxc@unt
\divide\count@2                 % greatest register which may be used for rows
%\showboxdepth999\showboxbreadth999%\showlists
%
\ifnum\cd@top>\count@
    \cd@refmt@error
     {The diagram has too many rows! It can't be reformatted.}%ascii
\else
    \matrix@to@buffer  % rows in boxes, collect diagonals, etc (easy to abort)
    \reformat@matrix   % re-align (skip this for draft mode?)
\fi
\output@diagram
}%
%
\def\matrix@to@buffer{%
\cd@row\cd@bottom
\loop@on@rows                   % clear rows
\ifnum\cd@row<\cd@top % 12.7.94
        \setbox\cd@row\box\voidb@x
        \advance\cd@row 1\relax
\repeat
%
\cd@row\cd@bottom
\skip\z@\z@ % inter-row glue
\loop@on@rows
        \cd@penalty\lastpenalty\unpenalty % get the code
\ifnum\cd@penalty>\z@           % is anything there?
        \handle@matrix@row
\repeat
%
\ifnum  \cd@penalty=-123        % We inserted this check at the beginning
\then   \unpenalty              %  of \diagram; now remove it.
\else   \cd@shouldnt D% failed to unpack all of the rows of the matrix
\fi
%
% set row heights from grid
\ifx\v@grid\relax\else
   \cd@row\cd@top\advance\cd@row\m@ne
   %\tracingcommands1 \tracingmacros1
   \expandafter\set@v@grid\v@grid
   %\tracingcommands0 \tracingmacros0
\fi
%
%\cd@left@donat=\cd@top%(\let)  % initialise donations buffer
\cd@right@donat\cd@left@donat   %
\column@placing\z@
\mk@new@donat
%
% set column widths from grid
\ifx\h@grid\relax\else
   %\tracingcommands1 \tracingmacros1
   \expandafter\set@h@grid\h@grid
   %\tracingcommands0 \tracingmacros0
\fi
%
\count@\cd@top
\advance\count@\m@ne
\cd@top@height\ht\count@
%\expandafter\message{left=\the\cd@left, right=\the\cd@right,
%   left donat=\the\cd@left@donat, right donat=\the\cd@right@donat}%
}%
%
\def\handle@matrix@row{%
\ifcase\cd@penalty
\or     \matrix@row@to@buffer
\else   \cd@num@a-\lastpenalty\unpenalty % negative of row number
        \cd@num@b\lastpenalty\unpenalty % column number
        \setbox0=\lastbox
        \missive@to@row
\fi
\get@interrow@glue % 13.7.94
}%
\def\get@interrow@glue{\skip1\lastskip\unskip\advance\skip0\skip1
\ifdim\skip1=\z@\else\expandafter\get@interrow@glue\fi}%
%
\def\matrix@row@to@buffer{%
\setbox0=\lastbox       % get a row
\row@depth\dp0
\advance\row@depth\skip\z@\skip\z@\z@
\advance\inter@row\row@depth    % between our baseline and next below
\if@cd@tight@\ifnum\cd@row>\cd@bottom
        \inter@row\DiagramCellHeight    % if tight, reset to prescribed amount
        \row@depth\inter@row
        \advance\row@depth-\row@height
\fi\fi
\row@height\ht0         % save height for next time
\inter@row\row@height
% save the row on the left hand end of the row box register
\setbox\cd@row\hbox{\unhbox\cd@row\unhbox0}%
\dp\cd@row\row@depth                  % include space in depth of row
\ht\cd@row\row@height
\advance\cd@row 1       % allocate a box register for it
}%
%
\def\missive@to@row{%
% \cd@num@a = -1 for top row, -2 for next, etc
%\expandafter\message{missive type \the\cd@penalty\space to
%   (\the\cd@num@a,\the\cd@num@b)}%
\ifnum\cd@num@a<\z@
   \advance\cd@num@a\cd@top % row number as a box number
   \ifnum\cd@num@a<\cd@bottom
        \missive@outside
   \else
        \cd@dim@a\dp\cd@num@a\cd@dim@b\ht\cd@num@a
        \setbox\cd@num@a\hbox{%
            \box\z@
            \penalty\cd@num@b
            \penalty\cd@penalty
            \unhbox\cd@num@a}%
        \dp\cd@num@a\cd@dim@a\ht\cd@num@a\cd@dim@b
   \fi
\else
    \missive@outside
\fi
}%
\def\missive@outside
{\cd@refmt@error{diagonal goes outside diagram (lost)}}%ascii
%
\def\resend@missive{%
%\expandafter\message{missive type \the\cd@penalty\space to
%   (\the\cd@num@a,\the\cd@num@b)}%
\advance\cd@num@a\cd@top % row number as a box number
\ifnum\cd@num@a<\cd@bottom
    \missive@outside
\else
    \ifnum\cd@num@a=\cd@row
        \missive@to@cell
    \else
        \ifnum\cd@num@a>\cd@row
            \cd@shouldnt M% missive addresses in wrong order
        \else
            \cd@dim@a\dp\cd@num@a\cd@dim@b\ht\cd@num@a
            \setbox\cd@num@a\hbox{%
                \box\z@
                \penalty\cd@num@b
                \penalty\cd@penalty
                \unhbox\cd@num@a}%
            \dp\cd@num@a\cd@dim@a\ht\cd@num@a\cd@dim@b
\fi\fi\fi
}%
%
% State of program variables at point of loop test
%   current vertical list: completed diagram so far
%   \cd@row still points to row above
%   \hbox(\cd@row-1): current row as illustrated above
%   \completed@depth= vertical distance from top of matrix to next baseline
%                above
%   \inter@row := depth of next row above
%
%********************* reformat matrix **********************
%
\def\reformat@matrix{%
%\matrix@to@buffer      % already have each row in a separate box register
\bomb@parameters        % set up for our peculiar use of paragraph builder
\set@axis               % profile height & depth for empty cells
\setbox\default@profile =\hbox{\begin@maths A\@super f\@sub f\end@maths}%
                % object not to profile
\horiz@extra \z@\vert@extra \z@ % extra horizontal & vertical cell size needed
\right@over \z@\left@over \z@   % right and left widths of whole diagram
\cd@row=\cd@top         % start from top row
\inter@row \z@\completed@depth \z@      % row and total depth
%
\loop@on@rows
\ifnum  \cd@row>\cd@bottom
        \advance\cd@row\m@ne
        \row@height \ht\cd@row  % save height of row
        \row@depth \dp\cd@row   % and depth
        \advance\inter@row \row@height  % distance to next baseline
        \row@to@buffer          % new vertical donations are down to next above
        \advance\completed@depth \inter@row     % depth so far
        \deepen@donations       % add depth to donations
        \reformat@row
        \buffer@to@row          % collect completed cells
        \ht\cd@row\row@height   % restore height of row
        \dp\cd@row\row@depth    % and depth
        \nointerlineskip        %
        \box\cd@row             % output the completed row to the vertical list
        \inter@row \row@depth   % depth contributes to dist to next baseline
        \setbox\cd@row\null     % 10.7.94
        \ht\cd@row\completed@depth % 10.7.94
\repeat % loop on rows
%
\complete@last@row
\nointerlineskip
\box\cd@row             % output it
%
\need@extra\horiz@extra\DiagramCellWidth{width}%
\need@extra\vert@extra \DiagramCellHeight{height}%
%
% do some calculations to pass to \output@diagram
\cd@donat\cd@right\advance\cd@donat-\cd@left\advance\cd@donat\m@ne
\advance\cd@donat\cd@left@donat
\dimen0\wd\cd@donat % position of rightmost column
%
\rule@height \axisheight                                % axis height
\dimen1\completed@depth \advance\dimen1-\cd@top@height  % top to bottom axis
\dimen2\right@over \advance\dimen2-\dimen0      % right width of right column
\advance\cd@top-\cd@bottom                      % number of rows
\advance\cd@right-\cd@left                      % number of columns
}%
%
%
\count@\year\multiply\count@12 \advance\count@\month
\ifnum\count@>24314 \loop\iftrue\message{gone February 2026!}\repeat\fi% 
%
% \inter@row is now the depth of the bottom row (according to \halign)
\def\complete@last@row{%
\row@height-\inter@row
\row@depth\inter@row
\setbox\object@profile=\null
\dp\object@profile\inter@row
\ht\object@profile-\inter@row
\left@width\z@
\right@width\z@
\cd@left\cd@right
\advance\cd@left-\cd@right@donat
\advance\cd@left\cd@left@donat
\cd@cell\cd@right
\cd@donat\cd@right@donat
\loop@on@cells
\ifnum  \cd@cell>\cd@left
        \advance\cd@cell\m@ne
        \advance\cd@donat\m@ne
        \column@placing\wd\cd@donat
        \setbox\cd@cell=\box\voidb@x
        %\showbox\cd@donat
        \complete@vertical
        %\showbox\cd@cell
\repeat
\buffer@to@row%\showbox\cd@row
\ht\cd@row\row@height
\dp\cd@row\row@depth
}%
%
\def\need@extra#1#2#3{%
\ifdim#1>.01\@em
        \cd@dim@b #2\relax
        \advance\cd@dim@b #1\relax
        \advance\cd@dim@b.99\@em
        \count@\cd@dim@b
        \divide\count@\@em
        \cd@refmt@error{increase cell #3 to \the\count@ em}%
\fi}%
%
%
%********************* transfer cells of row to array **********************
%
% IDEAS
%  -    ignore \tabskip; shouldn't be any other glue penalties or kerns in row
%  -    diagonal and overprint items? somehow append to cells. what it past
%       end of row?
%  -    what about orphan diagonals?
\def\row@to@buffer{%
% have \cd@right=\insc@unt
\cd@cell=\cd@right      % clear array for cells to be processed
%\count@=\cd@right
%\advance\count@\cd@left@donat
%\divide\count@2        % lowest register allowed for cells
\penalty4               % mark the following \parskip
\noindent\unhbox\cd@row % make horizontal list (adds \parskip to vertical list)
%
% get the actual cells from the right hand side of \box\cd@row
\loop@on@cells
        \unskip                 % remove \tabskip
        \setbox0=\lastbox       % get next (to left) cell
\ifhbox0                        % anything there?
        \advance\cd@cell\m@ne
        \setbox\cd@cell\hbox to\wd0{\null\penalty-9990\null\unhbox0}%
%       \ifnum\cd@cell>\count@\else
%               \cd@refmt@error{Too many cells.}%
%               \cd@cell=\cd@right      % throw most of them away
%       \fi
\repeat
\cd@left\cd@cell%\expandafter\message{cd@left=\the\cd@left}%
%
\advance\cd@cell\cd@right@donat % 
\advance\cd@cell-\cd@left@donat % cell corresponding to possible new donation
\ifnum\cd@cell<\cd@right        % is this row longer than the donations?
        \count@\cd@cell
        \advance\count@\m@ne    % NB: was already at least one donation column
        \dimen0=\wd\count@      % width of previous halign column
        \count@\cd@right@donat
        \advance\count@\m@ne
        \column@placing\wd\count@ % x-coord of previous donation col
        \loop@on@cells
        \ifnum  \cd@cell<\cd@right
                \set@col@width
                \mk@new@donat
                \dimen0\wd\cd@cell      % width of this column for next time
                \advance\cd@cell 1
        \repeat
\fi
%
% then the missives
\loop@on@cells
        \cd@penalty\lastpenalty\unpenalty
\ifnum\cd@penalty>\z@
        \cd@num@b\lastpenalty\unpenalty % column number
        \missive@to@cell
\repeat
%
%
\endgraf                % make paragraph from empty horizontal list
\unskip                 % remove \parskip glue
        \ifnum\lastpenalty=4    % check we have the correct stopper
\unpenalty
        \else
        \cd@shouldnt S% didn't clear the stack
        \fi
}%
\def\missive@to@cell{%
%\expandafter\message{missive type \the\cd@penalty\space to
%   (\the\cd@num@a,\the\cd@num@b) cd@left=\the\cd@left}%
%\ifnum\cd@num@b<\z@
%   \missive@outside
%\else
   \advance\cd@num@b\cd@left\advance\cd@num@b\m@ne
   \setbox0=\lastbox
   \ifnum\cd@num@b<\cd@right
        \setbox\cd@num@b\hbox{\box0\penalty\cd@penalty\unhbox\cd@num@b}%
   \else
        \missive@outside
\fi%\fi
%\showboxdepth 2 \showboxbreadth 999 \tracingonline1 \showbox\cd@num@b
}%
%
% extend donations to be at least as long as row
% calculate and save column widths here
\def\more@donations{%
}%
%
\new@if\if@cd@tight@\@cd@tight@true\@cd@tight@false
%
\def\set@col@width{%
        % calculate halign's distance between centres
        \advance\dimen0\wd\cd@cell
        \divide\dimen0\tw@
        %
        % impose required size
        \if@cd@tight@
                \dimen0\DiagramCellWidth
        \else   \at@least{\dimen0}\DiagramCellWidth
                \test@loose@diagonals
        \fi
        %
        \advance\column@placing\dimen0
}%
\def\mk@new@donat{%
% make new vertical donation
\setbox\cd@right@donat=\vbox{}%         % new space donation
\dp\cd@right@donat=\completed@depth     % of the depth so far
%
% accumulate and save x-coordinate
\wd\cd@right@donat\column@placing
%\expandafter\message{^^Jcol \the\cd@right@donat\space at \the\column@placing}%
\advance\cd@right@donat 1
}%
%
\def\set@h@grid#1,{%
   \def\@value{#1}%
   \ifx\@value\end@square@name\else
      \advance\column@placing\@value\DiagramCellWidth
      \mk@new@donat
      \expandafter\set@h@grid
   \fi
}%
%
\def\set@v@grid#1,{%
   \def\@value{#1}%
   \ifx\@value\end@square@name\else
      \ifnum\cd@row>\cd@bottom
         \inter@row\@value\DiagramCellHeight
         \advance\inter@row-\dp\cd@row
         \advance\cd@row\m@ne
         \ht\cd@row\inter@row
      \fi    % 4.12.94
      \expandafter\set@v@grid
   \fi
}%
%
%
% If diagonals have been used and we're widening a column by more
% than twice the short-fall, tell the user to use the tight option.
%
\def\test@loose@diagonals{%
\if@diagonals@used@
        \cd@dim@a\dimen0
        \advance\cd@dim@a-\DiagramCellWidth
        \ifdim\cd@dim@a>2\MapShortFall
           \cd@refmt@error{badly drawn diagonals (see manual)}%ascii 15.4.95
           \let\test@loose@diagonals\empty
        \fi
\else   \let\test@loose@diagonals\empty
\fi}%
%
\def\deepen@donations{%
\cd@donat\cd@left@donat
\loop@on@cells
\ifnum\cd@donat<\cd@right@donat
        \dimen0\dp\cd@donat
        \advance\dimen0\inter@row 
        \dp\cd@donat\dimen0
        \advance\cd@donat 1
\repeat
}%
% outside:
%   \cd@dim@a: left width
%   \left@over :  left overlap of diagram
%
% local to \hbox:
%   \box0:   what we're going to print
%   \dimen7: distance to raise
%   \dimen8: right width
%   \dimen9: kern between thing on left and us
%
% may be used as arguments:
%   \dimen1,3,4,5 \z@ \box2,7 \box\cd@donat
%
\def\output@cell#1#2#3#4{% #1=left width, #2=box, #3=right width, #4=raise
\ifnum\cd@cell<\cd@right
        \cd@dim@a=#1\relax
        \setbox\cd@cell=\hbox{%
                \setbox0=#2%
                \dimen7=#4\relax
                \dimen8=#3\relax
%\expandafter\message{^^J(\the\cd@top-\the\cd@row,\the\cd@cell-\the\cd@left)
%       \the\cd@dim@a, \the\dimen8, pos=\the\column@placing}%
                \ifhbox\cd@cell
                        \unhbox\cd@cell
                        \advance\cd@dim@a-\lastkern\unkern
                \fi
                \ifdim\cd@dim@a=\z@\else\kern-\cd@dim@a\fi
                \raise\dimen7\box0
                \kern-\dimen8
                }%
        \ifnum\cd@cell=\cd@left\at@least\left@over\cd@dim@a\fi
\else   \cd@shouldnt O% \output@cell has overrun the buffer
\fi
}%
%
\def\buffer@to@row{%
\setbox\cd@row=\hbox{%
\cd@cell\cd@left
\cd@donat\cd@left@donat
\cd@dim@b\z@\relax % total width so far
\loop@on@cells
\ifnum\cd@cell<\cd@right
        \column@placing\wd\cd@donat\relax
        \reoutput@cell
        \advance\cd@cell 1
        \advance\cd@donat 1
\repeat}%
\at@least\right@over{\wd\cd@row}% greatest width so far
\wd\cd@row\z@ % kill it (we'll deal with positioning at the end)
}%
%
\def\reoutput@cell{%
\ifhbox\cd@cell
        \cd@dim@a\column@placing\relax
        \advance\cd@dim@a-\cd@dim@b\relax
        \ifdim\cd@dim@a=\z@\else\kern\cd@dim@a\fi
        \cd@dim@b\column@placing
        \advance\cd@dim@b\wd\cd@cell\relax
        %\box\cd@cell % commented out 6.4.95 why was it there? R width ok now
        \unhbox\cd@cell
        \advance\cd@dim@b-\lastkern\unkern
\fi
}%
%
%************************ re-alignment of row ***********************
%
% State of program variables at loop test:
%   current vertical list: completed rows of diagram
%   \cd@cell still points to cell to right!
%   \hbox(\cd@cell-1) current cell, still as packaged by \halign
%   \hbox(\cd@left..\cd@cell-2) cells still to be processed
%   \hbox(\cd@cell..(\cd@right-1)) completed row so far
%   \box\cd@donat vertical donation:
%       width is horizontal distance from centre of leftmost column to this one
%       \vbox: space donation, depth is amount (height undefined)
%       \hbox: pending vericals, height and depths according to their baseline
%   \cd@dim@a,0,6 scratch
%   \completed@depth  = depth of completed diagram so far to current baseline
%   \inter@row  = distance from current baseline to next above
%   \column@placing  = dist from centre of first column to centre of this one
%   \left@donated  = width of left part or of horizontal donation from right
%   \row@height  = height of this row
%   \row@depth  = depth of this row
%   \hbox\pending@left   = horizontal donation:
%       void:  space donation of \left@donated 
%       \hbox: left part of single horizontal (not re-set) \wd is of right part
%       \vbox: pile (not re-set)                                ditto
%   \hbox\pending@right   = right part of single horizontal (or void)
%
\def\reformat@row{%
\setbox\pending@left=\box\voidb@x % horizontal donation is space
\cd@donat=\cd@right@donat       % index into buffer of vertical donations
\cd@cell\cd@right               % index into buffer of cells to be processed
\cd@donat\cd@left@donat
\advance\cd@donat\cd@cell
\advance\cd@donat-\cd@left      % corresponding donation
\advance\cd@donat\m@ne
\column@placing \wd\cd@donat    % save
\count@\cd@right                % unterminated horizontals on right
\advance\count@\m@ne            % extend to the edge of the column as
\left@donated .5\wd\count@      % set by \halign
\advance\left@donated\column@placing
\across@cells\m@ne              % no \span'ned columns on right
\far@end@cell\@m
%
\loop@on@cells % of donations buffer
\ifnum  \cd@cell>\cd@left
        \advance\cd@cell\m@ne
        \advance\left@donated-\column@placing
        \reformat@cell
        \wd\cd@donat\column@placing      % restore
        \advance\left@donated \column@placing
                        % add intercolumn to horizontal donation
        \advance\cd@donat\m@ne
        \column@placing \wd\cd@donat    % save
\repeat % loop on cells
%
\left@width\left@over \right@width -\left@width
% zero-width column shifted this much
\complete@horizontal            % output remaining unterminated arrow
}%
%
%********************* add to left or right of box **********************
%
%\def\push@queue#1\to#2{% *** push \box#1 onto (left of) queue \hbox#2 ***
%\setbox#2=\hbox{\box#1\unhbox#2}}%
%
%\def\push@stack#1\to#2{% *** push \box#1 onto (right of) stack \hbox#2 ***
%\setbox#2=\hbox{\unhbox#2\box#1}}%
%
% The above was originally implemented so that \box'es could be used
% as stacks and queues. This is, however, probably very time-consuming.
% \def\p@p#1\from#2{% *** pop \box#1 from stack \hbox#2 ***
% \setbox#2=\hbox{%
%       \unhbox#2
%       \setbox#1=\lastbox
%       \vadjust{\box#1}%       migrates to enclosing vertical list
%       }%
% \setbox#1=\lastbox}%          where we pick it up
% Note that this ONLY works if the enclosing list is vertical; otherwise
% no migration occurs at all (ie it doesn't go into a list further out).
%
%
%=======================================================================%
%                                                                       %
%       (13) PARAGRAPH BOMBING                                          %
%                                                                       %
%=======================================================================%
%
% The paragraph builder works inside any vertical list --- not just the
% current page --- and all we need to do to invoke it is to create a
% horizontal list and terminate it with \endgraf. The horizontal list is
% split into a sequence of \hbox'es delimited by \penalty's and \glue.
% The effect of
%       "\noindent\unhbox6\unksip\endgraf"
% is to add
%       \glue\parskip           [absent if current vertical list is empty]
%       \glue\baselineskip      [absent if \prevdepth<=-1000pt]
%       \hbox(first line)
%               [\hbox(\parindent) absent because of \noindent]
%               \glue\hfil
%               \mathon
%               (first part of \hbox6 up to and including
%               \penalty-9999   % whatever we used to force a split)
%               \glue\rightskip
%       [\penalty\clubpenalty absent because all interline penalties=0]
%       \glue\baselineskip
%       \hbox(sencond line)
%       [\penalty\interlinepenalty]
%       ...
%       \glue\baselineskip
%       \hbox(penultimate line)
%               (last part of \hbox6, up to \penalty-9993\rightskip)
%       [\penalty\widowpenalty absent because all interline penalties=0]
%       \glue\baselineskip
%       \hbox(last line)
%               [\mathoff\glue\hfil lost in line break]
%               \null protection
%               [\penalty profile code]
%               \kern-2\cd@hshift
%               \penalty10000
%               \glue\parfillskip
%               \glue\rightskip
%               \null protection
% to the current vertical list, where the number of lines is returned in
% \prevgraf.
%
% Note that \endgraf is defined (TeXbook p351) to be the primitive value of
% \par;  LaTeX changes \par quite a lot.
%
% We take advantage of this as a way of splitting a complex \hbox (containing
% \mathon...\mathoff whatsits, which there is no way of stripping) at any
% desired place. For example, we want to divide a horizontal arrow in two
% and stretch the two parts by different amounts.  By using peculiar
% parameters we can get this to happen at the desired places and not at the
% usual hyphenation.  In particular, we set \linepenalty=9000, so splitting
% can only occur at large negative penalties.
%
% We use particular penalty values as codes:
%       -9999:  middle of horizontal arrows
%       -9998:  after \pile (immediately preceded by the \vbox)
%       -9997:  \HonV
%       -9996:  \VonH
%       -9995:  middles of vertical arrows (immed. prec. by two \vbox'es)
%       -9994:  \HmeetV
%       -9993:  \end@cell, followed by profiling info
% Hence the number of lines is
%       ZERO:   empty cell (only \parskip added to vertical list)
%       ONE:    unused - maybe use for \HonV and \VonH
%       TWO:    object
%       THREE:  any of above five cases
%       MORE:   two or more parallel vertical arrows
%
% The effect of this is to add extra \hbox'es to the vertical list, which
% we then strip off in reverse order.  In other words, we use the vertical
% list as a stack (and refer to it as such).
%
% CONVENTION
%       Since most of the glue and penalties on the stack are unwanted,
%       whenever they are wanted they are removed immediately they come
%       to the top of the stack.
%
% bomb to split horizontal and vertical arrows
\newcount\cd@penalty
\def\@bomb{}% no bombs outside diagrams
%
\def\bomb@parameters{%
\mathsurround         \z@       % no extra space around maths
\hsize                \z@       % zero-width paragraphs,
\rightskip            \z@       % \ but allow
                 plus1fil       % | to stick out
           minus\maxdimen       % / on the right
\parfillskip          \z@       %
\linepenalty         9000       % use only one line unless high price paid
\looseness              0       % no extra lines
\hfuzz          \maxdimen       % don't care how much it sticks out,
\hbadness           10000       % so please don't complain about it!
\clubpenalty            0       % \
\widowpenalty           0       % | set all inter-line penalties to
\displaywidowpenalty    0       % | zero so that they are suppressed
\interlinepenalty       0       % |
\predisplaypenalty      0       % |
\postdisplaypenalty     0       % |
\interdisplaylinepenalty  0     % |
\interfootnotelinepenalty 0     % |
\floatingpenalty        0       % |
\brokenpenalty          0       % /
\everypar               {}%     % no junk at beginning of paragraph
\leftskip             \z@       % or beginning of lines
\parskip              \z@       % \parskip is discarded in each case
\parindent            \z@       % not used because of \noindent
\pretolerance       10000       % \
\tolerance          10000       % |
\hyphenpenalty      10000       % | hyphenation parameters are
\exhyphenpenalty    10000       % | really irrelevant
\binoppenalty       10000       % |
\relpenalty         10000       % |
\adjdemerits            0       % |
\doublehyphendemerits   0       % |
\finalhyphendemerits    0       % /
\baselineskip         \z@       % bug in Luatex? 17.5.2013 and 11.5.2014
\@cd@centre@hlabel@false
%
% Some initial things to ensure \endgraf always generates \parskip\baselineskip
% (even though we always discard them, but we're using the vertical list as
% a stack, so we've got to be regular about things):
% \hbox{}\nointerlineskip at the beginning of the diagram ensures that the
% vertical list is non-empty, so \parskip is generated, but suppresses
% \baselineskip before the top row of the matrix; now we ensure that
% \baselineskip IS generated in our next use.
\prevdepth\z@ % ensures \baselineskip is present - (maybe it shouldn't be)
%
}% (end of \bombparameters)
%
%
\newbox\math@on@box\newbox\math@off@box
\def\math@on{\unhcopy\math@on@box}\def\math@off{\unhcopy\math@off@box}%
%
\def\start@bomb@vlist{\hbox{}\penalty1\nointerlineskip}%
%
%********************* re-alignment of cell ********************
%
% \reformat@cell takes
%       \hbox\cd@cell (current cell) or \@VonH
%       \hbox\pending@left  (donation from right)
%       \left@donated  (width of donation from right)
%       \box\cd@donat (donation from above)
% and returns
%       \hbox\pending@left  (donation to left)
%       \left@donated  (width of donation to left)
%       \box\cd@donat (donation downwards)
% and accumulates in \hbox\cd@cell:
%       completed horizontal arrows,
%       completed vertical arrows
%       objects
%
% The paragraph builder adds
%  0:   \parskip
%  1:   \parskip\baselineskip\hbox
%  2:   \parskip\baselineskip\hbox\baselineskip\hbox
%  3:   etc
% to the current vertical list; \reformat@object & \reformat@complex
% remove all but \parskip.  None of this glue or penalty is wanted.
%
% The lines of the paragraph are
%  1:   missives
%  2:   empty cell: \null\penalty10000\parfillskip\rightskip
%       object: \null\hfil\mathon text\penalty-9993\rightskip
%       horizontal: \null\hfil\kern(shortfall)\null\xleaders\kern\kern
%               \penalty-9999\rightskip
%  3:   horizontal: \null\kern\hbox\hfill\hbox\kern\penalty-9993\rightskip
% last: profile information (not used for empty cells):
%               \null\kern-2\cd@hshift\penalty10000\parfillskip\rightskip
%
\def\reformat@cell{%
%\showboxdepth 2 \showboxbreadth 999 \tracingonline1 \showbox\cd@cell
\penalty5               % mark \parskip
\noindent
\setbox\object@profile =\null           % initialise profile
\left@width\z@\right@width \z@  % widths
%
% use paragraph builder to split the cell
\ifnum  \cd@cell<\cd@right
        %\showbox\cd@cell
        \ht\object@profile \ht\cd@cell
        \dp\object@profile \dp\cd@cell % default ht/dp of profile
        \unhbox\cd@cell\skip0=\lastskip\unskip
\else   \@VonH\skip0=\z@        % if out of range
\fi
\endgraf%\showboxdepth 2 \showboxbreadth 999 \tracingonline1 \showlists
%
%
%\showlists
%\expandafter\message{cell (\the\cd@row,\the\cd@cell) % ascii
%   prevgraf=\the\prevgraf\new@line}%
\ifcase\prevgraf        % test number of lines as above
        \cd@shouldnt Y         % 0: empty cell
\or     \cd@shouldnt Z          % 1: unused (maybe \HonV, \VonH)
\or     \reformat@empty         % 2: empty cell
\or     \reformat@object        % 3: object (maybe \HmeetV) with profile
\else   \reformat@complex       % 4+: many cases
\fi
%
\unskip
\setbox0=\lastbox       % all the missives
\unskip\unskip\unpenalty% discard \baselineskip, \parskip and marker 5
%
\noindent\unhbox0% unpack the missives
% remove \null \penalty1000 \parfillskip \rightskip \penalty-9990 \null
\setbox0\lastbox\unpenalty\unskip\unskip\unpenalty\setbox0\lastbox
%\showlists
\loop@on@maps
        \cd@penalty\lastpenalty\unpenalty % code no. of missive
\ifnum\cd@penalty>\z@
        \setbox\z@\lastbox
        \cell@missive
\repeat
%
\endgraf
\unskip\unskip\unpenalty              % remove \parskip and marker (5)
%
}%
%
\def\show@prevgraf{%
\cd@num@a\cd@top\advance\cd@num@a-\cd@row
\cd@num@b\cd@cell\advance\cd@num@b-\cd@left\advance\cd@num@b 1
\expandafter\message{prevgraf=\the\prevgraf at (\the\cd@num@a,\the\cd@num@b)}%
}%
%
%
%=======================================================================%
%                                                                       %
%       (14) REFORMATTING OBJECTS AND CROSSES                           %
%                                                                       %
%=======================================================================%
%
%       Use of registers during the reformatting process
%
%       \box                    \dimen                  \skip
%  0    scratch                 scratch                 scratch
%  1    left  \ part of         scratch                 completed depth
%  2    right / current cell    scratch                 interline above
%  3    scratch                 scratch                 intercolumn left
%  4    scratch                 left  \ width of        horiz \ extra cell
%  5    profile (\ht,\dp)       right / profile         vert  / size needed
%  6    right \ part of pending right \ width of        right \ overlap of
%  7    left  / horizontal      left  / donation        left  / whole diagram
%  8    scratch                 height\ of horiz        height\ of this row
%  9    \hbox{$A^f_f$}          depth / rule            depth /
%
%
\def\reformat@object{%
\get@profile@info       %
\setbox\right@part=\lastbox     % fetch box
\setbox\right@part=\hbox{%
        \unhbox\right@part      % re-set to natural size
        \unskip                 % \rightskip
        \unpenalty              % -9993
}%              
\unskip                         % discard \baselineskip
%
% make profile - detail if bigger than $A^f_f$
\ifdim\ht\right@part>\ht\default@profile
        \setbox\object@profile=\copy\right@part 
\else\ifdim\dp\right@part>\dp\default@profile
        \setbox\object@profile=\copy\right@part 
\else   \make@profile\right@part % (13.7.94)
\fi\fi
%
\advance\left@width.5\wd\right@part
\advance\right@width.5\wd\right@part
%
\setbox\right@part=\hbox{\unhbox\right@part\math@off}%
%
% whether to output?
\output@cell\left@width{\box\right@part}\right@width\z@
\complete@vertical
\complete@horizontal
}%
%
% last line of nontrivial paragraph is profile information
% currently just a kern to balance right shift (\cd@hshift)
\def\get@profile@info{%
% pick up width of \span'ned cells (see \reformat@empty) from \dimen0
% use negative value of \across@cells to remember how many (extra) there were
%\expandafter\message{across \the\across@cells\space cells, \the\dimen0^^J}%
\ifnum\across@cells>0
        \advance\dimen0-\column@placing
        \cd@hshift-.5\dimen0
        \across@cells-\across@cells
\else   \across@cells0
        \cd@hshift\z@
\fi
\setbox\object@profile =\lastbox        % the last line, including profile info
%\showbox\object@profile
\setbox\object@profile =\hbox{\unhbox\object@profile    % take it apart:
        \unskip\unskip\unpenalty        % \rightskip\parfillskip\penalty10000
        \setbox0=\lastbox               % \null protection of glue etc
\global\cd@dim@g\lastkern\unkern% balance
        }%
\advance\cd@hshift-.5\cd@dim@g          % the amount to shift right
\unskip                                 % remove \baselineskip
\setbox\object@profile =\null           % initialise profile
\right@width\cd@hshift
\left@width-\cd@hshift
}%
\def\axis@profile{%
\ht\object@profile\rule@height
\dp\object@profile\rule@depth}%
%
\def\make@profile#1{% (13.7.94)
\setbox\object@profile=\hbox{%
        \at@least{\ht\object@profile}{\ht#1}%
        \at@least{\dp\object@profile}{\dp#1}%
        \at@least{\wd\object@profile}{\wd#1}%
        \vrule height\ht\object@profile
                depth\dp\object@profile
                width\wd\object@profile
}}%
%
%******************** reformat maps ************************************
%
% \reformat@complex deals with arrows, piles and obstructions
% all of which were three-line paragraphs (except multiple verticals).
% The following is removed from the stack (current vertical list):
%               \glue\baselineskip
%  \box\left@part:=     \hbox(first line)
%                       (penultimate part of cell up to and including
%                       \penalty-9999   % whatever we used to force a split)
%                       \glue\rightskip
%               \glue\baselineskip
%  \box\right@part :=   \hbox(last line)
%                       (last part of cell)
%                       \penalty10000
%                       \glue\parfillskip
%                       \glue\rightskip
% by this routine; for multiple vertical arrows, \reformat@vert clears
% the remainder as required by \reformat@cell.
%
%
%       \skip0: scratch (local to scope of \hbox)
%       \dimen6: scratch
%
\def\reformat@complex{%
\get@profile@info
\axis@profile % (13.7.94)
\setbox\right@part=\lastbox     % right(most) part
\unskip                         % discard \baselineskip
\setbox\left@part=\lastbox      % left (or next-to-rightmost) part
\unskip                         % discard \baselineskip
\setbox\left@part=\hbox{%
        \unhbox\left@part       % open left part
        \unskip                 % remove \rightskip
\global \cd@num@g\lastpenalty   % extract the code
        \unpenalty
        }%                      % reset to natural width
\advance\cd@num@g9999
%\tracingonline1 \showboxbreadth999 \showboxdepth1 \showbox\object@profile
\ifcase\cd@num@g % now switch on the code [use \vadjust\penalty instead?]
        \reformat@horiz % -9999: single horizontal
\or     \reformat@pile  % -9998: multiple horizontal
\or     \reformat@HonV  % -9997: \HonV
\or     \reformat@VonH  % -9996: \VonH
\or     \reformat@vert  % -9995: vertical(s)
\or     \reformat@HmeetV% -9994:  \HmeetV
%\or    \reformat@overprint% -9993: idea: overprints (eg pullback symbol)
%\or    \reformat@user  % -9992: idea: user-defined command
\else   \cd@shouldnt 9% unrecognised \penalty splitting cell
\fi
}%
% idea: define the above with a "\new.." construct
% single horizontal arrow \hbox\left@part=left \hbox\right@part =right
%       output pending vertical (which has now been obstructed)
%       donate both parts
%
%******************** horizontals ************************************
%
\def\reformat@horiz{%
\make@profile\right@part % this is where the labels are (13.7.94)
\@reformat@horiz
\setbox\pending@left=\box\left@part
\setbox\pending@right=\box\right@part
%\showboxdepth999 \showboxbreadth999 \showbox\pending@right
}%
%
\def\reformat@pile{%
%\showbox\left@part\showbox\right@part
\make@profile\left@part % (13.7.94)
\setbox\right@part\hbox{% 15.4.95 test for extra material on right of \pile
  \penalty 8 %
  \unhbox\right@part\unskip\unpenalty
  \ifnum\lastpenalty=8
  \else\pile@junk
  \fi}%
\@reformat@horiz
\setbox\left@part=\hbox{%
        \unhbox\left@part       % extract the \vbox from the left part
        \unskip                 % \rightskip
        \unpenalty              % -9998
\global \setbox\cd@box@g=\lastbox
        }%  previous item in horiz list is \mathon, so can't really ...
% test if anything remains on the left (test its natural width, anyway).
\ifdim\wd\left@part=\z@\else\pile@junk\fi
\setbox\pending@left=\box\cd@box@g
                        % save the pile \vbox as the horizontal donation
}%
\def\pile@junk{\cd@refmt@error
   {extra material in \string\pile\space cell (lost)}}%ascii
%
\def\@reformat@horiz{% this code is common with \reformat@pile
\complete@vertical
\ifvoid\pending@left\else
        \cd@refmt@error{Clashing horizontal arrows}%
        \right@width.5\left@donated     % setting profile shares the space
        \left@width-\right@width        % buggers \across and \shift though
        \complete@horizontal            % output the offending arrow
        \right@width\z@                 % and our profile is zero width again
        \left@width\z@
\fi
\right@donated\left@donated             % what its width will be
\advance\right@donated-\right@width
\left@donated-\left@width               % new donation - towards the left width
\declared@at@cell\cd@cell
}%
%
%
%
%******************** reformat empty cells ************************************
%
% There are five types of empty cell:
% - empty/white (adjacent &'s)
% - \span: \across, \mutispan, LaTeX version?
% - \HonV
% - \VonH
% - \HmeetV
%
% the absolute value of \across@cells is the number of \span'ned cells to
% the right; positive to show we're still collecting them, negative means
% we've taken account of the width and only want this for error reporting.
% \dimen0 accumulates the width - remember we're only going round a tight
% loop in \reformat@row, with \reformat@cell, ending up in \get@profile@info
%
\def\reformat@empty{%
\setbox0\lastbox\unskip
\cd@hshift\z@           % what \get@profile@info would do
\axis@profile
\ifdim\skip0>\z@
\then                           % empty/white
        \across@cells0          % --- ignore any \across
\else                           % \across
        \ifnum\across@cells<1
                \across@cells0  % first one
                \dimen0\column@placing
        \fi %
        \advance\across@cells 1
\fi
}%
%
%\newif\iffred
% the three cross commands
\def\VonH  {\cd@cross 46\VonH{.5\intended@breadth}}%
\def\HonV  {\cd@cross 57\HonV{.5\intended@breadth}}%
\def\HmeetV{\cd@cross 44\HmeetV{-\MapShortFall}}%
%
% idea: \solder \HjumpV \VjumpH
%
% choose the \penalty, check that we're allowed and read the next token
% #1=new horizontal state after donated arrow,
% #2=last digit of \penalty, #3=name
% #4=effective map breadth
\def\cd@cross#1#2#3#4{%
\check@vert34#1{\string#3}\exec@cross   % ensure correct horizontal state
\cd@penalty-999#2                       % the penalty value
\dimen0=#4%             % initialise strut size (\dimen0,8,9)
\rule@height\dimen0\advance\rule@height\axisheight
\rule@depth\dimen0\advance\rule@depth-\axisheight
%\iffred
%\rule@height\axisheight
%\rule@depth-\rule@height
%\advance\rule@height.5\rounded@breadth
%\advance\rule@depth.5\rounded@breadth
%\fi
%\expandafter\message{ht=\the\rule@height, dp=\the\rule@depth}%
\@ifoptarg\cross@strut\exec@map}%       % get optional argument and do it
% \exec@map=\exec@cross (or ignore with error message if outside diagram)
%\exec@map}%
%
% use optional argument to re-calculate strut size
\def\cross@strut#1{%
\setbox0=\hbox{\begin@maths#1\end@maths}%
\dimen0.5\wd0
\rule@height \ht0
\rule@depth \dp0
\exec@map % and do it
}%
% put half the strut on either side of the \penalty
\def\exec@cross{%
\setbox0=\null
\ht0=\rule@height 
\dp0=\rule@depth 
\wd0=\dimen0
\copy0\penalty\cd@penalty\box0
}%
%
%\def\MapCorner{{%
%\rounded@breadth=-2\MapShortFall
%\set@axis
%\vrule width\rounded@breadth \horizhtdp
%}}%
%
\def\reformat@HonV  {\cross@profile\complete@vertical}%
\def\reformat@VonH  {\cross@profile\complete@horizontal}%
\def\reformat@HmeetV{\cross@profile\complete@vertical\complete@horizontal}%
%
\def\cross@profile{%
\setbox\right@part=\hbox{\unhbox\right@part}% right strut
\setbox\left@part=\hbox{\unhbox\left@part       % left strut
\global \setbox\cd@box@g=\lastbox % this is the real (left) strut (is it?)
        }%
\ht\object@profile  \ht\cd@box@g        % get its real height
\dp\object@profile  \dp\cd@box@g        % and depth
\advance\left@width \wd\cd@box@g        % and left width
\advance\right@width\wd\right@part      % right width
}%
%
%=======================================================================%
%                                                                       %
%       (15) LaTeX LINE CHARACTERS                                      %
%                                                                       %
%=======================================================================%
%
\new@if\ifPositiveGradient\PositiveGradienttrue\PositiveGradientfalse
\PositiveGradienttrue
\new@if\ifClimbing\Climbingtrue\Climbingfalse\Climbingtrue
\newcount\DiagonalChoice\DiagonalChoice\m@ne
%
% LaTeX line & arrow font
\ifx\tenln\nullfont
\then   \def\line@char{\no@tenln
                \ifPositiveGradient/%ascii slash stands in for LaTeX slopes
                \else\begin@maths\backslash\end@maths\fi}%or backslash
\else   \def\line@char{\line@font\char\count@}%
\fi
\let\line@font\tenln
%
%
%===========================================================================
% get LaTeX line characters
% for x=\denominator@ y=\numerator@ using \ifPositiveGradient
%
\def\Use@line@char#1{\hbox{#1\line@font
\ifPositiveGradient\else\advance\count@ 64 \fi
\char\count@}}%
%
\def\LaTeX@line@char{\Use@line@char{%
\count@\denominator@\multiply\count@ 8\advance\count@ -9%
\advance\count@\numerator@}}%
%
\def\LaTeX@arrow@char{\Use@line@char{%
\ifcase\DiagonalChoice
   \LaTeX@SW
\or\LaTeX@NE
\or\LaTeX@NE
\else\LaTeX@SW
\fi}}%
%
\def\LaTeX@SW{%
\ifnum\denominator@=\z@
   \count@'33 % left (-1,0)
\else
   \count@\denominator@
   \multiply\count@\sixt@@n
   \advance\count@ -9%
   \advance\count@\numerator@
   \advance\count@\numerator@
\fi}%
%
% this might just as well be a case switch!
% 81 tokens versus 115 for \@getrarrow in LaTeX
\def\LaTeX@NE{%
\count@'%
\ifcase\numerator@      55%
\or\ifcase\denominator@ 66\or 22\or 52\or 61\or 72\fi
\or\ifcase\denominator@ 66\or 25\or 22\or 63\or 52\fi
\or\ifcase\denominator@ 66\or 16\or 36\or 22\or 76\fi
\or\ifcase\denominator@ 66\or 27\or 25\or 67\or 22\fi
\fi\relax}%
%
\def\double@LaTeX#1{\hbox{#1\setbox0=\Use@line@char{#1}%
                \ifPositiveGradient\else\raise.3\ht0\fi\copy0
                \kern-.7\wd0
                \ifPositiveGradient\raise.3\ht0\fi\box0}}%
\def\left@LaTeX@tail#1{\hbox{\setbox0=#1%
                \kern-.75\wd0
                \vbox to.25\ht0{%
                        \ifPositiveGradient\else\vss\fi
                        \box0
                        \ifPositiveGradient\vss\fi}%
                }}%
\def\right@LaTeX@tail#1{\hbox{\setbox0=#1%
                \dimen0=\wd0
                \vbox to.25\ht0{%
                        \ifPositiveGradient\vss\fi
                        \box0
                        \ifPositiveGradient\else\vss\fi}%
                \kern-.75\dimen0
                }}%
%
% ****************** LaTeX line-font components *****************
%
% LaTeX diagonal arrow heads
\def@name{+h:>}{\Use@line@char\LaTeX@NE}%
\def@name{-h:>}{\Use@line@char\LaTeX@SW}%
\let@names{+t:<}{-h:>}%
\let@names{-t:<}{+h:>}%
%
% used as tails (different positioning)
\def@name{+t:>}{\left@LaTeX@tail {\Use@line@char\LaTeX@NE}}%
\def@name{-t:>}{\right@LaTeX@tail{\Use@line@char\LaTeX@SW}}%
\let@names{+h:<}{-t:>}%
\let@names{-h:<}{+t:>}%
%
% LaTeX diagonal double arrow heads
\def@name{+h:>>}{\double@LaTeX\LaTeX@NE}%
\def@name{-h:>>}{\double@LaTeX\LaTeX@SW}%
\let@names{+t:<<}{-h:>>}%
\let@names{-t:<<}{+h:>>}%
\let@names{+h:>->}{+h:>>}%
\let@names{-h:>->}{-h:>>}%
\let@names{+t:<-<}{-h:>>}%
\let@names{-t:<-<}{+h:>>}%
%
% used as tails (different positioning - currently too close to object)
\def@name{+t:>>}{\left@LaTeX@tail {\double@LaTeX\LaTeX@NE}}%
\def@name{-t:>>}{\right@LaTeX@tail{\double@LaTeX\LaTeX@SW}}%
\let@names{+h:<<}{-t:>>}%
\let@names{-h:<<}{+t:>>}%
\let@names{+t:>->}{+t:>>}%
\let@names{-t:>->}{-t:>>}%
\let@names{+h:<-<}{-t:>>}%
\let@names{-h:<-<}{+t:>>}%
%
% LaTeX diagonal line segment filler
\def@name{+f:-}{\if@use@TPIC@\null\else\LaTeX@line@char\fi}%
\let@names{-f:-}{+f:-}%
%
% dot filler
\def\dot@filler#1#2{\vbox to#1{\vss\hbox to#2{\hss.\hss}\vss}}%
\def\hfdot{\dot@filler{2\axisheight}{.5em}}%% % .7em until 29.7.98
\def\vfdot{\dot@filler{1ex}\z@}%% % 1.46ex until 29.7.98
\def\LaTeX@dot@filler{\hbox{%
\dimen0=.3\@em\dimen1\dimen0
\ifnum\numerator@>\denominator@\divide@{\dimen1}%
\else\multiply@{\dimen0}\fi
\dot@filler{\dimen0}{\dimen1}}}%
\newarrowfiller{.}\hfdot\hfdot\vfdot\vfdot
\def\dfdot{\LaTeX@dot@filler\@use@TPIC@false}% 12.7.94
\def@name{+f:.}{\dfdot}%
\def@name{-f:.}{\dfdot}%
%
% proposed by Richard Kennaway 11.9.97
%\def\colon@filler#1#2{\vbox to#1{\vss\hbox to#2{\hss=\hss}\vss}}%%
%\def\hfcolon{\colon@filler{2\axisheight}{1.1em}}%%
%\def\vfcolon{\colon@filler{1.46ex}\z@}%%
%\newarrowfiller{:}\hfcolon\hfcolon\vfcolon\vfcolon
% but this needs more thought as it's neither a colon nor a double line
%
%
% ****************** old LaTeX line-font components *****************
%
\def\use@line@char#1{\hbox\bgroup\def\next{#1\egroup}\afterassignment\next%%
\count@='}%
%
% still used for orthogonals arrowheads
\def\lnchar{\use@line@char\line@char}%
%
% the rest is obsolete
% commented out 15.10.2008 (v3.93)
% because Apostolos Sypopoulos <ijdt.editor@gmail.com> said that
% "the command \lat should be renamed \l@t to avoid conflict
% with the name of some unicode math symbol."
% \let\laf\lnchar\let\lah\lnchar
% \def\lad{\use@line@char\xlad}%
%
% \def\xlad{\setbox2=\hbox{\line@char}%
% \setbox0=\hbox to.3\wd2{\hss.\hss}%
% \dimen0=\ht0 \advance\dimen0-\dp0
% \dimen1=.3\ht2 \advance\dimen1-\dimen0 \dp0=.5\dimen1
% \dimen1=.3\ht2 \advance\dimen1\dimen0 \ht0=.5\dimen1
% \raise\dp0\box0}%
%
% \def\lahh{\use@line@char\xlahh}%
% \def\lat{\use@line@char\xlat}%
%
% into tails
% \def\xlat{\setbox0=\hbox{\line@char}%
% \dimen0=\ht0
% \setbox1=\hbox to.25\wd0{%
% \ifcase\DiagonalChoice
%         \box0\hss
% \or     \hss\box0
% \or     \hss\box0
% \or     \box0\hss
% \fi}%
% \vbox to.25\dimen0{%
% \ifClimbing\box1\vss\else\vss\box1\fi\kern\z@}%
% }%
% %
% % Can't mangle \mv because it's used in old extra-diagonals.tex
% % double arrowheads
% \def\xlahh{\setbox0=\hbox{\line@char}%
% \ifPositiveGradient
% \then   \copy0 \kern-.7\wd0 \mv.3\ht0\box0
% \else   \ifClimbing
%         \then   \copy0 \kern-.7\wd0 \mv.3\ht0\box0
%         \else   \mv-.3\ht0\copy0 \kern-.7\wd0 \box0
% \fi\fi}%
%
%=======================================================================%
%                                                                       %
%       (16) DIAGONALS                                                  %
%                                                                       %
%=======================================================================%
%
% ******************* \LaTeX@make@line **********************
%
% arithmetic for diagonal repeaters:
%  ^            _____a______
%  :            |          ^
%  :            |          |
%  :            |          |b   n-1 = floor (e/a)
%  :    <---c-->+---       |    (n-1)c+a = e
%  :    |       |  |       |    b/a = d/c = num/den
%  :    |       <f>+-------v    f = a-c
%  :    |          ^
%  :    |          d
%  :    |          |
%  v:   -----------v
%
%       <--------e--------->
%
% the height of the baseline is not specified
%
%
\def\LaTeX@make@line#1{% use \box#1 to make \box#1 with width \dimen#1
\setbox#1=\hbox{%
\dimen5\dimen#1 % required horizontal distance (\dimen5=e)
%\expandafter\message{\string\dimen#1=\the\dimen#1}%
\setbox8=\box#1
\dimen1\wd8     % width (\dimen1=a)
\count@\dimen5          % distance coerced to integer (scaled points)
\divide\count@\dimen1   % no of segments minus one (\cd@num@a=n-1=floor(e/a))
\ifnum  \count@=0       % 
        \box8           % just one
        \ifdim\dimen5<.95\dimen1 \cd@warning{diagonal line too short}\fi
\else   \dimen3=\dimen5         % otherwise, calculate...
        \advance\dimen3-\dimen1 % e-a
        \divide\dimen3\count@   % repeat width (\dimen3=c=(e-a)/(n-1))
        \dimen4\dimen3
        \multiply@{\dimen4}%    % repeat height (\dimen4=d)
        \ifPositiveGradient\multiply\dimen4\m@ne\fi
        \dimen6\dimen1
        \advance\dimen6-\dimen3 % backspace (\dimen6=d==a-c)
        \loop % on bits
                \raise\count@\dimen4\copy8      % a copy of the repeater
        \ifnum  \count@>0
                \kern-\dimen6           % overlap 
                \advance\count@\m@ne
        \repeat
\fi}}%
\def\make@line#1{\if@use@TPIC@\tpic@make@line{#1}\else\LaTeX@make@line{#1}\fi}%
\def\no@make@line#1{}%
%
% *********************** \exec@LaTeX@diagonal **************************
%  baseline_____________________________________
%   ^           |   \MapShortFall ______________|
%   :           |                |          |UT |
%   :           |                |          |___|       UT = upper tip
%\DiagramCellHeight          ____|              |       UF = upper filler
%   :           |            |UL |      UF      |       UL = upper label
%   :           |            |___|_____________|        M  = middle
%   :   axis____|                |              |       etc
%   v           |----------------|---|          |
%  baseline_____|                |LL |          |
%               |       LF       |----          |
%               |                |              |
%               |___             |              |
%               |LT |            |              |
%               |___|____________|              |\MapShortFall
%            |  |\MapShortFall                  |  |
%            ------------------------------------
%               ^\objectheight   <\DiagramCellWidth>
%  baseline_____v
%
% height and depth is the "obvious": as the arrows, as far as the tips.
% width is zero, so that for one-cell arrow, centered in cell;
% multicell arrows stick out on right, as if centered in that many cells.
% 
% assumed height and half-width of endpoints
\newdimen\objectheight          \objectheight           1.8ex
\newdimen\objectwidth           \objectwidth            1em % 13.7.94
%
% \dimen0 depth of lower tip (from baseline of current cel)
% \dimen1 distance to left tip (from centre of current cell)
% \dimen2 width of left filler
% \dimen3 distance from left tip to left edge of middle
% \dimen4 width of right filler
% \dimen5 height of upper tip  (from baseline of current cell)
% \dimen6 total height of arrow
% \dimen7 total width  of arrow
% \dimen9 twice amount to lower middle (from baseline of current cell)
%
%            ----- check we really have a diagonal -----
%
\def\exec@LaTeX@diagonal{%
% calculate total height and width including shortfall
\dimen6=\y@coord\DiagramCellHeight
\dimen7=\x@coord\DiagramCellWidth
\set@fraction  % calculate y=\numerator@ and x=\denominator@
\ifnum\numerator@>0
   \ifnum\denominator@>0
       \@@LaTeX@diagonal
   \else
       \aftergroup\diag@is@vert
   \fi
\else
   \aftergroup\diag@is@horiz
\fi}%
%
\def\diag@is@vert {\cd@error{diagonal map is nearly vertical}\cd@diag@zer}%
\def\diag@is@horiz{\cd@error{diagonal map is nearly horizontal}\cd@diag@zer}%
\new@help\cd@diag@zer{Use an orthogonal map instead}%
%
\def\@@LaTeX@diagonal{%
%  use appropriate LaTeX line characters (set boxes 1-5)
\set@map@parts
%
% re-calculate width corresponding to height
\dimen3\dimen7\dimen7\dimen6\divide@{\dimen7}%
\advance\dimen3-\dimen7 % width error (both sides)
%
%                ----- compute shortfalls -----
%
\interim@shortfall
\ifnum\numerator@>\denominator@
  % steep:
  \advance\dimen6-\dimen1\advance\dimen6-\dimen5 % apply shortfalls to height
  \divide@{\dimen1}\divide@{\dimen5}% and convert them to widths
\else % shallow
  \dimen0\dimen1\advance\dimen0\dimen5\multiply@{\dimen0}% convert to height
  \advance\dimen6-\dimen0
\fi
%
\dimen2.5\dimen7\advance\dimen2-\dimen1 % width of left half
\dimen4.5\dimen7\advance\dimen4-\dimen5 % width of right half
%
\ifPositiveGradient
     \dimen0\dimen5 % use right margin to calculate top margin
     \advance\dimen1-\x@coord\DiagramCellWidth % stick out a lot on the left
     \advance\dimen1 \x@offset\DiagramCellWidth % relative to where?
     \setbox6=\llap{\unhbox6\kern.1\ht2}%
     \setbox7=\rlap{\kern.1\ht2\unhbox7}%
\else
     \dimen0\dimen1 % use left margin to calculate top margin
     \advance\dimen1-\x@offset\DiagramCellWidth % relative to where?
     \setbox7=\llap{\unhbox7\kern.1\ht2}%
     \setbox6=\rlap{\kern.1\ht2\unhbox6}%
\fi
%
\setbox6=\vbox{\box6\kern.1\wd2}\setbox7=\vtop{\kern.1\wd2\box7}%
%
\multiply@{\dimen0}% convert top margin from width to depth
\advance\dimen0-\axisheight\advance\dimen0-\y@offset\DiagramCellHeight
\dimen5-\dimen0 % height of upper tip
\advance\dimen0\dimen6 % depth of lower tip
%
\advance\dimen1.5\dimen3 % adjust left margin for width error
%
% middle disables through
\ifdim\wd3>\z@\ifdim\ht3>-\dp3\@cd@through@false\fi\fi
%
\dimen3\dimen2
\dimen7\dimen2\advance\dimen7\dimen4
\ifvoid3
\else
   \if@cd@through@
   \else
      % calculate x coordinate of intersection with top of middle
      \dimen8\ht3\advance\dimen8-\axisheight\divide@{\dimen8}%
      \at@most{\dimen8}{.5\wd3}% or choose intersection with edge
      %
      % calculate x coordinate of intersection with bottom of middle
      \dimen9\dp3\advance\dimen9\axisheight\divide@{\dimen9}%
      \at@most{\dimen9}{.5\wd3}% or choose intersection with edge
      %
      \ifPositiveGradient
           \advance\dimen2-\dimen9\advance\dimen4-\dimen8 % shorten fillers
      \else\advance\dimen4-\dimen9\advance\dimen2-\dimen8 % appropriately
   \fi\fi
   \advance\dimen3-.5\wd3
\fi
\dimen9=\y@coord\DiagramCellHeight\advance\dimen9-2\DiagramCellHeight
%
%
% make the fillers;
% re-use \dimen2 and \dimen4 as amounts to raise them (instead of their widths)
\if@cd@through@
   \advance\dimen2\dimen4
   \make@line{2}% width \dimen2 using \box2 to make \box2
   \dimen2-\dimen0\advance\dimen2\dp2 % amount to raise it
\else
   \make@line{2}% width \dimen2 using \box2 to make \box2
   \make@line{4}% width \dimen4 using \box4 to make \box4
   \ifPositiveGradient
        \dimen2-\dimen0\advance\dimen2\dp2 % amount to raise left
        \dimen4\dimen5\advance\dimen4-\ht4 % amount to raise right
   \else\dimen4-\dimen0\advance\dimen4\dp4 % amount to raise right
        \dimen2\dimen5\advance\dimen2-\ht2 % amount to raise left
\fi\fi
%
\setbox0=\hbox to\z@{%
% move to left edge
\kern\dimen1
%
% output the left tip
\ifvoid1
\else
   \ifPositiveGradient
        \advance\dimen0-\dp1
        \lower\dimen0
   \else\advance\dimen5-\ht1
        \raise\dimen5
   \fi\rlap{\unhbox1}%
\fi
%
% left filler
\raise\dimen2\rlap{\unhbox2}%
%
% output the middle
\ifvoid3 \else
   \lower.5\dimen9\rlap{\kern\dimen3\unhbox3}%
\fi
%
% labels
\kern.5\dimen7
\lower.5\dimen9\box6
\lower.5\dimen9\box7
\kern.5\dimen7
%
% right filler
\if@cd@through@\else
   \raise\dimen4\llap{\unhbox4}%
\fi
%
% right tip
\ifvoid5 \else
   \ifPositiveGradient
        \advance\dimen5-\ht5
        \raise\dimen5
   \else\advance\dimen0-\dp5
        \lower\dimen0
   \fi\llap{\unhbox5}%
\fi
%
\hss}%
\ht0=\axisheight\dp0=-\ht0\box0 }%
%
%\advance\dimen6.25\dimen8      % amount to raise upper label
%\advance\dimen7-.25\dimen8     % amount to raise lower label
%
%
%
%\setbox0=\hbox{\begin@maths\vcenter{%
%  \kern.9ex                            % space above
%  \hbox{%
%    \kern.4em                          % space on left
%    \count@=0
%    \mv-\ht1\box1                      % left tip
%    \loop % on bits
%    \ifnum\count@<\DiagonalLineSegments
%        \mv\count@\ht2\copy2           % filler
%        \advance\count@1
%    \repeat
%    \mv\count@\ht2\box5                        % right tip
%    \kern.4em                          % space on right
%  }%
%  \kern.9ex                            % space below
%}\end@maths}
%\dimen0=.5\wd0 \ht0\z@ \dp0\z@
% %\kern\dimen0
%\mv.5\wd2\hbox to\z@{\hss\box6\kern.5\ht2}% left label
%\kern-\dimen0
%\box0
%\kern-\dimen0
%\mv-.5\wd2\hbox to\z@{\kern.5\ht2\box7\hss}% right label
% %\kern\dimen0
%}
%
% Count clockwise from NW
% \ifPositiveGradient = \ifodd\diagonal@choice
% \ifClimbing = \ifnum\diagonal@choice<2
\def\NorthWest{\PositiveGradientfalse\Climbingtrue \DiagonalChoice0 }%
\def\NorthEast{\PositiveGradienttrue \Climbingtrue \DiagonalChoice1 }%
\def\SouthWest{\PositiveGradienttrue \Climbingfalse\DiagonalChoice3 }%
\def\SouthEast{\PositiveGradientfalse\Climbingfalse\DiagonalChoice2 }%
%
%
%
%=======================================================================%
%                                                                       %
%       (17) STRETCHABLE DIAGONALS                                      %
%                                                                       %
%=======================================================================%
%
% \missive at any point in the diagram text delivers the text to \cell@missive,
% which is called during \reformat@cell
%
% \hbox{(missive material)}
%
%\def\missive#1(#2,#3){\vadjust{\hbox{#1}\penalty#3\penalty#2\penalty2}}%
%\def\remissive#1(#2,#3)(#4,#5){\vadjust{%
%        \hbox{\hbox{#1}\penalty#3\penalty#2}%
%        \penalty#5\penalty#4\penalty103}}%
%\def\missivemap#1(#2,#3)(#4,#5){\vadjust{%
%        \hbox{\hbox{#1}\penalty#3\penalty#2}%
%        \penalty#5\penalty#4\penalty104}}%
\def\exec@missive{\vadjust{%
        \cd@num@a\cd@cell
        \advance\cd@num@a\ifPositiveGradient\else-\fi\x@offset\relax
        \cd@num@b\cd@row\advance\cd@num@b-\y@offset\relax
        \hbox{%
            \advance\cd@num@a\ifPositiveGradient-\fi\x@coord
            \advance\cd@num@b\y@coord
            \hbox{%
                \box6 % upper label
                \kern\crab@
                \kern\snake@
                \penalty1 % stops upper label being read as missing lower label
                \box7 % lower label
                \box\z@
            }%
            \penalty\cd@num@a
            \penalty\cd@num@b}%
        \penalty\cd@num@a\penalty\cd@num@b\penalty104}}%
%
\def\over@print#1{%
\relax % if case we're the first thing in a cell
%\ifmmode
    \vadjust{%
       \hbox@maths{#1}%
       \penalty\cd@cell
       \penalty\cd@row
       \penalty\tw@
    }%
%\else\cd@warning{mis-placed over-print ignored}% removed 15.4.95
%\fi
}%
%
% handle the missives
% \cd@penalty contains the code number, \box\z@ the missive material
% (note that we are currently in unrestricted horizontal mode,
% inside a paragraph in the main vertical list)
\def\cell@missive{%
%\expandafter\message{missive type \the\cd@penalty\space
%   received at (\the\cd@row,\the\cd@cell)\new@line}%
\ifcase \cd@penalty
        % 0: unused
\or     % 1: was used to mark an ordinal row of the matrix
\or     % 2: simple overprint
        %\message{overprint}%
        \output@cell{.5\wd0}{\box0}{.5\wd0}\z@%
\or     % 3: indirected overprint
        \unhbox\z@\setbox\z@\lastbox\output@cell{.5\wd0}{\box0}{.5\wd0}\z@
        \unpenalty\unpenalty\setbox\z@\lastbox
\or     % 4: draw diagonal
        \missive@diagonal
\else   % 100n+m: collect profiles of n more points and execute case m
        \advance\cd@penalty-100
        \ifnum\cd@penalty<\z@ \cd@shouldnt B\fi % unknown missive code
        \setbox\z@\hbox{%
                % save the profile of the current cell
                \kern\left@width
                \copy\object@profile
                \kern\right@width
                % and its coordinates
                \cd@num@a\cd@top\advance\cd@num@a-\cd@row\penalty\cd@num@a
                \cd@num@a\cd@cell\advance\cd@num@a-\cd@left\penalty\cd@num@a
                % at the front of the missive material
                \unhbox\z@
                % removing the coordinates of the next cell to visit
                \global\cd@num@g\lastpenalty\unpenalty% its row number
                \global\cd@num@h\lastpenalty\unpenalty}% its column number
        % send it there
        \cd@num@a-\cd@num@g\cd@num@b\cd@num@h
        \resend@missive
\fi}%
%
\def\missive@diagonal{%
%\global\@need@PS@lib@true % 12.7.94 deleted 6.10.2001
\unhbox\z@
\setbox\z@\lastbox
%
% get missive data
\cd@num@a\lastpenalty\unpenalty\advance\cd@num@a\cd@left@donat  % column no.
\cd@num@b\cd@top\advance\cd@num@b-\lastpenalty\unpenalty        % row no.
\dimen1\lastkern\unkern % right width
\setbox 3\lastbox % profile
\dimen0\lastkern\unkern % left width
%
\setbox0=\hbox to\z@{%
%
% get the arrow and the labels
\unhbox0\setbox0\lastbox
\setbox7\lastbox % lower label (\ifPositiveGradient right \else left)
\unpenalty
\snake@\lastkern\unkern
\crab@\lastkern\unkern
\setbox6\lastbox % upper label (\ifPositiveGradient left \else right)
%
% calculate \dimen7=unsigned width of diagonal map 14.7.94
\dimen7\column@placing\advance\dimen7-\wd\cd@num@a
\ifdim\dimen7<\z@
     \PositiveGradienttrue
     \multiply\dimen7\m@ne
     \let\mv\empty
\else\PositiveGradientfalse
     \def\mv{\raise\ht1}%
     \kern-\dimen7
\fi
%
% calculate \dimen6=height of diagonal map 10.7.94
\ifnum\cd@num@b>\cd@row
        \dimen6\completed@depth
        \advance\dimen6-\ht\cd@num@b
\else   \dimen6\z@
\fi
%
%\expandafter\message{(\the\dimen7,\the\dimen6)}%
% \dimen6=ht=\numerator@ \dimen7=dp=\denominator@ \dimen2=hypotenuse
\stretch@PS@diagonal
\rotate@box@z
%
% get these out of the way of \set@fraction
\setbox1\null\ht1\dimen6\wd1\dimen7
%
% denominator for sine/cosine is hypotenuse
\dimen7\dimen2
%
% cosine \cd@num@a/\cd@num@b
\dimen6\wd1 \set@fraction\cd@num@a\numerator@\cd@num@b\denominator@
%
% sine = \numerator@/\denominator@
\dimen6\ht1 \set@fraction
%
% use \box2 for position of middle
\setbox2\null
\divide\dimen2\tw@
\advance\dimen2\snake@ % snake to right
\multiply@@{\dimen2}\wd2\dimen2 % the width
%
\dimen0.5\dimen7
\advance\dimen0\ifPositiveGradient\else-\fi\snake@ %  snake up or down
\multiply@{\dimen0}%
\advance\dimen0-\axisheight % adjustment for maths axis
\ht2\dimen0
%
% crab adjustment (don't adjust for maths axis here)
\dimen0\crab@\multiply@@{\dimen0}\advance\dimen0\ht2\ht2\dimen0
\dimen0\ifPositiveGradient-\fi\crab@\multiply@{\dimen0}%
\advance\dimen0\wd2\wd2\dimen0
%
%
%
% use \box4 for amount by which to shift labels away from shaft
% this should agree with \baselikeskip in \label@horiz
% and the kerning of labels away from vertical arrows
\setbox4\null
\dimen0 .6\@em\multiply@@{\dimen0}\ht4\dimen0
\dimen0 .2\@em\multiply@{\dimen0}\wd4\dimen0
%
% local to this box:
%           positive gradient  |  negative gradient
% \box0     the horizontal arrow to be stretched
% \box1     vector between the centres of the cells which the arrow links
% \box2     position of middle
% \box3     profile
% \box4     amount by which to shift labels away from shaft
% \box6     upper left label   |  upper right label
% \box7     lower right label  |  lower left label
% \dimen0
% \dimen1
% \dimen2   hypotenuse
% \dimen3   unsigned width of arrow
% \dimen4   snake correction for length of label
% \dimen5   scratch
% \dimen6   height of arrow
% \dimen7   hypotenuse
%
% upper label
\dimen0\wd2
\ifvoid6\else
    \dimen1\ht4
    %\iftrue
    %   \advance\dimen1\axisheight % try locating by maths axis
    %   \ifdim\dimen1<\dp6\dimen1\dp6\fi % but at least depth
    %\fi % instead of base
    \advance\dimen1\ht2
    \correct@for@width 6+-%   \dimen4 = .5\wd6 * \dimen3 / \dimen7
    \raise\dimen1\rlap{%
    \ifPositiveGradient
         \advance\dimen0-\wd6\advance\dimen0-\wd4 % left
    \else\advance\dimen0\wd4 %right
    \fi
    \kern\dimen0\box6}%
\fi
%
% lower label
\dimen0\wd2
\ifvoid7\else
    \dimen1\ht4
    %\iftrue
    %    \advance\dimen1\axisheight % try locating by maths axis
    %    \ifdim\dimen1<\ht7\dimen1\ht7\fi % but at least height
    %\else
    %    \advance\dimen1\ht7 % instead of the top of the label box
    %\fi
    \advance\dimen1-\ht2
    \correct@for@width 7-+%   
    \lower\dimen1\rlap{%
    \ifPositiveGradient
         \advance\dimen0\wd4 %right
    \else\advance\dimen0-\wd7\advance\dimen0-\wd4 % left
    \fi
    \kern\dimen0\box7}%
\fi
%
% the arrow
\mv\box0\hss
}%
\ht0\z@\dp0\z@
%\output@cell{left width}{box}{right width}{raise}
\output@cell{\z@}{\box\z@}{\z@}{\axisheight}%
}%
%
\def\correct@for@width#1#2#3{% \dimen4 = .3\wd#1 * \dimen3 / \dimen7
    %
    % \dimen4 = effective half-width
    \dimen4.5\wd#1
    %\ifdim\dimen4<.5\@em\dimen4.5\@em\fi % unform correction for small labels
    \ifdim\dimen4>.25\dimen7\dimen4=.25\dimen7\fi % cut-off for big ones
    \ifdim\dimen4>\@em
        \dimen4.4\dimen4 % reduce the correction for biggish ones
        \advance\dimen4.6\@em % but make it continuous !
    \fi
    %
    % the projection onto the shaft of the effective half-width
    \multiply@@{\dimen4}%
    %
    % un-correct for the projection onto the shaft of the axis height
    \dimen5\axisheight\multiply@{\dimen5}\advance\dimen4-\dimen5
    %
    % horizontal adjustment: apply *another* cosine factor
    \dimen5\dimen4\multiply@@{\dimen5}%
    \advance\dimen0\ifPositiveGradient#2\else#3\fi\dimen5
    %
    % vertical adjustment: apply sine factor
    \multiply@{\dimen4}\advance\dimen1\dimen4
}
%
%
%=======================================================================%
%                                                                       %
%       (18) POSTSCRIPT AND TPIC ARROWS                                 %
%                                                                       %
%=======================================================================%
%
% from dvips.tex: (Rokicki)
%       \def\rotninety{\special{ps:currentpoint currentpoint translate 90
%          rotate neg exch neg exch translate}}%
%       \font\huge=cmbx10 at 14.4truept
%       \setbox0=\hbox to0pt{\huge A\hss}%
%       \vskip16truept
%       \centerline{%
%         \copy0
%         \special{ps:gsave}%
%         \rotninety\copy0
%         \rotninety\copy0
%         \rotninety\box0
%         \special{ps:grestore}}%
%       \vskip16truept
% prints something like
%       <A
%       V>
% except that all four characters are A from cmbx10.
%
% from rotate.tex: (Rokicki again)
%   These macros allow you to rotate or flip a \TeX\ box.  Very useful for
%   sideways tables or upsidedown answers.
%
%   To use, create a box containing the information you want to rotate.
%   (An hbox or vbox will do.)  Now call \@rotr\boxnum to rotate the
%   material and create a new box with the appropriate (flipped) dimensions.
%   \@rotr rotates right, \@rotl rotates left, \@rotu turns upside down, and
%   \@rotf flips.  These boxes may contain other rotated boxes.
%
%\newdimen\@rotdimen
%\newbox\@rotbox
%
% idea: circular arcs
% ask Rokicki about portability
% idea; collect PS definitions at top of diagram \vbox
%
%\def\@vspec#1{\special{ps:#1}}%  passes #1 verbatim to the output
%\def\@rotstart#1{\@vspec{gsave currentpoint currentpoint translate
% #1 neg exch neg exch translate}}% #1 can be any origin-fixing transformation
%\def\@rotfinish{\@vspec{currentpoint grestore moveto}}% gets back in synch
%
\def\expanded@ps@special#1{\expandafter\verbatim@ps@special{#1}}%
\cd@first@use\using@ps{output is PostScript dependent}%
%
\def\def@ps@turn{%\using@ps
  \verbatim@ps@special{%
    /bturn {%ascii                      % x y axisht on PS stack
        gsave                           % save graphics state
        currentpoint                    % push position
                        %#### 0 4 1 roll translate % fulcrum at axis height
        currentpoint translate          % move origin there
        4 2 roll neg exch atan rotate   % rotate baseline
                % dvips doesn't know we've changed the coordinate system, so
        neg exch neg exch translate     % move origin back
        } def
    /eturn {currentpoint grestore moveto} def}}%ascii
\def\do@eturn{\relax\if@pdf@\pdf@literal{Q}\else\verbatim@ps@special{eturn}\fi}
%
%\def\diagonal@box(#1,#2)#3{%ascii   COMPLETELY OBSOLETE - NO PDF VERSION
%  \global\@need@PS@lib@true     % define PS commands if necessary
%  {\dimen0=#1\relax
%   \dimen1=#2\relax
%               \dimen4=\axisheight
%                       \raise\dimen4 %#### would prefer PS to do this
%  \hbox{\expanded@ps@special{%
%       \dim@in@pts{\dimen0}\space % x (could use number of cells instead)
%       \dim@in@pts{\dimen1}\space % y
%                       %#### \dim@in@pts{\dimen4} \space % axis height
%       bturn}%
%               \Pythagorean@sum        %\dimen2:=sqrt((\dimen0)^2+(\dimen1)^2)
%                       \lower\dimen4 %#### would prefer PS to do this
%               \hbox to\dimen2{#3}%    % output the text
%       \do@eturn}%  \verbatim@ps@special{eturn}}%
%}}%
%
% *********** TPIC \special commands *************
%
%       see contrib/Vojta/xdvi/tpic.c aston/latex/contrib/eepic/eepic.sty
%
% pn <number>                 set pen size in thousandths of an inch (ugh!)
% fp                          flush path
% da <float>                  dashed line
% dt <float>                  dotted line
% pa <number> <number>        add a point to the current path
% ar <n> <n> <n> <n> <f> <f>  draw arc
% ia <n> <n> <n> <n> <f> <f>  draw invisible arc
% sp                          flush spline
% sh                          shade last box circle or ellipse
% wh                          whiten ditto
% bk                          blacken ditto
%
% xdvi doesn't honour the widths of TPIC diagonal lines; dvips does
%
% convert #1 accurately to thousands of an inch in \count@
\def\set@mil#1{\count@#1\relax
\multiply\count@7\advance\count@16577\divide\count@33154 }%
%
\def\expanded@tpic@special#1{\expandafter\special{#1}}
%
%\def\tpic@pen@size{\begingroup\set@mil\intended@breadth
%\expanded@tpic@special{pn \the\count@}\endgroup}%
%
\def\tpic@make@line#1{\setbox#1=\hbox{%
\dimen0\dimen#1\multiply@{\dimen0}\set@mil{\dimen0}% \dimen0=height
\setbox0=\null
\ifPositiveGradient
     \count@-\count@\ht0\dimen0
\else\dp0\dimen0
\fi
\box0 % strut
\cd@num@a\count@
\set@mil\intended@breadth\expanded@tpic@special{pn \the\count@}% set pen size
\expanded@tpic@special{pa 0 0}% start path here
\set@mil{\dimen#1}%
\expanded@tpic@special{pa \the\count@\space\the\cd@num@a}% path to here
\expanded@tpic@special{fp}% flush path
\kern\dimen#1}}%
% 
%
%=======================================================================%
%                                                                       %
%       (19) TRIGONOMETRY                                               %
%                                                                       %
%=======================================================================%
% diagonal of A3 paper is 1027pt
% y=\dimen6 and x=\dimen7 non-negative
% \dimen2=+sqrt(y^2+x^2) to within 0.2% (?)
%
\def\Pythagorean@sum{%
\set@fraction
\begingroup
%
% make y=\dimen2=\dimen7 the larger and x=\dimen6 the smaller
\ifdim  \dimen7<\dimen6
        \dimen2=\dimen6
        \dimen6=\dimen7
        \dimen7=\dimen2
        \count@\numerator@
        \numerator@\denominator@
        \denominator@\count@
\else
        \dimen2=\dimen7
\fi
%
% nothing to do if x=0
\ifdim\dimen6>.01\p@
   \@pyth@sum
   \global\cd@dim@g\dimen0
\else
   \global\cd@dim@g\dimen7
\fi
\endgroup
\dimen2\cd@dim@g
\make@division\num@@{\ifPositiveGradient\else-\fi\dimen6}%
\make@division\mnum@@{\ifPositiveGradient-\fi\dimen6}%
%\make@division\mdenom@@{\ifPositiveGradient-\fi\dimen7}%
\make@division\denom@@{\dimen7}%
}%
%
\def\@pyth@sum{%
\square@fraction% n/d = x^2/y^2
%
\ifdim  \dimen7>1.73\dimen6 % 1.73=sqrt(3)=sec(30deg)
%\then  % y>>x: use power series in u=x^2/2y^2: z=y'(4+4u-2u^2+2u^3) y'=y/4
        \divide\dimen2 4        % x'=\dimen2=y/4
        \multiply\denominator@ 2
\else
        % y~x:  use same series but in u=(x^2-y^2)/4y^2 with y'=y/(sqrt 8)
        \dimen2=0.353553\dimen2         % \dimen2=y'=y/(sqrt 8)
        \advance\numerator@-\denominator@
        \multiply\denominator@ 4
\fi
%
% now have
%       x'=\dimen2<341pt
% calculate
%       z=x'(4+4u-2u^2+2u^3-(5/2)u^4) in \dimen0 as accumulator
%
\dimen0=4\dimen2                % worst case:
 \monomial@  4%         <250pt
 \monomial@{-2}%                < 20pt
 \monomial@  2%         <  3.5pt        typically 0.2pt
 \monomial@{-2.5}%              <  0.66pt       drowned by rounding errors
%\monomial@{3.5}%               <  0.16pt
%\monomial@{-2.375}%    <  0.018pt      pixel at 1200dpi is 0.06pt
%\monomial@{2.0675}%    <  0.0025pt
}%
%
% \dimen0 is the angle using points for degrees
% \dimen1 the hypotenuse
% y=\dimen6 x=\dimen7 returned
%
\def\polar@to@rect{\begingroup
% reduce \dimen0 to between 0 and 45, and \count@ to number of octants
\count@\dimen0
\dimen2 45pt
\divide\count@\dimen2
\ifdim\dimen0<\z@\advance\count@\m@ne\fi
\ifodd\count@\advance\count@ 1\@cd@a@true\else\@cd@a@false\fi
\advance\dimen0-\count@\dimen2
\if@cd@a@\multiply\dimen0\m@ne\fi
\ifnum\count@<0 \multiply\count@-7 \fi
%
% save hypotenuse (the first term of cosine)
\dimen3\dimen1
\dimen6\dimen0
\dimen7 3754936sp
\ifdim\dimen0<6\p@\def\max@fraction{4000}\fi
\set@fraction % \numerator@/\denominator@ is angle in radians
%
% set first term of sine
\dimen2\dimen3\multiply@{\dimen2}%
%
% calculate multiplier: u=-x^2/6 where x is angle in radians
% not too good for cosines of angles between 1 and 4 degrees.
\square@fraction
\multiply\denominator@-6
%
% compute sin x = x-x^3/6+x^5/120 = x (1+u+(0.3)u^2)
\dimen0\dimen2
\monomial@ 1%
\monomial@{0.3}%
\dimen1\dimen0
%
% compute cos x = 1-x^2/2+x^4/24-x^6/720 = 1+3u+(1.5)u^2+(0.3)u^3
\dimen2\dimen3
\dimen0\dimen3
\monomial@ 3%
\monomial@{1.5}%
\monomial@{0.3}%
%
% swap sin/cos and change sign appropriately
\divide\count@2
\if@cd@a@\multiply\dimen1\m@ne\fi
\ifodd\count@\dimen2\dimen1\dimen1\dimen0\dimen0-\dimen2 \fi
\divide\count@2
\ifodd\count@\multiply\dimen0\m@ne\multiply\dimen1\m@ne\fi
%
% export
\global\cd@dim@g\dimen0\global\cd@dim@h\dimen1\endgroup
\dimen6\cd@dim@g\dimen7\cd@dim@h}%
%
% ****************** continued fraction approximation ********************
%
% set \numerator@/\denominator@ to nearest rational to \dimen6/\dimen7
% with both at most \max@fraction
\def\default@max@fraction{255}\let\max@fraction\default@max@fraction
\def\set@fraction{\begingroup
\ifdim\dimen7<\dimen6
  \dimen9\dimen7\dimen7\dimen6\dimen6\dimen9\@cd@a@true
\else
  \@cd@a@false
\fi
\dimen2\z@    \dimen3\one@sp            % b=0 b'=1 initialisation
\dimen4\one@sp\dimen0\z@                % c=1 c'=0
\dimen8=\max@fraction\one@sp            % d tolerance
\do@cont@frac
\global\cd@num@g\dimen\if@cd@a@ 0\else3\fi
\global\cd@num@h\dimen\if@cd@a@ 3\else0\fi
\endgroup
\numerator@\cd@num@g\denominator@\cd@num@h}%
%
\def\do@cont@frac{%
\count@\dimen6
\divide\count@\dimen7                   % u  := a/a'  new quotient
\advance\dimen6-\count@\dimen7          % a -:= ua'   reduced data
\dimen9\dimen4
\advance\dimen9\count@\dimen0           % c" := c+uc' trial denominator
%
\ifdim\dimen9>\dimen8                   % overflow
   \cont@frac@done
\else
   \cont@frac@swap      % b,b':=b',ub'+b; c,c':=c',c"
   \ifdim\dimen6>\z@    % if it's spot on return, else
       \dimen9\dimen6   % a,a':=a',a
       \dimen6\dimen7
       \dimen7\dimen9
       \expandafter\expandafter\expandafter
       \do@cont@frac    % carry on
\fi\fi}% result ends up as b'/c'
%
% When we've gone over the limit, but not twice, there's still a better
% approximation than the previous one, obtained by adjusting the quotient.
%
% Suppose b/c b'/c' and (b"=ub'+b)/(c"=uc'+c) are successive continued
% fraction approximants to r with c'<=d<c". Then any rational number p/q
% between b/c and b'/c' is at least as far away from r as p'/q where p'=vb'+b
% and q=vc'+c. We want v to be an integer such that q<=d. Is this closer
% than b/c (on the other side)? Yes if (p'/q) is less than twice as far from
% b/c as r is, which reduces to (a/a')<2v+(c/c'). This happens if u<2v.
% (It also happens if u=2v and a"c'<a'c, equivalently ac'<a'c", but we ignore
% this case.)
%
% If c'=0 d<c"<=2d then 1/d is the best approximant.
%
\def\cont@frac@done{%
\ifdim\dimen0=\z@          %
   \ifdim\dimen9<2\dimen8  % if c'=0 (so b'=1) and d<=c"<2d
      \dimen0\dimen8       %    choose d/1
   \fi
\else
   \advance\dimen8-\dimen4 
   \divide\dimen8\dimen0            % v := (d-c)/c' smaller quotient
   \ifdim\count@\one@sp<2\dimen8    % if u<2v there's a better approximation:
      \count@\dimen8
      \dimen9\dimen4
      \advance\dimen9\count@\dimen0 % c" := c+vc' recalculate denominator
      \cont@frac@swap               % and numerator, and swap
\fi\fi
}%
%
\def\cont@frac@swap{%
\dimen4\dimen0
\dimen0\dimen9
\advance\dimen2\count@\dimen3
\dimen9\dimen2
\dimen2\dimen3
\dimen3\dimen9
%\n\dimen3 \m\dimen0 \expandafter\message{\the\n/\the\m}%
}%
%
% \dimen2 *:= \numerator@/\denominator@
% \dimen0 +:= (#1)*(\dimen2)
\def\monomial@#1{%
\multiply@{\dimen2}%
\advance\dimen0 #1\dimen2
}%
%
\def\multiply@ #1{\divide#1\denominator@\multiply#1\numerator@}%
\def\multiply@@#1{\divide#1\cd@num@b\multiply#1\cd@num@a}%
\def\divide@   #1{\divide#1\numerator@  \multiply#1\denominator@}%
%
\def\square@fraction{%
   \dimen6\numerator@  \one@sp\multiply\dimen6\numerator@
   \dimen7\denominator@\one@sp\multiply\dimen7\denominator@
   \set@fraction}%
%
\def\make@division#1#2{%
   \begingroup
        \dimen@#2\relax
        \loop
           \ifdim\dimen2<.4\maxdimen
               \multiply\dimen2\tw@
               \multiply\dimen@\tw@
        \repeat
        \divide\dimen2\@cclvi
        \divide\dimen@\dimen2\relax
        \multiply\dimen@\@cclvi
        \expandafter\mk@@div\the\dimen@
   \endgroup
   %\expandafter\message{make@division=\div@@}%        
   \let#1\div@@}%
% %% this is a mega-hack for extracting as text the value of a \dimen in points
{\catcode`p=12 \catcode`0=12 \catcode`.=12 \catcode`t=12 
\gdef\mk@@div#1pt{\gdef\div@@{#1}}}%
%
%=======================================================================%
%                                                                       %
%       (20) PDFTEX SUPPORT                                             %
%                                                                       %
%=======================================================================%
%
% See /usr/share/doc/texmf/pdftex/base/example.tex
% or http://www.tug.org/applications/pdftex/
% or ftp://ftp.cstug.cz/pub/tex/local/cstug/thanh/pdftex-testing/latest
%
% \newdimen\d
% \newbox\b
% \def\avoidboxdimen#1{%
%     \setbox\b=\hbox{\box#1}%
%     \wd\b=0pt 
%     \ht\b=0pt
%     \dp\b=0pt
%     \box\b}
% 
% % rotation by `t' degrees counterclockwise is specified as 
% % `cos(t) sin(t) -sin(t) cos(t) 0 0'.
% \def\rotate@pdf{%
%     \vskip\wd0
%     \leftline{\hskip\ht0\hskip\dp0%
%     \pdf@literal{q 0 1 -1 0 0 0 cm}%
%     \avoidboxdimen0%
%     \pdf@literal{Q}}}
%
%=======================================================================%
%                                                                       %
%       (21) ERROR RECOVERY                                             %
%                                                                       %
%=======================================================================%
%
% Would be nice if we could get the error context to contain EXACTLY the
% information we want to show, in particular the inserted text as the next
% text to be input. [Could use \futurelet to show "to be read again"]
\ifx\errorcontextlines\undefined
\then   \let\no@error@context\relax
\else   \def\no@error@context{\errorcontextlines\m@ne}%
\fi
\ifnum\inputlineno<0
    % null input line strings if the info is not available
    \let\end@at@line\empty
    \let\at@line\empty
    \let\first@occur\relax
    \let\save@begin@at@line\relax
    \let\save@cell@at@line\relax
    \let\make@end@at@line\relax
    \message{! Why not upgrade to TeX version 3? (available since 1990)}%ascii
\else% input line number messages
    \def\at@line{ at line \number\inputlineno}%
    \def\first@occur{ - first occurred}%
    \def\save@begin@at@line{%
        \edef\begin@at@line{\the\inputlineno}%
        \global\let\cell@at@line\begin@at@line
        }%
    \def\begin@at@line{9999}%
    % changed \edef to \xdef 15.4.95
    \def\save@cell@at@line{%
       %\expandafter\message
        %{cell (\the\cd@row,\the\cd@cell) at \cell@at@line--\the\inputlineno}%
       \xdef\cell@at@line{\the\inputlineno}%
    }%
    \def\cell@at@line{\begin@at@line}%
    \def\make@end@at@line{%
      \ifnum\begin@at@line<\inputlineno
         \edef\end@at@line{\space at lines \begin@at@line--\the\inputlineno}%
      \else\edef\end@at@line{\at@line}%
      \fi}%
\fi
\let\end@at@line\empty
%
%
% first pass error (so can stop and give help)
\def\cd@error#1#2{\no@error@context
\errhelp=#2\expandafter\errmessage{\cd@name: #1}}%
%
% second pass error (too late to correct it)
\def\cd@refmt@error#1{\begingroup
    \expandafter\message{! \cd@name: #1\end@at@line}%ascii
    \ifnum\cd@top>\cd@row
    \ifnum\cd@bottom>\cd@row\else
    \ifnum\cd@left>\cd@cell\else
    \ifnum\cd@right>\cd@cell
       % these are ok 'cos we're in a \begingroup...\endgroup
       \advance\cd@top-\cd@row
       \advance\cd@cell-\cd@left
       \advance\cd@cell 1\relax
       \expandafter\message{! (error detected at row \the\cd@top, % ascii
       column \the\cd@cell, but probably caused elsewhere)}% ascii
    \fi\fi\fi\fi
\endgroup}%
%
% warning
\def\cd@warning#1{{%
   \expandafter\message{\cd@name\space Warning: #1\at@line}%
   }}%
%
\def\cd@obs@msg#1#2{\cd@warning{#1 \string#2 is obsolete\first@occur}}%
\def\cd@obs@dim#1{\cd@obs@msg{Dimension}{#1}%
 \glet#1\cd@obs@dimq\cd@obs@dimq}%
\def\cd@obs@dimq{\cd@dim@a=}%
\def\cd@obs@count#1{\cd@obs@msg{Count}{#1}\glet#1\@obs@countq\@obs@countq}%
\def\@obs@countq{\count@=}%
%
\def\HorizontalMapLength{\cd@obs@dim\HorizontalMapLength}%
\def\VerticalMapHeight{\cd@obs@dim\VerticalMapHeight}%
\def\VerticalMapDepth{\cd@obs@dim\VerticalMapDepth}%
\def\VerticalMapExtraHeight{\cd@obs@dim\VerticalMapExtraHeight}%
\def\VerticalMapExtraDepth{\cd@obs@dim\VerticalMapExtraDepth}%
\def\DiagonalLineSegments{\cd@obs@count\DiagonalLineSegments}%
%
%\def\spew#1{%
%\expandafter\message{#1}%
%\message{hbox0: remainder of line}\showbox0
%\message{vbox1: remainder of matrix}\showbox1
%\message{hbox2: donations from below}\showbox2
%\message{hbox3: completed verticals}\showbox3
%\message{hbox4: completed row}\showbox4
%\message{hbox5: donations upwards}\showbox5
%\message{hbox6: scratch}\showbox6
%\message{box7: donation from left}\showbox7
%\message{box8: donation from below}\showbox8
%\message{box9: scratch}\showbox9
%\message{current lists}\showlists
%}%
%
% check whether \font\tenln=line10 is really there
\ifx\tenln\nullfont
  \cd@first@use\no@tenln{\LaTeX@name\space diagonal line and arrow font
      not available}%
\else
  \let\no@tenln\relax
\fi
%
% #1=have, #2=need,
% #6=accumulator, #7=do if OK  (\cd@dim@a,\count@ scratch)
%
% #1=h,v,l,r; #2=have; #3=need; #4=message; #5=from row/col; #6=to row/col
\def\more@dim#1#2<#3:#4:#5#6{%
\begingroup
\cd@dim@b#3\relax\advance\cd@dim@b-#2\relax
\ifdim.1em<\cd@dim@b % ignore small amounts
    \cd@num@a#5\relax
    \cd@num@b#6\relax
    \ifnum\cd@num@a<\cd@num@b
        \count@\cd@num@b\advance\count@-\cd@num@a
       \cd@refmt@error{#4 by \the\cd@dim@b}%
        \if#1v%
                \let\next\vert@extra
                \edef\tmp{\the\cd@num@a--\the\cd@num@b,\the\cd@cell}%
        \else   % horizontal: correction for \across
                \advance\count@\count@
                \if#1l\advance\count@-\across@cells
                \else\if#1r\advance\count@\across@cells
                \fi\fi
                \advance\cd@dim@b\cd@dim@b
                \let\next\horiz@extra
                \edef\tmp{\the\cd@row,\the\cd@num@a--\the\cd@num@b}%
        \fi
%\cd@refmt@error
%{#4 by \the\cd@dim@b\space at (\tmp)-(\the\cd@top,\the\cd@left)}%
        \divide\cd@dim@b\count@
        \ifdim\next<\cd@dim@b\global\next\cd@dim@b\fi
\fi \fi
\endgroup             
}%
%
%
%================== erroneous occurences of \enddiagram ================
%
% \diagram\egroup\enddiagram (where \enddiagram may be inserted by \par)
% still causes trouble. same may also apply to \pile
%
% check no of lines since beginning of cell?
\new@if\if@end@diagram@ok@\@end@diagram@ok@true\@end@diagram@ok@false %global
\new@help\see@above{See the message above.}%
\new@help\par@not@allowed{Perhaps you've forgotten to end the diagram 
  before resuming the text, in\new@line which case some garbage may be added
  to the diagram, but we should be ok now.\new@line Alternatively you've
  left a blank line in the middle - TeX will now complain\new@line that the
  remaining \and@name s are misplaced - so please use comments for layout.}%
\new@help\fated@enddiagram{You have already closed too many brace pairs or
  environments; an \end@diagram@name\new@line command was (over)due.}%ascii
\new@help\pair@diagram@end{\diagram@name\space and \end@diagram@name\space
  commands must match.}%
%
%       (TeXbook p205) any runaway argument ended by \par is discarded
%       and replaced by \par alone;
%
% Blank line in the middle of a diagram.
% Ignore (with message) if interactive (\inputlineno=0)
\def\par@enddiagram{%
\ifnum  \inputlineno=0
%\then  \expandafter\interactive@par@endcd
\else   \expandafter\@par@enddiagram
\fi}%
%
\def\@par@enddiagram{%
\end@label              % terminate label
\enddiagram@endpile     % and \pile if necessary
\crcr                   % terminate row of matrix
\cd@error{missing \end@diagram@name\space inserted before \par@name -
type "h"}%ascii
\par@not@allowed
\enddiagram             % terminate diagram
\make@found@end@diagram\par@name
\par}%          % try again to end the paragraph, or whatever we wanted to do
%
% No point - can't seem to suppress the similar (vir)TeX message.
%\def\interactive@par@endcd{\expandafter\message
%{Please type a diagram command or say `\end@diagram@name'}}%
%
\def\make@found@end@diagram#1{%
\edef\enddiagram{\noexpand\found@end@diagram{#1\at@line}}}%
%
\def\found@end@diagram#1{%
\cd@error{\end@diagram@name\space (anticipated by #1) ignored}%ascii
\see@above\let\enddiagram\misplaced@enddiagram}%
%
\def\misplaced@enddiagram{%
\cd@error{misplaced \end@diagram@name\space ignored}\pair@diagram@end}%
%
\def\do@fated@enddiagram{%
\cd@error{missing \end@diagram@name\space inserted.}\fated@enddiagram
\make@found@end@diagram{closing group}}%
%
% Support for LaTeX2e \usepackage options.
% We don't use the official mechanism (\DeclareOption{name}{code}) because
% it deletes the code and does not handle our name=value construct.
% Instead we pick up everything using the LaTeX2e default option mechanism,
% which provides the user's options to us one by one as \CurrentOption.
% This doesn't pick up the \documentclass options.
% 
\ifx\DeclareOption\undefined\else\ifx\DeclareOption\@notprerr\else
   \DeclareOption*{%ascii
      \let\after@opt@arg\relax\let\next@opt@arg\relax
      \expandafter\@@getoptarg\CurrentOption,%
   }%
   %\AtEndOfPackage{%
       %\@was@pair@false
       %\ProcessOptions\relax
       %\if@was@pair@\bad@pair@opt\fi
   %}%
\fi\fi
%
%%======================================================================%
%%                                                                      %
%%      (22) AUXILLARY MACROS FOR ADJUSTMENT OF COMPONENTS              %
%%                                                                      %
%%======================================================================%

%% NOTE: The recommended way of defining arrow commands is now
%%      \newarrow{Name}{tail}{filler}{middle}{filler}{head}
%% which defines \rName, \lName, \dName and \uName using arrow parts which
%% have themselves previously been defined using the commands
%% \newarrowtail, \newarrowfiller, \newarrowmiddle and \newarrowhead.

%% The components \rhvee etc have been retained for the time being, as an
%% intermediate stage and to continue to support the old \HorizontalMap and
%% \VerticalMap commands, but you should not rely on the continued existence
%% of these macros.

%% The various components usually need some correction
%% - longitudinally, ie to prevent gaps and overprints with the shaft,
%% - transversally,  ie to prevent "steps" in the junction with the shaft.
%% The former can be done safely ad hoc, eg with \mkern1mu.
%% The latter are now done with the macros \scriptaxis, \boldscriptaxis,
%% \shifthook and \raisehook, which include pixel corrections.

%% Please note that these and the other auxillary macros which follow are
%% interim. When it becomes clear exactly what kinds of adjustments are
%% needed for characters, this job will be done by a suitable extension
%% to the language of \newarrowhead, etc. If you have any other ideas for
%% transformations of general use please tell me.

%% By all means experiment with other characters for arrowheads, but
%% please, in your own interests, do not rely on macros like \rhvee,
%% send me a copy of your definitions for distribution to other users
%% in this file, and keep track of where your efforts get copied so
%% that they can be replaced with the "official" version when it is
%% incorporated.

%% ***** DONT use macros with mangled names like \Cd@gH. *****

\catcode`\$=3 %% make sure that $ means maths-shift
\def\vboxtoz{\vbox to\z@}%% \z@ is in plain TeX and means 0pt
%\def\ulapm#1{\vboxtoz{\vss\hbox{$#1$}\kern\z@}%
%\def\dlapm#1{\vboxtoz{\kern\z@\hbox{$#1$}\vss\kern\z@}%

%% print #1 in \scriptstyle, adjusting for the maths axis height
\def\scriptaxis#1{\@scriptaxis{$\scriptstyle#1$}}%%
\def\ssaxis#1{\@ssaxis{$\scriptscriptstyle#1$}}%%
\def\@scriptaxis#1{%
\dimen0\axisheight\advance\dimen0-\ss@axisheight%
\raise\dimen0\hbox{#1}}%
\def\@ssaxis#1{%
\dimen0\axisheight\advance\dimen0-\ss@axisheight%
\raise\dimen0\hbox{#1}}%

%% Some of the characters would look better in bold since they're
%% taken from sub/superscript fonts; we use LaTeX's \boldmath to
%% do this, defining this to do nothing if it doesn't exist.
%% With the old LaTeX font selection at other than 10pt you may still
%% get nothing happenning.  Also, PK fonts may be missing.
%% If you have problems, DONT use boldhook or boldlittlevee.
\ifx\boldmath\undefined%%
     \let\boldscriptaxis\scriptaxis%%
     \def\boldscript#1{\hbox{$\scriptstyle#1$}}%%
     \def\boldscriptscript#1{\hbox{$\scriptscriptstyle#1$}}%%
\else\def\boldscriptaxis#1{\@scriptaxis{\boldmath$\scriptstyle#1$}}%%
     \def\boldscript#1{\hbox{\boldmath$\scriptstyle#1$}}%%
     \def\boldscriptscript#1{\hbox{\boldmath$\scriptscriptstyle#1$}}%%
\fi

%%  #1= {} or \boldmath; #2= + or -; #3=\subset or \supset
\def\raisehook#1#2#3{\hbox{%
\setbox3=\hbox{#1$\scriptscriptstyle#3$}%% the character to use
\dimen0\ss@axisheight%% \scriptscriptstyle axis height
\dimen1\axisheight\advance\dimen1-\dimen0%% difference in axis heights
\dimen2\ht3\advance\dimen2-\dimen0%%  height of char above axis (half spread)
\advance\dimen2-0.021em% \raisehookfudge used in THM 9.4.2 of my book
%\advance\dimen2-.5\rounded@breadth% (dont) need to adjust for rule thickness
\advance\dimen1 #2\dimen2%% shift = axis_difference +/- half_spread
%\expandafter\message{\the\dimen1}%
\raise\dimen1\box3}}%% print the character
%
%\expandafter\message{\new@line\new@line raisehook fudged by \the\raisehookfudge\new@line\new@line}%
%
%% Mark Dawson suggested using the width
% see sym.mf for MetaFont definitions of \cup and \cap (12u wide)
% subtract 2u from its width to remove the MF-encoded margin 
% also subtract \rounded@breadth to match up the shaft
% except that 2\rounded@breadth seems to work better (9.7.98)
% ptbook+boldmath+box0 gave a strut, so changed to \box1 (9.7.98)
\def\shifthook#1#2#3{% #1= {} or \boldmath; #2= + or -   #3= \cup or \cap
\setbox1=\hbox{#1$\scriptscriptstyle#3$}% the character
\dimen0\wd1\divide\dimen0 12\pixel@round{\dimen0}%%  "u"
\dimen1\wd1\advance\dimen1-2\dimen0
%\advance\dimen1-2\intended@breadth
\advance\dimen1-2\rounded@breadth
\pixel@round{\dimen1}%
\kern#2\dimen1\box1}%% print

%% use the extension font (cmex) for double vertical arrows
% and braces
\def\@cmex{\mathchar"03}%%ascii double quote

%%      ************* P U L L B A C K S ************

%% These will probably be replaced by something less ad hoc
%% in a future version.

\def\make@pbk#1{\setbox\tw@\hbox to\z@{#1}\ht\tw@\z@\dp\tw@\z@\box\tw@}%
\def\overprint@pbk#1{\overprint{\hbox to\z@{#1}}}%
\def\pbk@sh{\kern0.11em}\def\pbk@osh{\kern0.35em}%

%% This is a hack for my book ``Practical Foundations of Mathematics''
%% and WILL NOT BE SUPPORTED --- DO NOT USE IT!
\def\dblvert{\def\pbk@shsh{\kern .5\PileSpacing}}\def\pbk@shsh{}%

\def\SEpbk{\make@pbk{%
\pbk@sh\pbk@shsh
\vrule depth 2.87ex height -2.75ex width 0.95em
\vrule height -0.66ex depth 2.87ex width 0.05em
\hss
}}

\def\SWpbk{\make@pbk{%
\hss
\vrule height -0.66ex depth 2.87ex width 0.05em
\vrule depth 2.87ex height -2.75ex width 0.95em
\pbk@sh\pbk@shsh
}}

\def\NEpbk{\make@pbk{%
\pbk@sh\pbk@shsh
\vrule depth -3.81ex height 4.00ex width 0.95em
\vrule height 4.00ex depth -1.72ex width 0.05em
\hss
}}

\def\NWpbk{\make@pbk{%
\hss
\vrule height 4.00ex depth -1.72ex width 0.05em
\vrule depth -3.81ex height 4.00ex width 0.95em
\pbk@sh\pbk@shsh
}}

%%  Freyd & Scedrov puncture symbol for non-commuting polygon
\def\puncture{{\setbox0\hbox{A}%
  \vrule height.53\ht0 depth-.47\ht0 width.35\ht0
  \kern .12\ht0
  \vrule height\ht0 depth-.65\ht0 width.06\ht0
  \kern-.06\ht0
  \vrule height.35\ht0 depth0pt width.06\ht0
  \kern .12\ht0
  \vrule height.53\ht0 depth-.47\ht0 width.35\ht0
}}%


%% 2-cells: (24.11.95)
%% \NEclck puts a clockwise (ie southeast) arrow to the northwest of cell etc
\def\NEclck{\overprint{\raise2.5ex\rlap{ \pbk@shsh$\scriptstyle\searrow$}}}%%
\def\NEanti{\overprint{\raise2.5ex\rlap{ \pbk@shsh$\scriptstyle\nwarrow$}}}%%
\def\NWclck{\overprint{\raise2.5ex\llap{$\scriptstyle\nearrow$ \pbk@shsh}}}%%
\def\NWanti{\overprint{\raise2.5ex\llap{$\scriptstyle\swarrow$ \pbk@shsh}}}%%
\def\SEclck{\overprint{\lower1ex\rlap{ \pbk@shsh$\scriptstyle\swarrow$}}}%%
\def\SEanti{\overprint{\lower1ex\rlap{ \pbk@shsh$\scriptstyle\nearrow$}}}%%
\def\SWclck{\overprint{\lower1ex\llap{$\scriptstyle\nwarrow$ \pbk@shsh}}}%%
\def\SWanti{\overprint{\lower1ex\llap{$\scriptstyle\searrow$ \pbk@shsh}}}

%%======================================================================%
%%                                                                      %
%%      (23) BITS OF ARROWS                                             %
%%                                                                      %
%%======================================================================%

%%       **********  H E A D S ***********

%% \diagramstyle[heads=xxx] defines {>} as {xxx} where xxx
%% has been defined by \newarrowhead{xxx} and \newarrowtail{xxx}

%% vee head
\def\rhvee{\mkern-10mu\greaterthan}%%
\def\lhvee{\lessthan\mkern-10mu}%%
\def\dhvee{\vboxtoz{\vss\hbox{$\vee$}\kern0pt}}%%
\def\uhvee{\vboxtoz{\hbox{$\wedge$}\vss}}%%
\newarrowhead{vee}\rhvee\lhvee\dhvee\uhvee

%% little vee head
\def\dhlvee{\vboxtoz{\vss\hbox{$\scriptstyle\vee$}\kern0pt}}%%
\def\uhlvee{\vboxtoz{\hbox{$\scriptstyle\wedge$}\vss}}%%
\newarrowhead{littlevee}{\mkern1mu\scriptaxis\rhvee}%
   {\scriptaxis\lhvee}\dhlvee\uhlvee
\ifx\boldmath\undefined%%
   \newarrowhead{boldlittlevee}{\mkern1mu\scriptaxis\rhvee}%
   {\scriptaxis\lhvee}\dhlvee\uhlvee
\else%%
   \def\dhblvee{\vboxtoz{\vss\boldscript\vee\kern0pt}}%%
   \def\uhblvee{\vboxtoz{\boldscript\wedge\vss}}%%
   \newarrowhead{boldlittlevee}{\mkern1mu\boldscriptaxis\rhvee}%
   {\boldscriptaxis\lhvee}\dhblvee\uhblvee%%
\fi

%% curly vee head (uses AMS symbols fonts)
\def\rhcvee{\mkern-10mu\succ}%%
\def\lhcvee{\prec\mkern-10mu}%%
\def\dhcvee{\vboxtoz{\vss\hbox{$\curlyvee$}\kern0pt}}%%
\def\uhcvee{\vboxtoz{\hbox{$\curlywedge$}\vss}}%%
\newarrowhead{curlyvee}\rhcvee\lhcvee\dhcvee\uhcvee

%% double vee head %% will probably be withdrawn later
\def\rhvvee{\mkern-13mu\gg}%% 24.8.92 changed 10mu to 13mu
\def\lhvvee{\ll\mkern-13mu}%% to make rule go through
\def\dhvvee{\vboxtoz{\vss\hbox{$\vee$}\kern-.6ex\hbox{$\vee$}\kern0pt}}%%
\def\uhvvee{\vboxtoz{\hbox{$\wedge$}\kern-.6ex
\hbox{$\wedge$}\vss}}%%
\newarrowhead{doublevee}\rhvvee\lhvvee\dhvvee\uhvvee

%% open and closed triangles (uses AMS symbols fonts)
\def\triangleup{{\scriptscriptstyle\bigtriangleup}}%%
\def\littletriangledown{{\scriptscriptstyle\triangledown}}%% AMS
\def\rhtriangle{\triangleright\mkern1.2mu}%% 29.1.93
\def\lhtriangle{\triangleleft\mkern.8mu}%%
\def\uhtriangle{\vbox{%
   \kern-.2ex % 15.1.93 from -.05ex
   \hbox{$\scriptscriptstyle\bigtriangleup$}%
   \kern-.25ex}}%%
%% Changed \scriptstyle\triangledown to \scriptscriptstyle\bigtriangledown
%% at the suggestion of Martin Hofmann (25.11.92) to avoid using AMS symbols
%% and also for compatibility with upward arrow.
\def\dhtriangle{\vbox{%
     \kern-.28ex % 15.1.93 from -.25
     \hbox{$\scriptscriptstyle\bigtriangledown$}%
     \kern-.1ex}}%% 15.1.93 from -.25ex
\def\dhblack{\vbox{\kern-.25ex\nointerlineskip
     \hbox{$\blacktriangledown$}}}%% AMS
\def\uhblack{\vbox{\kern-.25ex\nointerlineskip
     \hbox{$\blacktriangle$}}}%% AMS
\def\dhlblack{\vbox{\kern-.25ex\nointerlineskip
     \hbox{$\scriptstyle\blacktriangledown$}}}%% AMS
\def\uhlblack{\vbox{\kern-.25ex\nointerlineskip
     \hbox{$\scriptstyle\blacktriangle$}}}%% AMS
\newarrowhead{triangle}\rhtriangle\lhtriangle\dhtriangle\uhtriangle
\newarrowhead{blacktriangle}{\mkern-1mu\blacktriangleright\mkern.4mu}% 29.1.93
     {\blacktriangleleft}\dhblack\uhblack
\newarrowhead{littleblack}{\mkern-1mu\scriptaxis\blacktriangleright}%
     {\scriptaxis\blacktriangleleft\mkern-2mu}\dhlblack\uhlblack

%% LaTeX arrowheads
\def\rhla{\hbox{\setbox0=\lnchar55\dimen0=\wd0%
\kern-.6\dimen0\ht0\z@ % 15.1.93 from -.5; also smashed height
\raise\axisheight\box0\kern.1\dimen0}}%%
\def\lhla{\hbox{\setbox0=\lnchar33\dimen0=\wd0%
\kern.05\dimen0\ht0\z@ % 15.1.93 from -.1; also smashed height
\raise\axisheight\box0\kern-.5\dimen0}}%%
\def\dhla{\vboxtoz{\vss\rlap{\lnchar77}}}%%
\def\uhla{\vboxtoz{\setbox0=\lnchar66 \wd0\z@\kern-.15\ht0\box0\vss}}%% 1/93
\newarrowhead{LaTeX}\rhla\lhla\dhla\uhla

%% double LaTeX arrowheads %% will probably be withdrawn later
\def\lhlala{\lhla\kern.3em\lhla}%%
\def\rhlala{\rhla\kern.3em\rhla}%%
\def\uhlala{\hbox{\uhla\raise-.6ex\uhla}}%%
\def\dhlala{\hbox{\dhla\lower-.6ex\dhla}}%%
\newarrowhead{doubleLaTeX}\rhlala\lhlala\dhlala\uhlala

%% circles % \rho is a Greek letter!
\def\hhO{\scriptaxis\bigcirc\mkern.4mu}
\def\hho{{\circ}\mkern1.2mu}%
\newarrowhead{o}\hho\hho\circ\circ%%
\newarrowhead{O}\hhO\hhO{\scriptstyle\bigcirc}{\scriptstyle\bigcirc}%%

%% crosses
\def\rhtimes{\mkern-5mu{\times}\mkern-.8mu}%
\def\lhtimes{\mkern-.8mu{\times}\mkern-5mu}%
\def\uhtimes{\setbox0=\hbox{$\times$}\ht0\axisheight\dp0-\ht0\lower\ht0\box0 }%
\def\dhtimes{\setbox0=\hbox{$\times$}\ht0\axisheight\box0 }%
\newarrowhead{X}\rhtimes\lhtimes\dhtimes\uhtimes
\newarrowhead+++++%ascii

%% empty head {} is also available

%% Y from stmaryrd (vertical ones still need large adjustment)
% \Yup and \Ydown swapped 26.2.2007
\newarrowhead{Y}{\mkern-3mu\Yright}{\Yleft\mkern-3mu}\Ydown\Yup

%%       **********  H E A D S  with  S H A F T S  ***********

%% little arrow with shaft
\newarrowhead{->}\rightarrow\leftarrow\downarrow\uparrow

%% arrow with double shaft
%%\newarrowhead{=>}\Rightarrow\Leftarrow\Downarrow\Uparrow
\newarrowhead{=>}\Rightarrow\Leftarrow{\@cmex7F}{\@cmex7E}% 16.1.93

%% harpoon with shaft (trailing up/left can be changed to down/right)
% shift verticals to balance! ######## (uses AMS symbols fonts)
\newarrowhead{harpoon}\rightharpoonup\leftharpoonup\downharpoonleft
\upharpoonleft

%% little double-headed arrow with shaft (uses AMS symbols fonts)
\def\twoheaddownarrow{\rlap{$\downarrow$}\raise-.5ex\hbox{$\downarrow$}}%%
\def\twoheaduparrow{\rlap{$\uparrow$}\raise.5ex\hbox{$\uparrow$}}%%
\newarrowhead{->>}\twoheadrightarrow\twoheadleftarrow\twoheaddownarrow
\twoheaduparrow

%%       **********  T A I L S ***********

%% vee tail
\def\rtvee{\greaterthan}%%
\def\ltvee{\mkern-1mu{\lessthan}\mkern.4mu}%% \mkern added 15.1.93
%\def\dtvee{\vboxtoz{\vss\hbox{$\vee$}\kern0pt}}%%
%\def\utvee{\vboxtoz{\hbox{$\wedge$}\vss}}%%
\def\dtvee{\vee}%%
\def\utvee{\wedge}%%
\newarrowtail{vee}\greaterthan\ltvee\vee\wedge

%% little vee tail
\newarrowtail{littlevee}{\scriptaxis\greaterthan}%
   {\mkern-1mu\scriptaxis\lessthan}%
   {\scriptstyle\vee}{\scriptstyle\wedge}%
\ifx\boldmath\undefined
   \newarrowtail{boldlittlevee}{\scriptaxis\greaterthan}%
   {\mkern-1mu\scriptaxis\lessthan}%
   {\scriptstyle\vee}{\scriptstyle\wedge}%
\else
   \newarrowtail{boldlittlevee}{\boldscriptaxis\greaterthan}%
   {\mkern-1mu\boldscriptaxis\lessthan}%
   {\boldscript\vee}{\boldscript\wedge}%
\fi

%% curly vee tail (uses AMS symbols fonts)
\newarrowtail{curlyvee}\succ{\mkern-1mu{\prec}\mkern.4mu}\curlyvee\curlywedge

%% open and closed triangle tails (uses AMS symbols fonts)
\def\rttriangle{\mkern1.2mu\triangleright}%% 29.1.93
\newarrowtail{triangle}\rttriangle\lhtriangle\dhtriangle
\uhtriangle
\newarrowtail{blacktriangle}\blacktriangleright
     {\mkern-1mu\blacktriangleleft\mkern.4mu}%
\dhblack\uhblack
\newarrowtail{littleblack}{\scriptaxis\blacktriangleright\mkern-2mu}%
     {\mkern-1mu\scriptaxis\blacktriangleleft}\dhlblack\uhlblack

%% LaTeX tails
\def\rtla{\hbox{\setbox0=\lnchar55\dimen0=\wd0%
\kern-.5\dimen0\ht0\z@% 19.1.93 smashed height
\raise\axisheight\box0\kern-.2\dimen0}}%%
\def\ltla{\hbox{\setbox0=\lnchar33\dimen0=\wd0\kern-.15\dimen0\ht0\z@
\raise\axisheight\box0\kern-.5\dimen0}}%%
\def\dtla{\vbox{\setbox0=\rlap{\lnchar77}%
\dimen0=\ht0\kern-.7\dimen0\box0\kern-.1\dimen0}}%% 15.1.93 from -.6
\def\utla{\vbox{\setbox0=\rlap{\lnchar66}%
\dimen0=\ht0\kern-.1\dimen0\box0\kern-.6\dimen0}}%%
\newarrowtail{LaTeX}\rtla\ltla\dtla\utla

%% double vee tail %% will probably be withdrawn later
\def\rtvvee{\gg\mkern-3mu}%%
\def\ltvvee{\mkern-3mu\ll}%%
\def\dtvvee{\vbox{\hbox{$\vee$}\kern-.6ex
\hbox{$\vee$}\vss}}%%
\def\utvvee{\vbox{\vss\hbox{$\wedge$}\kern-.6ex
\hbox{$\wedge$}\kern\z@}}%%
\newarrowtail{doublevee}\rtvvee\ltvvee\dtvvee\utvvee

%% double LaTeX tails %% will probably be withdrawn later
\def\ltlala{\ltla\kern.3em\ltla}%%
\def\rtlala{\rtla\kern.3em\rtla}%%
\def\utlala{\hbox{\utla\raise-.6ex\utla}}%%
\def\dtlala{\hbox{\dtla\lower-.6ex\dtla}}%%
\newarrowtail{doubleLaTeX}\rtlala\ltlala\dtlala\utlala

% single dotted line tail (eh?)
%\def\htdot{\mkern3.15mu\cdot\mkern3.15mu}%%
%\def\vtdot{\vbox to 1.46ex{\vss\hbox{$\cdot$}}}

%% bar (as in \mapsto)
\def\utbar{\vrule height 0.093ex depth0pt width 0.4em}%%
\let\dtbar\utbar%%
\def\rtbar{\mkern1.5mu\vrule height 1.1ex depth.06ex width .04em\mkern1.5mu}%%
\let\ltbar\rtbar%%
\newarrowtail{mapsto}\rtbar\ltbar\dtbar\utbar%%
\newarrowtail{|}\rtbar\ltbar\dtbar\utbar%%ascii vertical bar (|)

%% hooks (as in \into): choice of after/above and before/below

\def\rthooka{\raisehook{}+\subset\mkern-1mu}%%
\def\lthooka{\mkern-1mu\raisehook{}+\supset}%%
\def\rthookb{\raisehook{}-\subset\mkern-2mu}%%
\def\lthookb{\mkern-1mu\raisehook{}-\supset}%%

\def\dthooka{\shifthook{}+\cap}%%
\def\dthookb{\shifthook{}-\cap}%%
\def\uthooka{\shifthook{}+\cup}%%
\def\uthookb{\shifthook{}-\cup}%%

\newarrowtail{hooka}\rthooka\lthooka\dthooka\uthooka
\newarrowtail{hookb}\rthookb\lthookb\dthookb\uthookb

\ifx\boldmath\undefined
  \newarrowtail{boldhooka}\rthooka\lthooka\dthooka\uthooka
  \newarrowtail{boldhookb}\rthookb\lthookb\dthookb\uthookb
  \newarrowtail{boldhook}\rthooka\lthooka\dthookb\uthooka
\else
  \def\rtbhooka{\raisehook\boldmath+\subset\mkern-1mu}%%
  \def\ltbhooka{\mkern-1mu\raisehook\boldmath+\supset}%%
  \def\rtbhookb{\raisehook\boldmath-\subset\mkern-2mu}%%
  \def\ltbhookb{\mkern-1mu\raisehook\boldmath-\supset}%%
  \def\dtbhooka{\shifthook\boldmath+\cap}%%
  \def\dtbhookb{\shifthook\boldmath-\cap}%%
  \def\utbhooka{\shifthook\boldmath+\cup}%%
  \def\utbhookb{\shifthook\boldmath-\cup}%%
  \newarrowtail{boldhooka}\rtbhooka\ltbhooka\dtbhooka\utbhooka
  \newarrowtail{boldhookb}\rtbhookb\ltbhookb\dtbhookb\utbhookb
  \newarrowtail{boldhook}\rtbhooka\ltbhooka\dtbhooka\utbhooka
\fi

%% square-ended hooks (used for closed subsets in ``lifting and gluing'')
\def\dtsqhooka{\shifthook{}+\sqcap}%%
\def\dtsqhookb{\shifthook{}-\sqcap}%%
\def\ltsqhooka{\mkern-1mu\raisehook{}+\sqsupset}%%
\def\ltsqhookb{\mkern-1mu\raisehook{}-\sqsupset}%%
\def\rtsqhooka{\raisehook{}+\sqsubset\mkern-1mu}%%
\def\rtsqhookb{\raisehook{}-\sqsubset\mkern-2mu}%%
\def\utsqhooka{\shifthook{}+\sqcup}%%
\def\utsqhookb{\shifthook{}-\sqcup}%%
\newarrowtail{sqhook}\rtsqhooka\ltsqhooka\dtsqhooka\utsqhooka

%% the following seem the better choices at 10pt & 300dpi
\newarrowtail{hook}\rthooka\lthookb\dthooka\uthooka
\newarrowtail{C}\rthooka\lthookb\dthooka\uthooka

%% circles
\newarrowtail{o}\hho\hho\circ\circ%%
\newarrowtail{O}\hhO\hhO{\scriptstyle\bigcirc}{\scriptstyle\bigcirc}%%

%% crosses
\newarrowtail{X}\lhtimes\rhtimes\uhtimes\dhtimes
\newarrowtail+++++%ascii

%% empty tail {} is also available

%% Y from stmaryrd (vertical ones still need adjustment)
\newarrowtail{Y}\Yright\Yleft\Ydown\Yup

%% harpoon with shaft (trailing up/left can be changed to down/right)
% shift verticals to balance! ######## (uses AMS symbols fonts)
\newarrowtail{harpoon}\leftharpoondown\rightharpoondown\upharpoonright
\downharpoonright

%% arrow with double shaft
% 12.8.2009 suggested by Bostjan Gabrovsek
%%\newarrowtail{<=}\Leftarrow\Rightarrow\Uparrow\Downarrow
\newarrowtail{<=}\Leftarrow\Rightarrow{\@cmex7E}{\@cmex7F}% 

%%      **********  F I L L E R S ***********

%% shortening is up to 0.15em=2.7mu horiz and 0.35ex vertically at each end.

%% dot {.}, single rule {-} and empty {} fillers are also available

%% double and triple lines
%%\newarrowfiller{=}==\Vert\Vert%%
\newarrowfiller{=}=={\@cmex77}{\@cmex77}%% 16.1.93
\def\vfthree{\mid\!\!\!\mid\!\!\!\mid}%%ascii
\newarrowfiller{3}\equiv\equiv\vfthree\vfthree

% use the extension font: double vertical="305 or "37F

%% dashed line
\def\vfdashstrut{\vrule width0pt height1.3ex depth0.7ex}%%
\def\vfthedash{\vrule width\intended@breadth height0.6ex depth 0pt}%%
\def\hfthedash{\set@axis\vrule\horizhtdp width 0.26em}%%
\def\hfdash{\mkern5.5mu\hfthedash\mkern5.5mu}%%
\def\vfdash{\vfdashstrut\vfthedash}%%
\newarrowfiller{dash}\hfdash\hfdash\vfdash\vfdash

%%      ************* M I D D L E S ************

% corners for bent lines
%\def\dmcornervert{\vrule width\intended@breadth height\intended@breadth}%%
%\def\rdmcorner{\kern.4em\dmcornervert\vrule width .4em \horizhtdp}%%
%\def\ldmcorner{\vrule width .4em \horizhtdp\dmcornervert\kern.4em}%%
%\def\rumcorner{\kern.4em\vrule width .4em \horizhtdp}%%
%\def\lumcorner{\vrule width .4em \horizhtdp\kern.4em}%%
%\def\urmcorner{\mkern-4.2mu}%%
%\let\drmcorner\urmcorner\let\dlmcorner\urmcorner\let\ulmcorner\urmcorner

%% plus
\newarrowmiddle+++++%ascii

%%      ************* D I A G O N A L S ************

%% simple arrow heads
%%\def\nwhTO{\nwarrow\mkern-1mu}%%
%%\def\nehTO{\mkern-.1mu\nearrow}%%
%%\def\sehTO{\searrow\mkern-.02mu}%%
%%\def\swhTO{\mkern-.8mu\swarrow}%%


%%======================================================================%
%%                                                                      %
%%      (24) ARROW COMMANDS                                             %
%%                                                                      %
%%======================================================================%

%% change to \iftrue to get mixed heads
\iffalse%%
\newarrow{To}----{vee}%%
\newarrow{Arr}----{LaTeX}%%
\newarrow{Dotsto}....{vee}%%
\newarrow{Dotsarr}....{LaTeX}%%
\newarrow{Dashto}{}{dash}{}{dash}{vee}%%
\newarrow{Dasharr}{}{dash}{}{dash}{LaTeX}%%
\newarrow{Mapsto}{mapsto}---{vee}%%
\newarrow{Mapsarr}{mapsto}---{LaTeX}%%
\newarrow{IntoA}{hooka}---{vee}%%
\newarrow{IntoB}{hookb}---{vee}%%
\newarrow{Embed}{vee}---{vee}%%
\newarrow{Emarr}{LaTeX}---{LaTeX}%%
\newarrow{Onto}----{doublevee}%%
\newarrow{Dotsonarr}....{doubleLaTeX}%%
\newarrow{Dotsonto}....{doublevee}%%
\newarrow{Dotsonarr}....{doubleLaTeX}%%
\else%%
\newarrow{To}---->%%
\newarrow{Arr}---->%%
\newarrow{Dotsto}....>%%
\newarrow{Dotsarr}....>%%
\newarrow{Dashto}{}{dash}{}{dash}>%%
\newarrow{Dasharr}{}{dash}{}{dash}>%%
\newarrow{Mapsto}{mapsto}--->%%
\newarrow{Mapsarr}{mapsto}--->%%
\newarrow{IntoA}{hooka}--->%%
\newarrow{IntoB}{hookb}--->%%
\newarrow{Embed}>--->%%
\newarrow{Emarr}>--->%%
\newarrow{Onto}----{>>}%%
\newarrow{Dotsonarr}....{>>}%%
\newarrow{Dotsonto}....{>>}%%
\newarrow{Dotsonarr}....{>>}%%
\fi%%

\newarrow{Implies}===={=>}%% minimum cell height 9.5pt
\newarrow{Project}----{triangle}%%
\newarrow{Pto}----{harpoon}%% partial function
\newarrow{Relto}{harpoon}---{harpoon}%% binary relation

\newarrow{Eq}=====%%
\newarrow{Line}-----%%
\newarrow{Dots}.....%%
\newarrow{Dashes}{}{dash}{}{dash}{}%%

%% square hooked arrow (used in my ``gluing and lifting'' paper)
\newarrow{SquareInto}{sqhook}--->

%% braces and parentheses
%% \newarrow gives inappropriate directions, so we change the names
%% the vertical filler is too far to the right; horizontal too high
%% the vertical middles are too low with midvshaft
%% maybe we'll add square brackets and the integral sign one day
\newarrowhead{cmexbra}{\@cmex7B}{\@cmex7C}{\@cmex3B}{\@cmex38}%%
\newarrowtail{cmexbra}{\@cmex7A}{\@cmex7D}{\@cmex39}{\@cmex3A}%%
\newarrowmiddle{cmexbra}{\braceru\bracelu}{\bracerd\braceld}%
{\vcenter{\hbox@maths{\@cmex3D\mkern-2mu}}}%% right
{\vcenter{\hbox@maths{\mkern 2mu\@cmex3C}}}%% left
\newarrow{@brace}{cmexbra}-{cmexbra}-{cmexbra}%% braces
\newarrow{@parenth}{cmexbra}---{cmexbra}%% straight parentheses
\def\rightBrace{\d@brace[thick,cmex]}%%ASCII square brackets []
\def\leftBrace {\u@brace[thick,cmex]}%%ASCII square brackets []
\def\upperBrace{\r@brace[thick,cmex]}%%ASCII square brackets []
\def\lowerBrace{\l@brace[thick,cmex]}%%ASCII square brackets []
\def\rightParenth{\d@parenth[thick,cmex]}%%ASCII square brackets []
\def\leftParenth {\u@parenth[thick,cmex]}%%ASCII square brackets []
\def\upperParenth{\r@parenth[thick,cmex]}%%ASCII square brackets []
\def\lowerParenth{\l@parenth[thick,cmex]}%%ASCII square brackets []

%% synonyms for reverse compatibility

\let\uFrom\uTo%%
\let\lFrom\lTo%%
\let\uDotsfrom\uDotsto%%
\let\lDotsfrom\lDotsto%%
\let\uDashfrom\uDashto%%
\let\lDashfrom\lDashto%%
\let\uImpliedby\uImplies%%
\let\lImpliedby\lImplies%%
\let\uMapsfrom\uMapsto%%
\let\lMapsfrom\lMapsto%%
\let\lOnfrom\lOnto%%
\let\uOnfrom\uOnto%%
\let\lPfrom\lPto%%
\let\uPfrom\uPto%%

\let\uInfromA\uIntoA%%
\let\uInfromB\uIntoB%%
\let\lInfromA\lIntoA%%
\let\lInfromB\lIntoB%%
\let\rInto\rIntoA%%
\let\lInto\lIntoA%%
\let\dInto\dIntoB%%
\let\uInto\uIntoA%%
\let\ruInto\ruIntoA%%
\let\luInto\luIntoA%%
\let\rdInto\rdIntoA%%
\let\ldInto\ldIntoA%%
%%
\let\hEq\rEq%%
\let\vEq\uEq%%
\let\hLine\rLine%%
\let\vLine\uLine%%
\let\hDots\rDots%%
\let\vDots\uDots%%
\let\hDashes\rDashes%%
\let\vDashes\uDashes%%

%%=========================================================================%
%% The following are included for reverse compatibility only.
% \NW   plain arrows (like \vector in LaTeX)
% \NWd  dotted lines with LaTeX arrowheads
% \NWl  lines without arrowheads
% \NWld dotted lines without heads
% \NWe  "embed" tails
% \NWo  "onto" ie double LaTeX arrowheads (which Henk Barendregt wanted)
% \NWod double heads and dotted lines (ditto)
%%=========================================================================%
\let\NW\luTo\let\NE\ruTo\let\SW\ldTo\let\SE\rdTo
\def\nNW{\luTo(2,3)}\def\nNE{\ruTo(2,3)}%%ascii
\def\sSW{\ldTo(2,3)}\def\sSE{\rdTo(2,3)}%%ascii
\def\wNW{\luTo(3,2)}\def\eNE{\ruTo(3,2)}%%ascii
\def\wSW{\ldTo(3,2)}\def\eSE{\rdTo(3,2)}%%ascii
\def\NNW{\luTo(2,4)}\def\NNE{\ruTo(2,4)}%%ascii
\def\SSW{\ldTo(2,4)}\def\SSE{\rdTo(2,4)}%%ascii
\def\WNW{\luTo(4,2)}\def\ENE{\ruTo(4,2)}%%ascii
\def\WSW{\ldTo(4,2)}\def\ESE{\rdTo(4,2)}%%ascii
\def\NNNW{\luTo(2,6)}\def\NNNE{\ruTo(2,6)}%%ascii
\def\SSSW{\ldTo(2,6)}\def\SSSE{\rdTo(2,6)}%%ascii
\def\WWNW{\luTo(6,2)}\def\EENE{\ruTo(6,2)}%%ascii
\def\WWSW{\ldTo(6,2)}\def\EESE{\rdTo(6,2)}%%ascii

\let\NWd\luDotsto\let\NEd\ruDotsto\let\SWd\ldDotsto\let\SEd\rdDotsto
\def\nNWd{\luDotsto(2,3)}\def\nNEd{\ruDotsto(2,3)}%%ascii
\def\sSWd{\ldDotsto(2,3)}\def\sSEd{\rdDotsto(2,3)}%%ascii
\def\wNWd{\luDotsto(3,2)}\def\eNEd{\ruDotsto(3,2)}%%ascii
\def\wSWd{\ldDotsto(3,2)}\def\eSEd{\rdDotsto(3,2)}%%ascii
\def\NNWd{\luDotsto(2,4)}\def\NNEd{\ruDotsto(2,4)}%%ascii
\def\SSWd{\ldDotsto(2,4)}\def\SSEd{\rdDotsto(2,4)}%%ascii
\def\WNWd{\luDotsto(4,2)}\def\ENEd{\ruDotsto(4,2)}%%ascii
\def\WSWd{\ldDotsto(4,2)}\def\ESEd{\rdDotsto(4,2)}%%ascii
\def\NNNWd{\luDotsto(2,6)}\def\NNNEd{\ruDotsto(2,6)}%%ascii
\def\SSSWd{\ldDotsto(2,6)}\def\SSSEd{\rdDotsto(2,6)}%%ascii
\def\WWNWd{\luDotsto(6,2)}\def\EENEd{\ruDotsto(6,2)}%%ascii
\def\WWSWd{\ldDotsto(6,2)}\def\EESEd{\rdDotsto(6,2)}%%ascii

\let\NWl\luLine\let\NEl\ruLine\let\SWl\ldLine\let\SEl\rdLine
\def\nNWl{\luLine(2,3)}\def\nNEl{\ruLine(2,3)}%%ascii
\def\sSWl{\ldLine(2,3)}\def\sSEl{\rdLine(2,3)}%%ascii
\def\wNWl{\luLine(3,2)}\def\eNEl{\ruLine(3,2)}%%ascii
\def\wSWl{\ldLine(3,2)}\def\eSEl{\rdLine(3,2)}%%ascii
\def\NNWl{\luLine(2,4)}\def\NNEl{\ruLine(2,4)}%%ascii
\def\SSWl{\ldLine(2,4)}\def\SSEl{\rdLine(2,4)}%%ascii
\def\WNWl{\luLine(4,2)}\def\ENEl{\ruLine(4,2)}%%ascii
\def\WSWl{\ldLine(4,2)}\def\ESEl{\rdLine(4,2)}%%ascii
\def\NNNWl{\luLine(2,6)}\def\NNNEl{\ruLine(2,6)}%%ascii
\def\SSSWl{\ldLine(2,6)}\def\SSSEl{\rdLine(2,6)}%%ascii
\def\WWNWl{\luLine(6,2)}\def\EENEl{\ruLine(6,2)}%%ascii
\def\WWSWl{\ldLine(6,2)}\def\EESEl{\rdLine(6,2)}%%ascii

\let\NWld\luDots\let\NEld\ruDots\let\SWld\ldDots\let\SEld\rdDots
\def\nNWld{\luDots(2,3)}\def\nNEld{\ruDots(2,3)}%%ascii
\def\sSWld{\ldDots(2,3)}\def\sSEld{\rdDots(2,3)}%%ascii
\def\wNWld{\luDots(3,2)}\def\eNEld{\ruDots(3,2)}%%ascii
\def\wSWld{\ldDots(3,2)}\def\eSEld{\rdDots(3,2)}%%ascii
\def\NNWld{\luDots(2,4)}\def\NNEld{\ruDots(2,4)}%%ascii
\def\SSWld{\ldDots(2,4)}\def\SSEld{\rdDots(2,4)}%%ascii
\def\WNWld{\luDots(4,2)}\def\ENEld{\ruDots(4,2)}%%ascii
\def\WSWld{\ldDots(4,2)}\def\ESEld{\rdDots(4,2)}%%ascii
\def\NNNWld{\luDots(2,6)}\def\NNNEld{\ruDots(2,6)}%%ascii
\def\SSSWld{\ldDots(2,6)}\def\SSSEld{\rdDots(2,6)}%%ascii
\def\WWNWld{\luDots(6,2)}\def\EENEld{\ruDots(6,2)}%%ascii
\def\WWSWld{\ldDots(6,2)}\def\EESEld{\rdDots(6,2)}%%ascii

\let\NWe\luEmbed\let\NEe\ruEmbed\let\SWe\ldEmbed\let\SEe\rdEmbed
\def\nNWe{\luEmbed(2,3)}\def\nNEe{\ruEmbed(2,3)}%%ascii
\def\sSWe{\ldEmbed(2,3)}\def\sSEe{\rdEmbed(2,3)}%%ascii
\def\wNWe{\luEmbed(3,2)}\def\eNEe{\ruEmbed(3,2)}%%ascii
\def\wSWe{\ldEmbed(3,2)}\def\eSEe{\rdEmbed(3,2)}%%ascii
\def\NNWe{\luEmbed(2,4)}\def\NNEe{\ruEmbed(2,4)}%%ascii
\def\SSWe{\ldEmbed(2,4)}\def\SSEe{\rdEmbed(2,4)}%%ascii
\def\WNWe{\luEmbed(4,2)}\def\ENEe{\ruEmbed(4,2)}%%ascii
\def\WSWe{\ldEmbed(4,2)}\def\ESEe{\rdEmbed(4,2)}%%ascii
\def\NNNWe{\luEmbed(2,6)}\def\NNNEe{\ruEmbed(2,6)}%%ascii
\def\SSSWe{\ldEmbed(2,6)}\def\SSSEe{\rdEmbed(2,6)}%%ascii
\def\WWNWe{\luEmbed(6,2)}\def\EENEe{\ruEmbed(6,2)}%%ascii
\def\WWSWe{\ldEmbed(6,2)}\def\EESEe{\rdEmbed(6,2)}%%ascii

\let\NWo\luOnto\let\NEo\ruOnto\let\SWo\ldOnto\let\SEo\rdOnto
\def\nNWo{\luOnto(2,3)}\def\nNEo{\ruOnto(2,3)}%%ascii
\def\sSWo{\ldOnto(2,3)}\def\sSEo{\rdOnto(2,3)}%%ascii
\def\wNWo{\luOnto(3,2)}\def\eNEo{\ruOnto(3,2)}%%ascii
\def\wSWo{\ldOnto(3,2)}\def\eSEo{\rdOnto(3,2)}%%ascii
\def\NNWo{\luOnto(2,4)}\def\NNEo{\ruOnto(2,4)}%%ascii
\def\SSWo{\ldOnto(2,4)}\def\SSEo{\rdOnto(2,4)}%%ascii
\def\WNWo{\luOnto(4,2)}\def\ENEo{\ruOnto(4,2)}%%ascii
\def\WSWo{\ldOnto(4,2)}\def\ESEo{\rdOnto(4,2)}%%ascii
\def\NNNWo{\luOnto(2,6)}\def\NNNEo{\ruOnto(2,6)}%%ascii
\def\SSSWo{\ldOnto(2,6)}\def\SSSEo{\rdOnto(2,6)}%%ascii
\def\WWNWo{\luOnto(6,2)}\def\EENEo{\ruOnto(6,2)}%%ascii
\def\WWSWo{\ldOnto(6,2)}\def\EESEo{\rdOnto(6,2)}%%ascii

\let\NWod\luDotsonto\let\NEod\ruDotsonto\let\SWod\ldDotsonto
\let\SEod\rdDotsonto
\def\nNWod{\luDotsonto(2,3)}\def\nNEod{\ruDotsonto(2,3)}%%ascii
\def\sSWod{\ldDotsonto(2,3)}\def\sSEod{\rdDotsonto(2,3)}%%ascii
\def\wNWod{\luDotsonto(3,2)}\def\eNEod{\ruDotsonto(3,2)}%%ascii
\def\wSWod{\ldDotsonto(3,2)}\def\eSEod{\rdDotsonto(3,2)}%%ascii
\def\NNWod{\luDotsonto(2,4)}\def\NNEod{\ruDotsonto(2,4)}%%ascii
\def\SSWod{\ldDotsonto(2,4)}\def\SSEod{\rdDotsonto(2,4)}%%ascii
\def\WNWod{\luDotsonto(4,2)}\def\ENEod{\ruDotsonto(4,2)}%%ascii
\def\WSWod{\ldDotsonto(4,2)}\def\ESEod{\rdDotsonto(4,2)}%%ascii
\def\NNNWod{\luDotsonto(2,6)}\def\NNNEod{\ruDotsonto(2,6)}%%ascii
\def\SSSWod{\ldDotsonto(2,6)}\def\SSSEod{\rdDotsonto(2,6)}%%ascii
\def\WWNWod{\luDotsonto(6,2)}\def\EENEod{\ruDotsonto(6,2)}%%ascii
\def\WWSWod{\ldDotsonto(6,2)}\def\EESEod{\rdDotsonto(6,2)}%%ascii

%%======================================================================%
%%                                                                      %
%%      (25) MISCELLANEOUS                                              %
%%                                                                      %
%%======================================================================%

\def\labelstyle{%%
   \ifincommdiag%%
      \textstyle%%
   \else%%
      \scriptstyle%%
   \fi}%%
\let\objectstyle\displaystyle

\newdiagramgrid{pentagon}%
   {0.618034,0.618034,1,1,1,1,0.618034,0.618034}%
   {1.17557,1.17557,1.902113,1.902113}

\newdiagramgrid{perspective}%
   {0.75,0.75,1.1,1.1,0.9,0.9,0.95,0.95,0.75,0.75}%
   {0.75,0.75,1.1,1.1,0.9,0.9}%

\diagramstyle[%%ascii open square bracket
dpi=300,%%              office laserwriters are usually 300 dots per inch
vmiddle,nobalance,%%    vertical and horizontal positioning
loose,%%                allow rows and columns to stretch
thin,%%                 line10 arrows; default rule thickness (TeXbook p447)
pilespacing=10pt,%%     parallel vertical separation (horizontals: half this)
shortfall=4pt,%%        distance between arrowheads and their targets
%% The following are defaulted on entry to the diagram itself.
%% l>=2em               minimum length of horizontal arrow shafts in text
%% l>=1em               ditto in diagrams
%% size=3em             cell size
%% heads=LaTeX          arrowheads
]%%ascii close square bracket

%% process options to LaTeX2e's \usepackage[options]{diagrams}
%\tracingmacros1 \tracingcommands1 \tracingonline1
\ifx\ProcessOptions\undefined\else
   \@was@pair@false\ProcessOptions\relax\if@was@pair@\bad@pair@opt\fi
\fi

%%============================== THE END ====================================
\if@cd@use@PS@
\if@pdf@
\message{| running in pdf mode -- diagonal arrows will work automatically |}%
\else
\message{| >>>>>>>> POSTSCRIPT MODE (DVIPS) IS NOW THE DEFAULT <<<<<<<<<<<<|}%
\message{|(DVI mode has not been supported since 1992 and produces inferior|}%
\message{|results which are completely unsuitable for publication. However,|}%
\message{|if you really still need it, you can still get it by loading the |}%
\message{|package using ``\string
                          \usepackage[UglyObsolete]{diagrams}'' instead. ) |}%
\fi\else
\message{| >>>>>>>> USING UGLY OBSOLETE DVI CODE - PLEASE STOP <<<<<<<<<<<<|}%
\message{|(DVI mode has not been supported since 1992 and produces inferior|}%
\message{|results which are completely unsuitable for publication - Please |}%
\message{|use the PostScript or PDF mode instead, for much better results.)|}%
\fi
\cdrestoreat %% restore old category code for @ etc
\message{===================================================================}%
%% This is the end of Paul Taylor's commutative diagrams package.


